Zero-bin subtraction and the $q_{\mathrm{T}}$ spectrum beyond leading power

In this paper, we present an algorithm to construct the qT distribution at NLO accuracy to arbitrary power precision, including the assembly of suitable zero-bin subtrahends, in a mathematically well-defined way for a generic choice of rapidity-divergence regularisation prescription. In its derivation, we divide the phase space into two sectors, the interior of the integration domain as well as the integration boundary, which we include here for the first time. To demonstrate the applicability and usefulness of our algorithm, we calculate the NNLP corrections for Higgs hadroproduction for the first time. We observe that our approximate NNLP-accurate qT spectra replicate the asymptotic behaviour of the full QCD calculation to a much better degree than the previously available results, both within the $q_{\mathrm{T}}\to 0$ limit and in the large-qT domain for all the involved partonic processes. While playing a minor role at larger transverse momenta, we show that the newly incorporated boundary contribution plays a vital role in the $q_{\mathrm{T}}\to 0$ limit, where any subleading power accuracy would be lost without them. In particular, our NNLP-accurate qT expansion can approximate the exact qT distribution up to $q_{\mathrm{T}}\sim30\,\text{GeV}$ at the percent level for rapidities $|Y_H|\lesssim 3$.

==> text/ref_generator.tex <==
\section{Introduction} \label{sec:intro} Differential observables of the Drell-Yan processes and Higgs hadroproduction play paramount roles in precisely determining the Standard Model (SM) input parameters and probing New Physics scenarios. They have therefore drawn extensive experimental and theoretical attention in the recent decades. The latest measurements of the Drell-Yan processes have been carried out by the ATLAS~\cite{ATLAS:2015iiu,ATLAS:2017rzl, ATLAS:2019zci,ATLAS:2023lsr}, CMS~\cite{CMS:2015hyl,CMS:2018ktx, CMS:2018mdl,CMS:2019raw,CMS:2020cph}~and~LHCb~\cite{LHCb:2021bjt} collaborations at the LHC at colliding energies of $\sqrt{s}=7$, $8$, and $13\,\text{TeV}$, as well as the CDF and D\O\ collaborations at $\sqrt{s}=1.96~$TeV at the Tevatron~\cite{D0:2012kms,CDF:2012gpf, CDF:2013dpa,CDF:2022hxs}. Inclusive and differential fiducial cross section measurements for Higgs boson production, on the other hand, have been presented in \cite{ATLAS:2014xzb,CMS:2015zpx,ATLAS:2017qey,CMS:2018gwt, ATLAS:2020wny,ATLAS:2022fnp,ATLAS:2022qef,ATLAS:2023hyd,ATLAS:2023pwa, CMS:2023gjz}. Along with the progress in experimental precision, strides were also made in the fixed-order calculations. The QCD corrections are known up to third order for both the Drell-Yan processes \cite{Melnikov:2006kv,Catani:2009sm,Camarda:2019zyx,Duhr:2020seh, Duhr:2021vwj,Chen:2021vtu,Chen:2022cgv,Neumann:2022lft,Baglio:2022wzu, Gehrmann-DeRidder:2023urf} and Higgs production \cite{Dawson:1990zj, Djouadi:1991tka,Spira:1995rr,Harlander:2002wh,Anastasiou:2002yz, Ravindran:2003um,Anastasiou:2015vya,Anastasiou:2016cez, Mistlberger:2018etf,Chen:2014gva,Boughezal:2015aha,Boughezal:2015dra, Chen:2016zka,Caola:2015wna,Cieri:2018oms,Billis:2021ecs,Chen:2021azt, Chen:2021isd,Cal:2023mib}. Electroweak corrections have mostly been studied for Drell-Yan production \cite{Li:2012wna,Dittmaier:2015rxo,Bonciani:2019nuy,Dittmaier:2020vra, Bonciani:2021zzf,Armadillo:2022bgm,Buccioni:2022kgy}, but are known for Higgs production as well \cite{Actis:2008ug,Anastasiou:2008tj}. Of the differential observables, the transverse momentum distribution of the colourless final state is of the particular concern in this work. Even though fixed order calculations are able to produce reliable predictions in the majority of the phase space, substantial corrections can emerge from higher perturbative order within the low~\qT~regime, as a result of soft and collinear radiation, where the bulk of the cross section resides. Hence, in order to arrive at a sufficiently convergent result in perturbation theory, a variety of the resummation techniques that are capable of exponentiating \textit{the most singular}, so-called leading power (\LP), behaviour of the~\qT~distribution at every order have been developed in the past decades. Examples are the CSS formalism~\cite{Collins:1981uk,Collins:1981va, Collins:1984kg,Catani:2000vq,Bozzi:2005wk,Bozzi:2007pn}, the momentum space resummation~\cite{Ebert:2016gcn,Monni:2016ktx,Bizon:2017rah, Bizon:2019zgf,Bizon:2018foh}, and the SCET-based analyses \cite{Becher:2010tm,GarciaEchevarria:2011rb,Becher:2011dz,Chiu:2011qc, Chiu:2012ir,Li:2016axz,Li:2016ctv}. The subsequent resummation improved \qT~distributions have been evaluated up to approximate \NNNNLL accuracy \cite{Becher:2010tm,Bozzi:2010xn, Becher:2011xn,Banfi:2011dx,Banfi:2011dm,Banfi:2012du,Catani:2015vma, Scimemi:2017etj,Bizon:2018foh,Bacchetta:2019sam,Bizon:2019zgf, Becher:2020ugp,Ebert:2020dfc,Re:2021con,Camarda:2021ict,Ju:2021lah, Camarda:2023dqn,Neumann:2022lft,Moos:2023yfa} for the Drell-Yan process and \NNNLLp in the case of Higgs production \cite{Belyaev:2005bs, Bozzi:2005wk,Becher:2020ugp,Becher:2012yn,Neill:2015roa,Bizon:2017rah, Chen:2018pzu,Bizon:2018foh,Gutierrez-Reyes:2019rug,Harlander:2014hya, Billis:2021ecs,Cal:2023mib} as to the Higgs production. Recently, to further improve the precision as well as the phase space coverage of the \qT~resummation, the factorisation pattern of \textit{the subleading power} contribution has been investigated within both the non-perturbative region $\Lambda_{H}\lesssim\qT\ll Q_H$ \cite{Balitsky:2017gis,Balitsky:2020jzt,Balitsky:2021fer, Balitsky:2017flc,Vladimirov:2021hdn,Ebert:2021jhy,Gamberg:2022lju, Rodini:2022wic,Rodini:2023plb,Vladimirov:2023aot,Rodini:2023mnh} and the perturbative zone $\Lambda_{H}\ll\qT\ll Q_H$ \cite{Ebert:2018gsn, Inglis-Whalen:2021bea,Inglis-Whalen:2022vyn}, where $\Lambda_{H}$ and $Q_H$ characterise the hadronic and hard scales in the process under consideration, respectively. At present, a resummation of those subleading power corrections has not been accomplished yet beyond \LL. Similarly, subleading power corrections also play a role in the limit $\qT\to 0$. Here, the \LP approximation can only recover the most singular behaviour of the exact distribution at any given order in a fixed-order expansion, leaving behind integrable (but numerically problematic) singularities and constant terms. These non-vanishing remainders are of particular concern in \qT-based subtraction and slicing methods for higher-order calculations \cite{Bizon:2018foh,Chen:2018pzu,Camarda:2021ict}. Related results on power suppressed contribution can be found from \cite{Oleari:2020wvt,Cieri:2019tfv,Camarda:2021jsw,Ebert:2020dfc, Ebert:2019zkb} concerning the slicing subtraction method, the endpoint singularity in the Higgs production and decay~\cite{Liu:2022ajh,Liu:2020tzd, Liu:2020eqe,Liu:2020ydl,Liu:2019oav,Liu:2021chn,Liu:2018czl,Liu:2017vkm}, the event shapes in the leptonic and hadron colliders \cite{Buonocore:2023mne,Agarwal:2023fdk,vanBeekveld:2019prq,Chen:2023wah, Ebert:2018lzn,Moult:2018jjd,Moult:2017jsg,Moult:2016fqy,Pal:2023vec}, and the threshold resummation~\cite{vanBijleveld:2023vck,vanBeekveld:2021hhv, Laenen:2020nrt,vanBeekveld:2019cks,Bonocore:2016awd,Bonocore:2015esa, Bonocore:2014wua,Laenen:2010uz,Laenen:2008gt,Laenen:2008ux, Broggio:2023pbu,Beneke:2018gvs,Beneke:2022obx,Beneke:2019oqx, Beneke:2019mua,Bonocore:2021cbv,Bhattacharya:2021hae,AH:2020qoa, Bahjat-Abbas:2019fqa,Balsach:2023ema,Engel:2023rxp,Engel:2023ifn}. To derive the factorisation formulae beyond the leading power approximation, one of the prerequisites is to consistently combine the contributions from the constituent dynamic regions, generally comprising the hard, collinear, and soft modes \cite{Balitsky:2017gis, Balitsky:2020jzt,Balitsky:2021fer,Balitsky:2017flc,Vladimirov:2021hdn, Ebert:2021jhy,Gamberg:2022lju,Rodini:2022wic,Rodini:2023plb, Vladimirov:2023aot,Rodini:2023mnh,Ebert:2018gsn,Inglis-Whalen:2021bea, Inglis-Whalen:2022vyn}.% \footnote{ The irrelevance of the Glauber vertices is presumed in the subleading power factorisation of \cite{Balitsky:2017gis,Balitsky:2020jzt, Balitsky:2021fer,Balitsky:2017flc,Vladimirov:2021hdn,Ebert:2021jhy, Gamberg:2022lju,Rodini:2022wic,Rodini:2023plb,Vladimirov:2023aot, Rodini:2023mnh,Ebert:2018gsn,Inglis-Whalen:2021bea,Inglis-Whalen:2022vyn}. Up to now, a rigorous proof of the cancellation of the Glauber contributions beyond the leading power approximation is still absent, to our best knowledge. The leading power discussion on inclusive observables can be found in~\cite{Collins:1997sr,Collins:2004nx,Gaunt:2014ska,Schwartz:2018obd}. } Although these dynamic regions are well defined in given segments of the phase space or the loop integrals, in practical calculations one often extrapolates their contributions from their respective intrinsic domains to the entire integration range, necessitating a robust systematic subtraction process to remove their overlap. This procedure is frequently referred to as the \emph{zero-bin subtraction} \cite{Manohar:2006nz,Idilbi:2007yi,Idilbi:2007ff,Chiu:2009yx}, the soft subtraction \cite{Ji:2004xq,Ji:2004wu,Idilbi:2007yi,Idilbi:2007ff, Echevarria:2011epo}, or the overlap reduction~\cite{Goerke:2017ioi, Inglis-Whalen:2020rpi,Inglis-Whalen:2021bea}. At leading power, zero-bin subtraction proceeds with deducting the soft contribution from the collinear sectors, and has been demonstrated to be valid up to \NNNLO~\cite{Echevarria:2015byo, Echevarria:2015usa,Li:2016axz,Li:2016ctv,Luo:2019hmp,Luo:2019bmw, Luo:2019szz,Luo:2020epw}. Similar conclusions can also be found in the analysis of the subleading angular coefficients (suppressed by a factor of $\qT/Q_H$ w.r.t.\ leading singular terms) in the Drell-Yan process and the semi-inclusive deep-inelastic scatterings~\cite{Vladimirov:2021hdn, Ebert:2021jhy,Gamberg:2022lju,Rodini:2023plb}. However, for the subleading inclusive observables of the Drell-Yan process the zero-bin subtraction becomes more involved, as it comprises mixed contributions in the overlapping area from the lowest power accuracy up to \NLP \cite{Inglis-Whalen:2020rpi,Inglis-Whalen:2021bea}. Even though such recipes to construct zero-bin subtractions can establish a factorisation at the \NLP level, a robust algorithm that is capable of generating zero-bin subtrahends at an arbitrary power and choice of a rapidity-divergence regularisation prescription is still missing. % Investigations towards this goal were pioneered by \cite{Jantzen:2011nz}, in which a mathematically well-defined derivation was delivered for the power series of the one-loop integrals in a variety of kinematical limits. Therein, the analysis of the massive Sudakov form factor is intimately related to the asymptotic behaviour of the \qT~distribution. Their power expansion begins with the introduction of a group of auxiliary cutoff scales along the integration path, from which the relevant scales of the process are well separated and the defining dynamic regions can be prescribed accordingly. Within these regions, the expansions are straightforward and always well-defined. This is then followed by a recombination procedure to lift all dependences on the auxiliary scales, thereby extrapolating the expanded integrands from their intrinsic domains to the entire integration range. % During this procedure, however, a set of constituents emerge, consisting of doubly and triply expanded integrands in line with their respective distinct scaling laws which account for the overlapping contributions amongst different modes and turn out to be in part the zero-bin subtrahends. While integrals with a single definite scaling rule for every integration variable are subjected only to a single expansion, multiple expansions can induce ambiguous interpretations of the resulting integral as the integration variables in general observe distinct scaling rules for each dynamic mode. Subsequently, this ambiguity limits the applicability of the formalism in \cite{Jantzen:2011nz} to only a special range of rapidity regularisation schemes, such as the analytic regulator \cite{Becher:2010tm,Becher:2011dz} and the pure rapidity regulator \cite{Ebert:2018gsn,Moult:2019vou}. % When using more generic regularisation schemes, e.g.\ the exponential regulator \cite{Li:2016axz,Li:2016ctv}, doubly and triply expanded integrals instead call for an unambiguous counting rule at each power accuracy to yield results that are independent of the scheme. % As a matter of fact, any reliance on the choice of rapidity regulators in carrying out the power expansion will hinder the establishment of the rapidity renormalisation group \cite{Chiu:2011qc}, which, akin to the renormalisation group governing the virtuality divergence, requires the equivalence of the power series resulting from various rapidity-divergence regularisation approaches. In the following, we will make use of the \NLO \qT~distribution of the process $pp\to H+X$ as a demonstrative example to accomplish this goal. Since our derivation mainly concerns the pattern of the denominators of the squared transition amplitudes, the conclusion here can also be generalised to the analysis of the Drell-Yan processes, $pp\to V+X$ with $V=W,Z$. We commence by following the strategy outlined in \cite{Jantzen:2011nz} to categorise the phase space so as to detach the emerging scales and thereby carry out the expansion in momentum space. Afterwards, instead of extrapolating the expanded integrands on the cumulative level, in this work we shift the auxiliary boundaries at a particular power accuracy only while maintaining the equality to the power series derived from the momentum space. As a result, a set of multiple expanded integrals emerge to balance the overextended collinear sectors power by power. We use these to construct the zero-bin subtrahends and thereby retrieve the scalings for the occurring integration variables. We will demonstrate that the zero-bin subtrahends proposed in this paper are straightforwardly applicable to all rapidity regulators that preserve their expressions before and after asymptotic expansions, including the analytic regulator \cite{Becher:2010tm,Becher:2011dz}, the exponential regulator \cite{Li:2016axz,Li:2016ctv}, and the pure rapidity regulator \cite{Ebert:2018gsn,Moult:2019vou}. In addition, with a few adaptations, our algorithm presented here can also be generalised to use the $\Delta$-regulator \cite{Chiu:2009yx, Echevarria:2011epo,Echevarria:2015usa,Echevarria:2015byo, Echevarria:2016scs} and the $\eta$-regulator \cite{Chiu:2011qc,Chiu:2012ir}. This accommodates the majority of the rapidity-divergence regularisation schemes in use at this time. Our paper is organised as follows. In Sec.\ \ref{sec:asyexp:mom} we develop our framework to compute, in a general way, all power corrections to \NLO accuracy. To this end, we will use Sec.~\ref{sec:qTNLO} and \ref{sec:setups}, taking the example of Higgs hadroproduction at LHC, to review the fixed order calculation on the \qT\ spectrum and thereby categorise the phase space into two sectors according to the origins of the power corrections. The first sector, associated with the asymptotic expansion of the boundary condition, will be investigated in Sec.~\ref{sec:red:qT:boundary}. The other one takes in the bulk of phase space and thus forms the main concern of this paper. We will devote Sec.~\ref{sec:red:qT:central} to elaborate on its expansion procedure, in particular highlighting the structural pattern of the emerging zero-bin subtrahends. At last, in Sec.~\ref{sec:asyexp:recap}, we combine the relevant ingredients and present the power series of the \qT\ spectrum of our example process $pp\to H+X$. Sec.~\ref{sec:asyexp:outputs} then is dedicated to the application of the framework derived in Sec.~\ref{sec:asyexp:mom}, where the power corrections will be appraised up to \NNLP for the first time. We calculate it in three different approaches, including the momentum cutoff scales, the homogenous regularisation scheme, and the inhomogeneous regulator, to regulate the rapidity divergences. We will demonstrate that after appropriate combination, all three methods result in the same analytic expressions at least up to \NNLP, echoing the rapidity renormalisation group \cite{Chiu:2011qc}. Finally, we will scrutinise our \NNLP results in Sec.~\ref{sec:asyexp:numeric} by comparing to the full QCD calculation. Eventually, we summarise our findings in Sec.~\ref{sec:conclusions}. \section{Theoretical framework}\label{sec:asyexp:mom} In this section, we introduce the formalism we derive the next-to-leading and next-to-next-to-leading power expansions, dubbed \NLP and \NNLP respectively. We will use the case of Higgs production at hadron colliders, $p+p \to H+X$, as an illustrative example. The results we derive, however, are similarly applicable to the production of any other colour-neutral final state. \subsection{Analysis of the NLO fixed order results}\label{sec:qTNLO} To introduce our notation, we start our analysis by recalling the general expression %NLO expression for the differential cross section of the process $p+p \to H+X$ in proton-proton collisions. According to the QCD factorization theorem~\cite{Collins:1989gx}, the differential \qT~spectra at NLO can be calculated as follows, \begin{align}\label{eq:qcd:qT} \frac{\done \sigma_H}{\done Y_H\, \done \qT^2} \;=\; & \frac{1}{16\pi\, s^2}\sum_{i,j} \int^{k_+^{\mathrm{max}}}_{0}\!\!\!\!\done k_+\, \int^{k_-^{\mathrm{max}}}_{0}\!\!\!\!\done k_-\, \delta(k_+k_--\qT^2)\; \frac{f_{i/n}(\xi_n)}{\xi_n}\, \frac{f _{j/\nbar}(\xi_{\nbar})}{\xi_{\nbar}}\; \overline{\sum_{\mathrm{col},\mathrm{pol}} } \big|\mathcal{M}(i+j\to H+k)\big|^2\,\nonumber\\ \;=\; & \frac{1}{16\pi\, s^2}\sum_{i,j} \int^{k_+^{\mathrm{max}}}_{k_+^{\mathrm{min}}}\, \frac{\done k_+}{k_+} \frac{f_{i/n}(\xi_n)}{\xi_n} \frac{f _{j/\nbar}(\xi_{\nbar})}{\xi_{\nbar}}\; \overline{\sum_{\mathrm{col},\mathrm{pol}} } \big|\mathcal{M}(i+j\to H+k)\big|^2\,, \end{align} where $\sqrt{s}$ denotes the collider centre-of-momentum energy of the incoming protons. $Y_H$ and $\qT$ stand for the rapidity and transverse momentum of the Higgs boson measured in the laboratory reference frame, respectively. The boundaries of the phase space integral are given by the variables $k_+^{\mathrm{max}}$ and $k_+^{\mathrm{min}}$, with \begin{align}\label{eq:def:b.c.} k_+^{\mathrm{max}}=\sqrt{s}-\mT e^{-Y_H}\,,\qquad k_+^{\mathrm{min}}=\frac{\qT^2}{k_-^{\mathrm{max}}}=\frac{\qT^2}{\sqrt{s}-\mT e^{+Y_H}}\;. \end{align} Therein, $\mT^2\equiv m_H^2+\qT^2$ is the transverse mass of the Higgs boson, $m_H$ being the mass of the Higgs boson. In the integrand of Eq.~\eqref{eq:qcd:qT}, $f_{i/n}$ and $f _{j/\nbar}$ represent the parton distribution functions (PDFs) for the partons $i$ and $j$ in the protons $n$ and $\nbar$, respectively, with the argument $\xi_{n(\nbar)}$ encoding the momentum fractions carried by the incident particle $i(j)$ with respect to its mother proton $n(\nbar)$. In this paper, we will use the 5 flavour scheme, and correspondingly, the partons $\{i,j,k\}\in\{u,\bar{u},d,\bar{d},c,\bar{c},s,\bar{s},b,\bar{b},g\}$ will be considered massless and taken fully into account in the following analysis. $|\mathcal{M}|^2$ denotes the squared amplitudes for the contributing partonic channel $i+j\to H+k$. Since the main focus of this paper is on the region where $\qT$ approaches, but is not equal to, zero, only tree level contributions will participate in Eq.~\eqref{eq:qcd:qT}. \changed{In the large top mass limit, the amplitudes for the processes $i+j\to H+k$ can be calculated in the low energy Higgs effective field theory (HEFT) \cite{Kluberg-Stern:1974iel,Nielsen:1975ph,Wilczek:1977zn,Nielsen:1977sy,Inami:1982xt,Spiridonov:1984br,Chetyrkin:1997un}. Therein, the creation and annihilation of the Higgs boson are governed by the effective Lagrangian, \begin{align} \mathcal{L}_{\text{eff}} &= \frac{\alpha_s(\mu) }{12 \pi v} C_t(m_t,\mu) G^{\mu\nu,a} G_{\mu\nu}^{a} H\, , \label{eq:Leff} \end{align} where $\alpha_s$ stands for the strong coupling constant. $v$ denotes the Higgs vacuum expectation value. $H$ and $G_{\mu\nu}^a$ represent the Higgs field operator and the gluon field strength tensor, respectively. The radiative contribution from the top quark loop is encoded by the Wilson coefficient $C_t$, which, up to now, has been calculated up to the four-loop order in the literatures~\cite{Inami:1982xt, Djouadi:1991tk, Chetyrkin:1997iv, Chetyrkin:1997un, Chetyrkin:2005ia, Schroder:2005hy, Baikov:2016tgj}. In this work, we only take into account its LO contribution in accordance with the perturbative accuracy of Eq.~\eqref{eq:qcd:qT}. In writing Eq.~\eqref{eq:Leff}, we have omitted the operators inducing the Higgs-light-quark interaction, as the 5 active flavour scheme is adhered to throughout our investigation. } \changed{ Combining Eq.~\eqref{eq:Leff} with the QCD Lagrangian enables ones to generate the squared amplitudes for the process $i+j\to H+k$. Having summed and averaged, as appropriate, over all the colour and polarisation configurations, the results read \cite{Ravindran:2002dc,Glosser:2002gm},} \begin{equation} \label{eq:msq} \begin{split} \overline{\sum_{\mathrm{col},\mathrm{pol}}} \big|\mathcal{M}(g+g\to H+g)\big|^2 &=\, \frac{3\lambda^{\changed{2}}_t}{32}\, \frac{m_H^8+s_{ij}^4+s_{ik}^4+s_{jk}^4}{s_{ij}s_{ik}s_{jk}} \,,\\ % \overline{\sum_{\mathrm{col},\mathrm{pol}}} % \big|\mathcal{M}(q(\bar{q})+g\to H+q(\bar{q}))\big|^2 % &=\, % -\frac{\lambda_t}{24}\, % \frac{s^2_{ij}+s^2_{jk}}{s_{ik}}\,,\\g+g\to H+gg+q(\bar{q})\to H+q(\bar{q}) \overline{\sum_{\mathrm{col},\mathrm{pol}}} \big|\mathcal{M}(g+q(\bar{q})\to H+q(\bar{q}))\big|^2 &= \,-\frac{\lambda^{\changed{2}}_t}{24}\,\frac{s^2_{ij}+s^2_{ik}}{s_{jk}}\,,\\ \overline{\sum_{\mathrm{col},\mathrm{pol}}} \big|\mathcal{M}(q+\bar{q}\to H+g)\big|^2 &=\, \frac{\lambda^{\changed{2}}_t}{9}\,\frac{s^2_{ik}+s^2_{jk}}{s_{ij}}\,,\\ % \overline{\sum_{\mathrm{col},\mathrm{pol}}}\big| % \mathcal{M}(\bar{q}+q\to H+g)\big|^2 % &=\,\frac{\lambda_t}{9}\,\frac{s^2_{ik}+s^2_{jk}}{s_{ij}}\,, \end{split} \end{equation} \changed{where the parameter $\lambda_t$ is introduced to collect the coupling constants, i.e., $\lambda^2_t\equiv {4\alpha_s^3C_t^2}/{(9\pi v^2)}$. The missing expressions for $q(\bar{q})g$ and $\bar{q}q$ initial states can be derived from the above by swapping the roles of $i$ and $j$. } %where the coupling parameter $\lambda_t\equiv {4\alpha_s^3C_t^2}/{(9\pi v^2)}$ collects the strong coupling constant $\alpha_s$ as well as the %vacuum expectation value $v$, and the Wilson coefficient $C_t$ %of the HEFT governing the Higgs-gluon interaction. %Up to now, $C_t$ has been calculated up to the four-loop order in %the literature~\cite{Inami:1982xt, Djouadi:1991tk, Chetyrkin:1997iv, % Chetyrkin:1997un, Chetyrkin:2005ia, Schroder:2005hy, Baikov:2016tgj}. %In this work, we only take into account its LO contribution in %accordance with the perturbative accuracy of the amplitudes of %Eq.~\eqref{eq:msq}. %The missing expressions for $q(\bar{q})g$ and $\bar{q}q$ %initial states can be derived from the above by swapping the %roles of $i$ and $j$. \changed{The expressions in Eq.~\eqref{eq:msq} involve} the scalar products of the momenta of the initial and final particles, \begin{equation} \begin{split}\label{eq:def:sji} s_{ij} =&\phantom{+}2p_i\cdot p_j =\left(k_++\mT e^{-Y_H}\right)\, \left(k_-+\mT e^{+Y_H}\right)\,,\\ s_{ik} =&-2p_i\cdot p_k= -\left(k_++\mT e^{-Y_H}\right)k_- \,, \\ s_{jk} =&-2p_j\cdot p_k= -\left(k_-+\mT e^{+Y_H}\right)k_+ \,. \end{split} \end{equation} Therein, $k_{\pm}$ denotes the light cone component of the momentum of the emitted parton $k$. To be precise, with the help of the light-like reference vectors $n^{\mu}$ and $\nbar^{\mu}$, aligned with incoming beams and satisfying $n\cdot\nbar=2$, it is defined as \begin{align} \label{eq:def:lcone} p_k^{\mu} =\frac{p_k\cdot n}{2}\nbar^{\mu} +\frac{p_k\cdot \nbar}{2}{n}^{\mu} +p_{k,\bot}^\mu \equiv\frac{k_-}{2}\nbar^{\mu} +\frac{k_+}{2}{n}^{\mu} +k_{\bot}^\mu \equiv\big[k_-,k_+,k_{\bot} \big]\,. \end{align} In this notation, the momentum fractions $\xi_n$ and $\xi_{\nbar}$ of Eq.~\eqref{eq:qcd:qT} can be written as \begin{align}\label{eq:qcd:def:Xi} \xi_n =\frac{k_++\mT e^{-Y_H}}{\sqrt{s}}\qquad\text{and}\qquad \xi_{\nbar} =\frac{k_-+\mT e^{+Y_H}}{\sqrt{s}}\;. \end{align} In the following sections, we will investigate the asymptotic properties of Eq.~\eqref{eq:qcd:qT} in the vicinity of $\qT=0$, adhering to the following definition of the expansion accuracy, counting powers of $\qT^2$, throughout, \begin{equation}\label{eq:def:acc} \begin{split} \frac{\done \sigma_H}{\done Y_H\, \done \qT^2}=& \, \underbrace{\sum_m\,\frac{\Delta_{\LP}^{(m)}\,(L_H)^m}{\qT^2}}_{\LP} \, + \, \underbrace{\sum_m\,\Delta_{\NLP}^{(m)}\,(L_H)^m}_{\NLP} \, + \, \underbrace{\sum_m\, \qT^2\,\Delta_{\NNLP}^{(m)}\,(L_H)^m }_{\NNLP} \, + \, \dots\, . \\ \end{split} \end{equation} Therein, the \qT~differential distribution in Eq.~\eqref{eq:qcd:qT} is expanded in the low \qT~domain. At a given power precision,~e.g.\ N$^{\omega+1}$LP, all non-logarithmic \qT~dependences have been collected in the pre-factor $\qT^{2\omega}$ with $(\omega\ge-1)$. They leave behind the logarithmic terms $L_H\equiv\ln[\qT^2/m_H^2]$ and the coefficient functions $\Delta_{\mathrm{N}^{\omega+1}\mathrm{LP}}^{(m)}\equiv\Delta_{\mathrm{N}^{\omega+1}\mathrm{LP}}^{(m)}[m_H,\,s,\,Y_H;\; f_{i/n},\,f_{j/\nbar}]$ which accounts for the convolution of the PDFs $f_{i/n}$ and $f_{j/\nbar}$ as well as the functions of the hard scales $s$ and $m_H$. According to this definition, the LP contribution is expected to accommodate the most singular behaviour in the low \qT~regime, while the higher power corrections experience progressively stronger suppression factor $\qT^{2(\omega-1)}$. Correspondingly, $\Delta_{\LP}$ is known extremely precisely, up to approximate fourth order \cite{Catani:2007vq,Catani:2012qa, Catani:2022sgr,Catani:2011kr,Luo:2020epw,Luo:2019szz,Ebert:2020yqt, Gehrmann:2012ze,Gehrmann:2014yya,Echevarria:2016scs,Luo:2019hmp, Luo:2019bmw,Gutierrez-Reyes:2019rug,Chetyrkin:1997iv, Chetyrkin:1997un,Gehrmann:2014vha,Gehrmann:2010ue,Baikov:2009bg, Gehrmann:2005pd,Harlander:2000mg, Duhr:2022yyp,Moult:2022xzt,Schroder:2005hy,Chetyrkin:2005ia, Lee:2022nhh,Chakraborty:2022yan}, while the $\Delta_{\NLP}$ has only been computed recently to \NLO accuracy \cite{Ebert:2018gsn}. All further higher-power corrections are hitherto unknown, and we will use the remainder of this section to introduce a mathematically well-defined approach to develop a framework to compute the $\Delta_{\mathrm{N}^{\omega+1}\mathrm{LP}}$ for all $\omega\ge-1$ at \NLO accuracy before deriving the respective \NLO-correct expression for $\Delta_\NNLP$ explicitly. In the following subsections we will be evaluating the coefficients $\Delta_{\mathrm{N}^{\omega+1}\mathrm{LP}}^{(m)}$. In Sec.~\ref{sec:setups}, we will derive additional power corrections originating from the kinematics of the process and thereby categorise the phase space integral of Eq.~\eqref{eq:qcd:qT} into two sectors. The first sector encompasses the domains in the vicinity of $k^{\mathrm{max}}_+$ and $k^{\mathrm{max}}_-$, accounting for the power suppressed contributions induced by the boundary conditions of the phase space integral, see Eq.~\eqref{eq:def:b.c.}. We will make use of Sec.~\ref{sec:red:qT:boundary} to discuss the asymptotic properties from this region. The second sector consists of the remaining regions, entailing a variety of scales along the integration path and is therefore the main concern of this paper. We will elaborate in Sec.~\ref{sec:red:qT:central} on the power expansion of this contribution. Eventually, with the results of the two, we are capable of deriving the power series for the \qT~spectrum in Sec.~\ref{sec:asyexp:recap}. % %They will be discussed in Sec.~\ref{sec:red:qT:boundary} and % %We will % % %we will investigate the power corrections in kinematics, thereby recasting the \qT~distribution in eq.~\eqref{eq:qcd:qT} into the products of a set of homogeneous functions concerning only the hard scales multiplied by the integrals accommodating distinct segments of the phase space. %%Those hard coefficients can be extracted from the squared amplitudes in Eqs.~\eqref{eq:msq} %Regarding those dynamic integrals, one sort of them account for the power suppressed corrections driven by boundary conditions of eq.~\eqref{eq:def:b.c.} and will be elaborated on in Sec.~\ref{sec:red:qT:boundary}, while the other kind of the integrals consist of the bulk of the phase space and therefore constitute the main concern of this paper. We will first of all make use of Sec.~\ref{sec:asyexp:qT:mom} to analyze their asymptotic properties in the small \qT~region from the momentum space, for which a group of dynamic regions are introduced. %Sec.~\ref{sec:asyexp:qT:extrapl} is then dedicated to performing the continuation on those restricted areas. Therein, in order to remove the ensuing overlapping contributions over the course, we propose an algorithm to exercise the zero-bin subtraction procedure, which is expected to be applicable for any choice of rapidity regulator at an arbitrary power. Eventually, in Sec.~\ref{sec:asyexp:comp}, we deliver a comparison between our strategy and those in the previous literatures. %With those ingredients at hand, we are capable of deriving the power series for the \qT~spectrum in Sec.~\ref{sec:asyexp:recap}. % % % $\mathcal{M}$ represents the amplitudes %With the usual light cone decomposition %\begin{align} % k^{\mu}=\frac{k\cdot n}{2}\nbar^{\mu}+\frac{k\cdot \nbar}{2}{n}^{\mu}+k^\mu_{\bot} %\end{align} %and the shorthands $k_-\equiv k\cdot n$ and $k_+\equiv k\cdot \nbar$, %we define % %where $\mT\equiv\sqrt{m_H^2+\qT^2}$. % % %\begin{align} % \mathcal{L}_{\mathrm{eff}}=\frac{\alpha_s}{4\pi}\frac{C_t}{3v} {G}^{\alpha,\mu \nu} {G}^{\alpha}_{\mu \nu}H %\end{align} %defines the effective Higgs-gluon interaction, with %$v$ is the Higgs vacuum expectation value; $H$ represents the physical Higgs boson after electroweak symmetry breaking; $G_{\mu\nu}^a$ is the field strength tensor of the gluon field. %In the following, we will ignore the masses of the light quarks, %but keep the Yukawa couplings $y_q$ non-vanishing. %The strong coupling $\alpha_s$, and the Wilson coefficient $C_t$ %of the effective operator are renormalised in the %$\overline{\text{MS}}$ scheme at the scale $\mu$. %The Wilson coefficient $C_t$ is known up to the four-loop order %in the SM \cite{Inami:1982xt, Djouadi:1991tk, Chetyrkin:1997iv, Chetyrkin:1997un, Chetyrkin:2005ia, Schroder:2005hy, Baikov:2016tgj}. % % %The squared amplitude for the channels %$g+g\to H+g$, $g+q(\bar{q})\to H+q(\bar{q})$, and %$q+\bar{q}\to H+g$ read~\cite{Ravindran:2002dc}, %\begin{align} % \overline{\sum_{\mathrm{col},\mathrm{pol}} }\big|\mathcal{M}(g+g\to H+g)\big|^2&= \frac{3\lambda_t}{32}\frac{m_H^8+s_{ij}^4+s_{ik}^4+s_{jk}^4}{s_{ij}s_{ik}s_{jk}} \,,\\ % \overline{\sum_{\mathrm{col},\mathrm{pol}} }\big|\mathcal{M}(q(\bar{q})+g\to H+q(\bar{q}))\big|^2&=-\frac{\lambda_t}{24}\frac{s^2_{ij}+s^2_{jk}}{s_{ik}}\,\\ % \overline{\sum_{\mathrm{col},\mathrm{pol}} }\big|\mathcal{M}(q+\bar{q}\to H+g)\big|^2&=\frac{\lambda_t}{9}\frac{s^2_{ik}+s^2_{jk}}{s_{ij}}\,, %\end{align} %with %\begin{align} % s_{ij}=&+2p_i\cdot p_j=\left(k_++\mT e^{-Y_H}\right)\,\left(k_-+\mT e^{+Y_H}\right)\,\\ % s_{ik}=&-2p_i\cdot p_k= -\left(k_++\mT e^{-Y_H}\right)k_- \, \\ % s_{jk}=&-2p_j\cdot p_k= -\left(k_-+\mT e^{+Y_H}\right)k_+ \, \\ %\end{align} %and %\subsection{Asymptotic expansion in the momentum space}\label{sec:asy:mom} \subsection{Prerequisites for the power expansion} \label{sec:setups} \changed{ %Power expansion of the double differential spectrum $ {\done \sigma_H}/{(\done Y_H\, \done \qT^2)}$ mainly concerns the relation of the kinematic variables in the squared amplitudes of Eq.~\eqref{eq:msq}. Therefore, to start with, we introduce % the magnitudes of the light-cone coordinates $\mT e^{\pm Y_H}$ and $k_{\pm}$ in the squared amplitudes of Eq.~\eqref{eq:msq}. Therefore, to facilitate the discussion, it merits recasting Eq.~\eqref{eq:msq} here into a form possessing the manifest dependences on the light-cone momenta. We start the discussion with the transformation on the squared amplitudes in Eq.~\eqref{eq:msq}. As the power expansion in the low \qT\ domain primarily concerns the relation of the kinematic variables $k_{\pm}$ and $\mT e^{\pm Y_H}$, it is beneficial for us to regroup the results in Eq.~\eqref{eq:msq} due to the $k_{\pm}$ and $\mT e^{\pm Y_H}$ dependences. To this end, it merits reminding that the numerators of $|\mathcal{M}|^2$s can be all recast in terms of the polynomials in the invariant scalars $s_{ij}$, $s_{ik}$, and $s_{jk}$, on account of the on-shell condition $ m_H^2\,=\,s_{ij}\,+\,s_{ik}\,+\,s_{jk}$. After bringing in the result in Eq.~\eqref{eq:def:sji} and carrying out the polynomial expansion, the numerators of $|\mathcal{M}|^2$s are then made into a finite series of the products of $k_{\pm}$ and $\mT e^{\pm Y_H}$, more specifically, \begin{equation}\label{eq:qcd:def:H:num} \begin{split} \overline{\sum_{\mathrm{col},\mathrm{pol}}} \big|\mathcal{M}_{[\kappa]}\big|^2 \Bigg|_{\mathrm{Numerator}} \,\rightarrow\, \sum_{\rho,\sigma}\, {(k_+)^{m}}\, {(k_-)^{n} }\, {c}^{m,n}_{[\kappa]} \left(\mT,Y_H\right)\,, \end{split} \end{equation} where the contributing partonic channels are denoted by the subscript $\kappa=\{gg,gq(\bar{q}),q(\bar{q})g,q\bar{q},\bar{q}q\}$. ${c}^{m,n}_{[\kappa]}$ is a function of the hard scales $\mT e^{\pm Y_H}$, with the superscripts $\{m,n\}\ge0$ corresponding to the powers of $k_{\pm}$. Combining Eq.~\eqref{eq:qcd:def:H:num} with the denominators of $|\mathcal{M}|^2$s in Eq.~\eqref{eq:msq} and pulling out a common factor consisting of the coupling parameter $\lambda_t$ and the colliding energy $\sqrt{s}$, it yields that, \begin{equation}\label{eq:qcd:def:H} \begin{split} \overline{\sum_{\mathrm{col},\mathrm{pol}}} \big|\mathcal{M}_{[\kappa]}\big|^2 \,\equiv&\; {16\lambda_t^2\pi s}\, \sum_{\{\beta\}} \sum_{\rho,\sigma}\, \frac{(k_+)^{\sigma}}{(k_++m_\mathrm{T}e^{-Y_H})^{\beta_n-1}}\, \frac{ (k_-)^{\rho} }{(k_-+m_\mathrm{T}e^{Y_H})^{\beta_\nbar-1}}\, \mathcal{H}^{\rho,\sigma}_{[\kappa],\{\beta\}} \left(\mT,Y_H,s\right)\,, \end{split} \end{equation} where a novel hard sector $\mathcal{H}^{\rho,\sigma}_{[\kappa],\{\beta\}}$ is introduced to assimilate ${c}^{\rho,\sigma}_{[\kappa],\{\beta\}}$ in Eq.~\eqref{eq:qcd:def:H:num} and also the colliding energy $\sqrt{s}$. Based on Eq.~\eqref{eq:msq}, the indices $\rho$, $\sigma$ and $\beta_{n,\nbar}$ in $\mathcal{H}^{\rho,\sigma}_{[\kappa],\{\beta\}}$ are always integers for the process $pp\to H+X$ at NLO. At variance with Eq.~\eqref{eq:qcd:def:H:num}, the superscripts $\rho$ and $\sigma$ in Eq.~\eqref{eq:qcd:def:H} can be of negative values, as the squared amplitudes in the $g+g\to H+g$ and $g+q(\bar{q})\to H+q(\bar{q})$ channels are both able to contribute extra light-cone components $k_{\pm}$ from the denominators, thereby lowering the powers of Eq.~\eqref{eq:qcd:def:H:num}. Also, according to Eq.~\eqref{eq:msq}, $\beta_{n,\nbar}$ are always taken greater than or equal to one. At last, it should be emphasized that the parameterization in Eq.~\eqref{eq:qcd:def:H} is not unique, since one can always re-weight the numerator and denominator of the results in Eq.~\eqref{eq:msq} by a common factor, e.g., $(k_-+m_{\mathrm{T}} e^{+Y_H})^2$, and then expand the numerator, without modifying the fraction. This kind of arbitrariness may impact the expressions of individual $\mathcal{H}^{\rho,\sigma}_{[\kappa],\{\beta\}}$s and also the length on the r.h.s of Eq.~\eqref{eq:qcd:def:H}, but will not make any differences on the squared amplitudes $|\mathcal{M}|^2$. } %\changed{ %Analogous transformation is expected to be applicable in the Drell-Yan process at NLO as well~\cite{Gonsalves:1989ar}, but more considerations are still needed when the N$^2$LO ingredients are of one's concern. For instance, in case of the real-virtual corrections of \cite{Gonsalves:1989ar,Schmidt:1997wr}, aside from the rational functions of the scalar products $s_{ij}$, $s_{ik}$, and $s_{jk}$, akin to Eq.~\eqref{eq:msq}, the transcendental ones can also participate into the transition matrix elements, and in turn invoke extra structures in Eq.~\eqref{eq:qcd:def:H}. Those %} \changed{ Substituting Eq.~\eqref{eq:qcd:def:H} together with Eq.~\eqref{eq:qcd:def:Xi} into Eq.~\eqref{eq:qcd:qT}, we recast the \qT~spectrum as, \begin{equation}\label{eq:qcd:qT:kpm} \begin{split} \frac{\done \sigma_H}{\done Y_H\, \done \qT^2} \,=&\; \lambda^2_t\,\sum_{\kappa}\, \sum_{\{\beta\}}\, \sum_{\rho,\sigma } \, \mathcal{H}^{\rho,\sigma}_{[\kappa],\{\beta\}} \left(\mT,Y_H,s\right) \, \\ &\times\; \int^{k_+^{\mathrm{max}}}_{k_+^{\mathrm{min}}} \frac{\done k_+}{k_+}\; (k_-)^{\rho} \, (k_+)^{\sigma} \, {F}^{(0)}_{i/n,\beta_n}\left(k_++\mT e^{-Y_H}\right)\, {F}^{(0)}_{j/\nbar,\beta_\nbar}\left( k_-+\mT e^{+Y_H} \right)\,. \end{split} \end{equation} Herein, the integrand} contains the derivatives of the scaled PDFs of the light-cone components $(k_{\pm}+\mT e^{\mp Y_H})$, generically defined as \begin{align}\label{eq:def:FioN:FjoNbar} {F}^{(\alpha_n)}_{i/n,\beta_n}\left(Q_n\right) &\equiv \frac{\partial^{\alpha_n}}{\partial Q_n^{\alpha_n}} \left[ \frac{f_{i/n}\left({Q_n}/{\sqrt{s}}\right)}{Q_n^{\beta_n}} \right]\,, \quad\quad {F}^{(\alpha_\nbar)}_{j/\nbar,\beta_\nbar}\left(Q_\nbar\right) \equiv \frac{\partial^{\alpha_\nbar}}{\partial Q_\nbar^{\alpha_\nbar}} \left[ \frac{f_{j/\nbar}\left(Q_\nbar/{\sqrt{s}}\right)} {Q_\nbar^{\beta_\nbar}} \right]\,, \end{align} where ${Q}_{n}$ and $Q_\nbar$ represent the two kinematic variables, $\alpha_n$ and $\alpha_\nbar$ determine the rank of the derivative, and $\beta_n$ and $\beta_\nbar$ are the powers to which they scale their respective PDFs. Collectively, we denote the latter $\{\alpha\}$ and $\{\beta\}$. For the results derived in full QCD, see Eq.~\eqref{eq:qcd:qT}, only the zero-rank scaled PDFs are involved. Hence, only the $\alpha_n=\alpha_\nbar=0$ case is present in Eq.~\eqref{eq:qcd:qT:kpm}. The $\alpha_n,\alpha_\nbar>0$ expressions, however, will enter in the higher-power \qT\ expansion. In the following, we will concern ourselves with the analytic properties of the functions ${F}^{(\alpha_n)}_{i/n,\beta_n}\left(Q_n\right)$ and ${F}^{(\alpha_\nbar)}_{j/\nbar,\beta_\nbar}\left(Q_\nbar\right)$. However, due to the fact that the PDFs $f_{i/n}$ and $f_{j/\nbar}$ have their origin in the non-perturbative regime of QCD and, thus, their analytic expressions are not fully established, we make the following assumptions: \begin{enumerate} \item[(a)] For a given $\alpha_n,\alpha_\nbar>0$ the ${F}^{(\alpha_n)}_{i/n,\beta_n}\left(Q_n \right)$ and ${F}^{(\alpha_\nbar)}_{j/\nbar,\beta_\nbar}\left(Q_\nbar\right)$, as well as their arbitrary order derivatives, exist and are bounded over the domain $\Lambda_{\mathrm{H}}\le{Q}_{n(\nbar)}\le\sqrt{s}$ for all $\beta_n$ and $\beta_\nbar$, where $\Lambda_{\mathrm{H}}$ represent a hadronisation scale\;. \item[(b)] ${F}^{(\alpha_n)}_{i/n,\beta_n}\left(Q_n+\delta Q_n\right)$ and ${F}^{(\alpha_\nbar)}_{j/\nbar,\beta_\nbar}\left(Q_\nbar+\delta Q_\nbar\right)$ have convergence radii $|\delta{Q}_{n(\nbar)}|<{Q}_{n(\nbar)}$ as long as $\left({Q}_{n(\nbar)} + \delta{Q}_{n(\nbar)}\right)$ and ${Q}_{n(\nbar)}$ are both well within the interval $\left[\Lambda_{\mathrm{H}},\sqrt{s}\right]$\,. \end{enumerate} Please note, if the PDFs are fitted in a basis of Chebyshev polynomials, as proposed in \cite{Bonvini:2012sh,Bonvini:2014joa,Diehl:2021gvs}, and thereby $f_{i/n}$ and $f_{j/\nbar}$ can be then expressed in terms of $\ln^k(\xi_n)/\xi_n^h$ and $\ln^k(\xi_\nbar)/\xi_\nbar^h$, respectively, the second assumption is immediately fulfilled. Equipped with the above ansatz, we are able to expand Eq.~\eqref{eq:qcd:qT:kpm} in the vicinity of $\qT=0$. To this end, we start with the expansion of the kinematic variable $\mT $ in the hard coefficient function $\mathcal{H}^{\rho,\sigma}_{[\kappa],\{\beta\}}$. In the small \qT~domain where $\qT\ll m_H$, we can perform an expansion of the transverse mass \mT\ of the Higgs boson around its invariant mass $m_H$, \begin{align}\label{eq:asy:mom:mT} \mT \,=\, m_H\,\cdot\, \sum_{h=0}^{\infty}\,\frac{1}{h!}\, \frac{\Gamma[\tfrac{3}{2}]}{\Gamma[\frac{3}{2}-h]}\, \left(\frac{\qT^2}{m_H^2}\right)^h\,. \end{align} We can use this result to expand the hard coefficient $\mathcal{H}^{\rho,\sigma}_{[\kappa],\{\beta\}}$ around $\qT=0$, giving \begin{equation}\label{eq:asy:mom:c} \begin{split} \mathcal{H}_{[\kappa],\{\beta\}}^{\rho,\sigma}&(\mT,Y_H,s)\\ =&\, \sum_{h=0}^{\infty}\frac{(\mT-m_H)^h}{h!}\, \left\{ \frac{\partial^h}{\partial \mT^h}\, \mathcal{H}_{[\kappa],\{\beta\}}^{\rho,\sigma}(\mT,Y_H,s) \bigg|_{\mT\to m_H} \right\}\, \\ =&\, \sum_{h,l=0}^{\infty}\,\sum_{g=0}^h\,\frac{(-1)^{h-g}}{g!\,l!\,(h-g)!}\, \frac{\Gamma[\frac{g}{2}+1]}{\Gamma[\frac{g}{2}-l+1]}\, \left(\frac{\qT^2}{m^2_H}\right)^l\,m_H^h\, \mathcal{H}_{[\kappa],\{\beta\}}^{(h),\rho,\sigma}(m_H,Y_H,s)\,, \end{split} \end{equation} where we have introduced $\mathcal{H}_{[\kappa],\{\beta\}}^{(h),\rho,\sigma}(m_H,Y_H,s) \equiv\frac{\partial^h}{\partial \mT^h}\,\mathcal{H}_{[\kappa],\{\beta\}}^{\rho,\sigma}(\mT,Y_H,s)\bigg|_{\mT\to m_H}$. An analogous expansion can also be applied to the derivatives of the scaled PDFs ${F}^{(\alpha_n)}_{i/n,\beta_n}$ and ${F}^{(\alpha_\nbar)}_{j/\nbar,\beta_\nbar}$. To this end, we re-express their arguments below in order to isolate all \qT~dependences, \begin{align}\label{eq:asy:mom:pdfs:arg} k_{\pm}+\mT e^{\mp Y_H} \to \left[k_{\pm}+m_He^{\mp Y_H}\right] +\left(\mT -m_H\right)\,e^{\mp Y_H}. \end{align} In proximity to $\qT=0$, the second term on the right handed side (r.h.s) is always smaller in magnitude with respect to the first one. Therefore, we can expand ${F}^{(\alpha_n)}_{i/n,\beta_n}(k_{+}+\mT e^{- Y_H})$ and ${F}^{(\alpha_\nbar)}_{j/\nbar,\beta_\nbar}(k_{-}+\mT e^{+ Y_H})$ around $(k_{+}+m_He^{- Y_H})$ and $(k_{-}+m_He^{+ Y_H})$, respectively, \begin{equation}\label{eq:asy:mom:pdfs} \begin{split} F^{(0)}_{i/n,\beta_n}&\left(k_{+}+\mT e^{- Y_H}\right)\\ &=\, \sum_{h=0}^{\infty}\,\frac{(\mT-m_H)^h}{h!}\,(e^{-Y_H})^h\, F^{(h)}_{i/n,\beta_n}\left(k_{+}+m_He^{- Y_H}\right)\\ &=\, \sum_{h,l=0}^{\infty}\sum_{g=0}^h\, \frac{(-1)^{h-g} }{g! \,l! \,(h-g)!}\, \frac{\Gamma[\frac{g}{2}+1]}{\Gamma[\frac{g}{2}-l+1]}\, \left(\frac{\qT^2}{m^2_H}\right)^l\, \left( m_H e^{-Y_H} \right)^h\, F^{(h)}_{i/n,\beta_n}\left(k_{+}+m_He^{- Y_H}\right)\,,\\ F^{(0)}_{j/\nbar,\beta_\nbar}&\left(k_{-}+\mT e^{+Y_H}\right)\\ &=\, \sum_{h=0}^{\infty}\,\frac{(\mT-m_H)^h}{h!}\,(e^{+Y_H})^h\, F^{(h)}_{j/\nbar,\beta_\nbar}\left(k_{-}+m_He^{+Y_H}\right)\\ &=\, \sum_{h,l=0}^{\infty}\sum_{g=0}^h\, \frac{(-1)^{h-g} }{g! \,l! \,(h-g)!}\, \frac{\Gamma[\frac{g}{2}+1]}{\Gamma[\frac{g}{2}-l+1]}\, \left(\frac{\qT^2}{m^2_H}\right)^l\, \left( m_H e^{+Y_H} \right)^h\, F^{(h)}_{j/\nbar,\beta_\nbar}\left(k_{-}+m_He^{+Y_H}\right)\,. \end{split} \end{equation} Inserting the expressions of Eqs.~\eqref{eq:asy:mom:c}-\eqref{eq:asy:mom:pdfs} into Eq.~\eqref{eq:qcd:qT:kpm}, the \qT~spectrum now takes the following form, \begin{align}\label{eq:qcd:qT:kpm:exp1} &\frac{\done \sigma_H}{\done Y_H\, \done \qT^2} \,=\, \lambda_t^2\, \sum_{\omega}\, \left({\qT^2}\right)^{\omega}\, \sum_{[\kappa]}\, \sum_{\{\alpha,\beta\}}\,\sum_{\rho,\sigma }\, \widetilde{\mathcal{H}}^{(\omega ),\rho,\sigma}_{[\kappa],\{\alpha,\beta\}} \left(m_H,Y_H,s\right) \, \bigg\{ \widetilde{\mathcal{I}}^{ \rho,\sigma}_{[\kappa],\{\alpha,\beta\}} \,+\, \Delta\widetilde{\mathcal{I}}^{ \rho,\sigma}_{[\kappa],\{\alpha,\beta\}} \bigg\}\;. \end{align} Therein, $\widetilde{\mathcal{H}}^{(\omega),\rho,\sigma }_{[\kappa],\{\alpha,\beta\}}$ is introduced to absorb the factorials, gamma functions, as well as powers of the hard scales $m_H$ and $\sqrt{s}$ emerging from Eqs.~\eqref{eq:asy:mom:c}-\eqref{eq:asy:mom:pdfs}, \begin{equation}\label{eq:qcd:defHtilde} \begin{split} \widetilde{\mathcal{H}}^{(\omega),\rho,\sigma }_{[\kappa],\{\alpha,\beta\}} \,=&\; \left(\frac{1}{m^2_H}\right)^{\omega}\, \sum_{l_n=0}^{\omega}\, \sum_{l_\nbar=0}^{\omega-l_n}\, \sum_{\alpha_h=0}^{\infty}\, \prod_{x=\{h,n,\nbar\}} \left\{ \sum_{g_x=0}^{\alpha_x}\frac{(-1)^{\alpha_x-g_x} }{g_x! \,l_x! \,(\alpha_x-g_x)!}\, \frac{\Gamma[\frac{g_x}{2}+1]}{\Gamma[\frac{g_x}{2}-l_x+1]}\, \right\}\\ &\times \left( m_H e^{-Y_H} \right)^{\alpha_n}\, \left( m_H e^{+Y_H} \right)^{\alpha_\nbar}\, \left( m_H \right)^{\alpha_h}\, {\mathcal{H}}^{ (\alpha_h),\rho,\sigma }_{[\kappa],\{\beta\}}\,, \end{split} \end{equation} where $l_h=\omega-l_n-l_\nbar\ge0$. The \qT~dependences have been factored out from $\widetilde{\mathcal{H}}^{(\omega ),\rho,\sigma}_{[\kappa],\{\alpha,\beta\}}$ and the arguments of ${F}^{(\alpha_n)}_{i/n,\beta_n}$ and ${F}^{(\alpha_\nbar)}_{j/\nbar,\beta_\nbar}$. The remaining ones participate through boundary conditions as defined in Eq.~\eqref{eq:def:b.c.}. To address them as well, we divide the phase space integral of Eq.~\eqref{eq:qcd:qT:kpm:exp1} into two sectors, $\widetilde{\mathcal{I}}^{ \rho,\sigma}_{[\kappa],\{\alpha,\beta\}}$ and $\Delta\widetilde{\mathcal{I}}^{ \rho,\sigma}_{[\kappa],\{\alpha,\beta\}}$, with \begin{align} \label{eq:def:I:central} \widetilde{\mathcal{I}}^{ \rho,\sigma}_{[\kappa],\{\alpha,\beta\}} =&\, \int^{\tilde{k}^{\mathrm{max}}_+}_{\tilde{k}^{\mathrm{min}}_+}\, \frac{\done k_+}{k_+} (k_-)^{\rho} \, (k_+)^{\sigma} \, {F}^{(\alpha_n)}_{i/n,\beta_n}\left(k_++m_He^{-Y_H}\right)\, {F}^{(\alpha_\nbar)}_{j/\nbar,\beta_\nbar}\left(k_-+m_He^{+Y_H} \right)\,,\\ \label{eq:def:I:boundary} \Delta\widetilde{\mathcal{I}}^{ \rho,\sigma}_{[\kappa],\{\alpha,\beta\}} =&\, \left( \int_{\tilde{k}^{\mathrm{max}}_+}^{{k}^{\mathrm{max}}_+}\!\!\!\! +\int^{\tilde{k}^{\mathrm{min}}_+}_{{k}^{\mathrm{min}}_+} \right) \frac{\done k_+}{k_+} (k_-)^{\rho} \, (k_+)^{\sigma} \, {F}^{(\alpha_n)}_{i/n,\beta_n}\!\!\left(k_++m_He^{-Y_H}\right) {F}^{(\alpha_\nbar)}_{j/\nbar,\beta_\nbar}\!\!\left(k_-+m_He^{+Y_H} \right)\,,\!\!\!\!\!\! \end{align} by means of the following boundaries, \begin{align} \tilde{k}_+^{\mathrm{max}} = \sqrt{s}-m_H e^{-Y_H}\,,\quad\quad\tilde{k}_+^{\mathrm{min}} = {\qT^2}/(\sqrt{s}-m_H e^{+Y_H}) \,. \end{align} Consequently, $\Delta\widetilde{\mathcal{I}}^{ \rho,\sigma}_{[\kappa],\{\alpha,\beta\}}$ contains all $\mT$ dependences. In analysing the scaling behaviour, we find that within the central region $e^{\pm Y_H}\sim\mathcal{O}(1)$, the integration variables $k_{\pm}$ exhibit unambiguous scaling in each integration region. Therefore, as will be illustrated in~Sec.~\ref{sec:red:qT:boundary}, the power expansion of $\Delta\widetilde{\mathcal{I}}^{ \rho,\sigma}_{[\kappa],\{\alpha,\beta\}}$ follows an analogous pattern to those in Eqs.~\eqref{eq:asy:mom:c}-\eqref{eq:asy:mom:pdfs}. Nevertheless, $\widetilde{\mathcal{I}}^{ \rho,\sigma}_{[\kappa],\{\alpha,\beta\}}$ behaves differently. From its expression in Eq.~\eqref{eq:def:I:central}, a number of different scales have been enclosed in the integration range of $\widetilde{\mathcal{I}}^{ \rho,\sigma}_{[\kappa],\{\alpha,\beta\}}$, starting from the ultrasoft scale ${k^{\mathrm{min}}_+}\sim\mathcal{O}(\qT^2/m_H)$, through the soft one $k_{\pm}\sim\mathcal{O}(\qT)$, and ending up with the hard scale ${k^{\mathrm{max}}_+}\sim\mathcal{O}(m_H)$. They all correspond to a distinct way of expanding the integrands. To this end, in Sec.~\ref{sec:red:qT:central}, we will make use of a set of momentum cutoffs to unambiguously treat them. % % , ranging from ${k^{\mathrm{max}}_+}\sim\mathcal{O}(m_H)$ down to ${k^{\mathrm{min}}_+}\sim\mathcal{O}(\qT^2/m_H)$ % %he latter case concerns the contributions neighbouring the boundaries, % % %In comparison with eq.~\eqref{eq:qcd:qT:kpm}, all the \qT~dependences have been factored out from the transverse mass $\mT $ in the hard coefficient as well as the fraction functions ${F}^{ (\omega)}_{i/n,\beta} $ and ${F}^{ (\omega)}_{j/\nbar,\alpha} $, such that the reduced arguments $m_H e^{\pm Y_H}$ both observe uniform scaling $\sim\mathcal{O}(1)$. %Nevertheless, the asymptotic series in eq.~\eqref{eq:qcd:qT:kpm:exp1} is still not homogeneous in $\qT$ yet on the grounds that $\mT $ participates into the boundary conditions as defined in eq.~\eqref{eq:def:b.c.} and also that the phase space integral a variety of scales ranging from ${k^{\mathrm{max}}_+}\sim\mathcal{O}(1)$ down to ${k^{\mathrm{min}}_+}\sim\mathcal{O}(\qT^2/m_H)$. %To this end, $ \Delta\widetilde{\mathcal{I}}^{ \rho,\sigma }_{[\kappa], \{\alpha,\beta\} }$ encompasses all the remaining $\mT$ dependences. % % % %According to eq.~\eqref{eq:def:I:boundary}, the integration variable $k_+$ always observes unambiguous scaling in each interval of $ \Delta\widetilde{\mathcal{I}}^{ \rho,\sigma }_{[\kappa], \{\alpha,\beta\} }$ and thus, as will be elaborated in~Sec.~\ref{sec:red:qT:boundary}, the expansion of $ \Delta\widetilde{\mathcal{I}}^{ \rho,\sigma }_{[\kappa], \{\alpha,\beta\} }$ bears a resemblance to those in eqs.~(\ref{eq:asy:mom:c}-\ref{eq:asy:mom:pdfs}). % % % On the other hand, $\widetilde{\mathcal{I}}^{ \rho,\sigma }_{[\kappa], \{\alpha,\beta\} }$ defined in eq.~\eqref{eq:def:I:central} carries the bulk of the phase space. Since the variable $k_+$ therein endures varying magnitude across the domain of integration, in Sec.~\ref{sec:red:qT:central}, we will perform the expansion by introducing a group of dynamic regions. \subsection{Power corrections on the boundary}\label{sec:red:qT:boundary} We have mentioned above that besides the integrand itself, the integration boundaries are other sources for power corrections. In the following, we will thus expand the integral $\Delta\widetilde{\mathcal{I}}^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\}}$ within the central region $e^{\pm Y_H}\sim \mathcal{O}(1)$. As illustrated in Eq.~\eqref{eq:def:I:boundary}, $\Delta\widetilde{\mathcal{I}}^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\}}$ consists of the integral of $k_+$ over two intervals, ${k}_+ \in[\tilde{k}_+^{\mathrm{max}}, {k}_+^{\mathrm{max}}]$ and ${k}_+ \in[ {k}_+^{\mathrm{min}}, \tilde{k}_+^{\mathrm{min}}]$. In each of them, the momentum $k^{\mu}$ of the emitted particle is subject to an unambiguous scaling, \begin{align} \label{eq:def:kc:boundary} {k}_+ \in[\tilde{k}_+^{\mathrm{max}}, {k}_+^{\mathrm{max}}]\;:\quad k_+\sim \mathcal{O}(m_H)\,,\quad k_-\sim \mathcal{O}(\qT^2/m_H)\,, \quad \kTvec=-\qTvec\,,\\ \label{eq:def:kcbar:boundary} {k}_+ \in[ {k}_+^{\mathrm{min}}, \tilde{k}_+^{\mathrm{min}}]\;:\quad k_+\sim \mathcal{O}(\qT^2/m_H)\,,\quad k_-\sim \mathcal{O}(m_H)\,, \quad \kTvec=-\qTvec\,, \end{align} where the transverse recoil $\kTvec$ is determined by the momentum conservation. Considering that the momenta $k_{\pm}$ in Eqs.~\eqref{eq:def:kc:boundary}-\eqref{eq:def:kcbar:boundary} are nearly corresponding to the hardest emission along the beam direction that are kinematically allowed (in a logarithmic sense), henceforth, we dub them the $n$-ultra-collinear and $\nbar$-ultra-collinear modes, respectively. In the following, we will make use of those two scaling laws to expand $\Delta\widetilde{\mathcal{I}}^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\}}$ within the low \qT~regime. We first consider the $n$-ultra-collinear contribution, applying Eq.~\eqref{eq:def:kc:boundary} to Eq.~\eqref{eq:def:I:boundary} yields \begin{equation} \label{eq:asyexp:deltaI:uc} \begin{split} \Delta \widetilde{\mathcal{I}}^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\}}\Bigg|_{uc} \,=\,& \int_{\tilde{k}^{\mathrm{max}}_+}^{ {k}^{\mathrm{max}}_+}\, \frac{\done k_+}{k_+}\, (k_-)^{\rho} \, (k_+)^{\sigma} \, {F}^{(\alpha_n)}_{i/n,\beta_n}\left(k_++m_He^{-Y_H}\right)\, {F}^{(\alpha_\nbar)}_{j/\nbar,\beta_\nbar}\left( k_-+m_He^{+Y_H} \right)\\ =\,& (\qT^2)^{\rho}\, \int_{0}^{ (m_H-\mT)e^{-Y_H}}\, \done\hat{k}_+\, (\hat{k}_+ + \tilde{k}^{\mathrm{max}}_+)^{\sigma-\rho-1} \\ &\hspace*{20mm}\times\, {F}^{(\alpha_n)}_{i/n,\beta_n}\left(\hat{k}_++\sqrt{s}\right)\, {F}^{(\alpha_\nbar)}_{j/\nbar,\beta_\nbar} \left( \frac{\qT^2}{\hat{k}_+ +\tilde{k}^{\mathrm{max}}_+}+ m_He^{+Y_H} \right)\\ =\,& \sum_{\tilde{\alpha}_n,\tilde{\alpha}_\nbar=0}^{\infty}\, \frac{(\qT^2)^{\rho+\tilde{\alpha}_\nbar}}{\tilde{\alpha}_n!\,\tilde{\alpha}_\nbar!} \, {F}^{(\alpha_n+\tilde{\alpha}_n)}_{i/n,\beta_n}\left(\sqrt{s}\right)\, {F}^{(\alpha_\nbar+\tilde{\alpha}_\nbar)}_{j/\nbar,\beta_\nbar}\left( m_He^{+Y_H} \right)\, \mathcal{B}^{\rho,\sigma}_{+,\{\alpha,\beta\}} \,, \end{split} \end{equation} where in the second step the integration variable is transformed such that the power suppressed residual terms can be extracted, i.e.\ \begin{equation}\label{eq:trans:kp} k_+ \,\to\, \underbrace{\quad\hat{k}_+\quad}_{\sim\mathcal{O}(\qT^2/m_H)} \,+\, \underbrace{\quad\tilde{k}_+^{\mathrm{max}}\quad}_{\sim\mathcal{O}(m_H)}\,. \end{equation} Based on this scaling behaviour, the functions ${F}^{(\alpha_n)}_{i/n,\beta_n}$ and ${F}^{(\alpha_\nbar)}_{j/\nbar,\beta_\nbar}$ can be expanded around $\sqrt{s}$ and $m_He^{+Y_H}$, respectively, in the last step of Eq.~\eqref{eq:asyexp:deltaI:uc}, thereby removed from the $\hat{k}_+$-integral. The remaining $\hat{k}_+$ dependences are collected in the function $\mathcal{B}^{\rho,\sigma}_{+,\{\alpha,\beta\}}$, defined through \begin{equation}\label{eq:def:Gp} \begin{split} \mathcal{B}^{\rho,\sigma}_{+,\{\alpha,\beta\}} \equiv&\; \int_{0}^{ (m_H-\mT)e^{-Y_H}}\done\hat{k}_+\; (\hat{k}_+ + \tilde{k}^{\mathrm{max}}_+)^{\sigma-\rho-\tilde{\alpha}_\nbar-1} (\hat{k}_+)^{\tilde{\alpha}_n}\\ =&\; \int_{0}^{ (m_H-\mT)e^{-Y_H}}\done\hat{k}_+\; (\hat{k}_+)^{\tilde{\alpha}_n}\, \left(\tilde{k}^{\mathrm{max}}_+\right)^{\sigma-\rho-\tilde{\alpha}_\nbar-1} \\ &\hspace*{10mm}\times \Bigg\{ \theta(\sigma-\rho-\tilde{\alpha}_\nbar-1)\, \sum_{\gamma=0}^{\sigma-\rho-\tilde{\alpha}_\nbar-1}\, \frac{1}{\gamma!}\, \left(\frac{\hat{k}_+}{\tilde{k}^{\mathrm{max}}_+}\right)^{\gamma}\, \frac{\Gamma[\sigma-\rho-\tilde{\alpha}_\nbar]} {\Gamma[\sigma-\rho-\tilde{\alpha}_\nbar-\gamma]}\\ &\hspace*{17mm}{}+\, \bar{\theta}(\sigma-\rho-\tilde{\alpha}_\nbar-1)\, \sum_{\gamma=0}^{\infty}\, \frac{(-1)^{\gamma}}{\gamma!}\, \frac{\Gamma[\gamma-\sigma+\rho+\tilde{\alpha}_\nbar+1]}{\Gamma[-\sigma+\rho+\tilde{\alpha}_\nbar+1]}\, \left(\frac{\hat{k}_+}{\tilde{k}^{\mathrm{max}}_+}\right)^{\gamma}\, \Bigg\} \,. \end{split} \end{equation} Herein, we use the Heaviside theta function $\theta(x)$, with $\theta(x)=1$ for $x\ge0$ and $0$ otherwise, and its counter part $\bar{\theta}(x)\equiv1-\theta(x)$ to account for the expansion of the integrand. Even though within the central rapidity region $e^{\pm Y_H}\sim\mathcal{O}(1)$ and thus $\tilde{k}^{\mathrm{max}}_+\sim\mathcal{O}(m_He^{\pm Y_H}) $, the integrand of Eq.~\eqref{eq:def:Gp} has already admitted a formally asymptotic series in $({\hat{k}_+}/{\tilde{k}^{\mathrm{max}}_+})$, the participation of $\mT$ into the upper boundary condition can invoke inhomogeneous behaviour after completing the phase space integral. To this end, a further expansion is necessary with the aid of Eq.~\eqref{eq:asy:mom:mT}. It follows that \begin{equation} \begin{split} \label{eq:asyexp:deltaI:ec:int} \int_{0}^{(m_H-\mT)e^{-Y_H}}\,\done\hat{k}_+\, \hat{k}_+^{\tilde{\alpha}_n+\gamma}\, =&\, \sum_{\gamma_2=0}^{\infty}\, \sum_{\gamma_1=0}^{1+\gamma+\tilde{\alpha}_n}\, \frac{(-1)^{\gamma_1}}{\gamma_1!\,\gamma_2!}\, \left(\frac{\qT^2}{m_H^2}\right)^{\gamma_2}\,(e^{-Y_H}m_H)^{1+\tilde{\alpha}_n+\gamma }\\ &\hspace*{20mm}\times\, \frac{\Gamma[1+\tfrac{\gamma_1}{2}]} {\Gamma[1-\gamma_2+\tfrac{\gamma_1}{2}]}\, \frac{\Gamma[\tilde{\alpha}_n+\gamma+1]} {\Gamma[\tilde{\alpha}_n+\gamma-\gamma_1+2]}\,. \end{split} \end{equation} Combining Eqs.~\eqref{eq:def:Gp}-\eqref{eq:asyexp:deltaI:ec:int} with Eq.~\eqref{eq:asyexp:deltaI:uc}, we then accomplish the expansion of the $n$-ultra-collinear sector in the small parameter $(\qT/m_H)$. An analogous procedure can be similarly applied onto the $\nbar$-ultra-collinear case, with the exception of the conversion of the integration variable $k_+$ to $k_-$ by means of the on-shell condition $k_+k_-=\qT^2$ and the substitution of $e^{+Y_H}$ for $e^{-Y_H}$ in Eq.~\eqref{eq:asyexp:deltaI:ec:int}, as appropriate. From those results, we observe that the boundary corrections here are always associated with PDFs at the opposite end and therefore are a priori expected to play an negligible role in comparison to $\widetilde{\mathcal{I}}^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\}}$ in Eq.\ \eqref{eq:def:I:central}. While this is expected to hold for the first few terms in the power expansion, it is possible that the higher power corrections from $\widetilde{\mathcal{I}}^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\}}$ become of a similar size as the boundary corrections from $\Delta\widetilde{\mathcal{I}}^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\}}$, such that both parts of contributions are essential to reproduce the desired asymptotic behaviour of the \qT~spectrum. In Sec.~\ref{sec:asyexp:numeric}, we will deliver a quantitative assessment thereof. \subsection{Power corrections over the interior domain} \label{sec:red:qT:central} \subsubsection{Asymptotic expansion in momentum space} \label{sec:asyexp:qT:mom} We can now perform the power expansion on the integral $\widetilde{\mathcal{I}}^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\}}$ in the low $\qT$~area within the central rapidity region $e^{\pm Y_H}\sim \mathcal{O}(1)$. As exhibited in Eq.~\eqref{eq:def:I:central}, $\widetilde{\mathcal{I}}^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\}}$ encompasses a variety of scales along the integration path, including the ultra-soft scale $k_+\sim \mathcal{O}(\qT^2/m_H)$, the soft one $k_+\sim \mathcal{O}(\qT)$, and the hard one $k_+\sim\mathcal{O}(m_H)$. Every one of those momentum modes in practice prompts a distinct expansion of $\widetilde{\mathcal{I}}^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\} }$. Hence, in the spirit of the expansion by regions method \cite{Beneke:1997zp,Smirnov:1998vk,Smirnov:1999bza, Smirnov:2002pj,Jantzen:2011nz} and also according to the pattern of the resulting power series, we categorise the phase space as follows~\footnote{% It is interesting to note that the analogous strategy in refining the dynamic regions has also been utilised previously in the literature~\cite{Balitsky:2009xg,Balitsky:2013fea, Balitsky:2017flc,Balitsky:2019ayf,Balitsky:2022vnb,Balitsky:2023hmh} in probing the $k_{\mathrm{T}}$ factorisation in the small-$x$ area.}, \begin{equation}\label{eq:def:col-n:soft:col-nbar:cutoff} \begin{split} n\text{-collinear~mode}:\;\; \;& \nu_n<k_+\le \tilde{k}^{\mathrm{max}}_+;\,\vphantom{\frac{\qT^2}{\nu_{\nbar}}}\\ \text{transitional range}:\;\; \;& \frac{\qT^2}{\nu_{\nbar}}<k_+\le \nu_n;\,\\ \nbar\text{-collinear~mode}:\;\; \;& \tilde{k}^{\mathrm{min}}_+\le k_+\le \frac{\qT^2}{\nu_{\nbar}} \; . \end{split} \end{equation} Here, a pair of auxiliary scales $\{\nu_{n},\nu_{\nbar}\}$ are introduced to separate the $n$- and $\nbar$-collinear regions from the moderate range in between. Throughout this paper, $\{\nu_{n},\nu_{\nbar}\}$ are chosen to be of similar magnitudes to the hard scales $m_H e^{ \pm Y_H}$ but always small enough that in the intermediate domain of Eq.~\eqref{eq:def:col-n:soft:col-nbar:cutoff} the light-cone components $k_+$ and $k_-$ are both well contained within the convergence radii of ${F}^{(\alpha_n)}_{i/n,\beta_n}$ and ${F}^{(\alpha_\nbar)}_{j/\nbar,\beta_\nbar}$, as stipulated in Sec.~\ref{sec:setups}, more specifically, \begin{align}\label{eq:def:scaling:nun:nunbar} m_H e^{-Y_H}\gtrsim\nu_n\sim \mathcal{O}(m_H)\gg\qT\,, \quad\quad m_H e^{Y_H}\gtrsim\nu_{\nbar}\sim \mathcal{O}(m_H)\gg\qT\,. \end{align} Alternative choices of those two auxiliary boundaries can be used to examine the asymptotic behaviour of $\widetilde{\mathcal{I}}^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\}}$. For example, the scales proposed in~\cite{Balitsky:2023hmh} may impact the expressions of the individual sectors defined in Eq.~\eqref{eq:def:col-n:soft:col-nbar:cutoff} but will leave the resulting power series unchanged upon summation of all ingredients. Having chosen $\{\nu_{n},\nu_{\nbar}\}$ according to Eq.~\eqref{eq:def:scaling:nun:nunbar}, the momentum $k^{\mu}$ obeys the unambiguous scaling law $k_+\sim\mathcal{O}(m_H)\gg k_-\sim \mathcal{O}(\qT^2/m_H)$ in the $n$-collinear mode, from which we can expand ${F}^{(\alpha_\nbar)}_{j/\nbar,\beta_\nbar}$ around the intrinsic scale $m_H e^{+Y_H}$, \begin{align}\label{eq:def:asyexp:c:mom} \widetilde{\mathcal{I}}^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\} }\Bigg|_{c}\, =\, \sum_{\omega=\rho}^{\infty}\,(\qT^2)^{\omega}\, \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}} \Bigg|_{c} \,, \end{align} where \begin{align}\label{eq:def:asyexp:c:mom:at:omega} \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}} \Bigg|_{c} \, \equiv\, \int^{\tilde{k}^{\mathrm{max}}_+}_{\nu_n}\, \frac{\done k_+}{k_+}\, \frac{(k_+)^{\sigma-\omega}}{(\omega-\rho)!} \, {F}^{(\alpha_n)}_{i/n,\beta_n}\left(k_++m_H e^{-Y_H}\right)\, {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)\,. \end{align} Here, all $\qT$ dependences have been extracted into the prefactor of Eq.~\eqref{eq:def:asyexp:c:mom} to express the manifest power accuracy of the contribution. $\widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}$ collects all hard scales and thus is always of $\mathcal{O}(1)$. It merits noting that in the central rapidity region $e^{\pm Y_H}\sim\mathcal{O}(1)$, the lower boundary $\nu_n$ in Eq.~\eqref{eq:def:asyexp:c:mom:at:omega} is well separated from the upper one and thus there is no need to utilise a further expansion here, in contrast to Eq.~\eqref{eq:asyexp:deltaI:uc}. The same method can also be applied to the $\nbar$-collinear mode, after transforming the integration variable from $k_+$ to $k_-$ through the on-shell condition $k_+ k_-=\qT^2$. It evaluates to, \begin{align}\label{eq:def:asyexp:cbar:mom} \widetilde{\mathcal{I}}^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\}} \Bigg|_{\bar{c}}\, =\, \sum_{\omega=\sigma}^{\infty}\,(\qT^2)^{\omega}\, \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}} \Bigg|_{\bar{c}}\,, \end{align} with \begin{align}\label{eq:def:asyexp:cbar:mom:at:omega} \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}} \Bigg|_{\bar{c}}\, \equiv\, \int^{\frac{\qT^2}{\tilde{k}^{\mathrm{min}}_+}}_{\nu_{\nbar}}\, \frac{\done k_-}{k_-}\, \frac{(k_-)^{\rho-\omega}}{(\omega-\sigma)!} \, {F}^{(\alpha_n+\omega-\sigma)}_{i/n,\beta_n}\left(m_H e^{-Y_H}\right)\, {F}^{(\alpha_\nbar)}_{j/\nbar,\beta_\nbar}\left(k_-+m_H e^{+Y_H}\right)\,. \end{align} %{eq:def:asyexp:c:mom}{eq:def:asyexp:cbar:mom:at:omega} %where $\widetilde{I}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }$ encode the corrections at the $\omega$-th power. %During the derivation, the on-shell condition $k_-k_+=\qT^2$ has been applied to convert the component $k_-$ to $k_+$. %The functions ${F}_{i/n}$ and $ {F}_{j/\nbar}$ are employed to collect the ensuing PDFs and the denominators $(k_{\mp}+m_H e^{\pm Y_H})^{\kappa}$, more specifically, %\begin{align} %{F}^{\{\beta \},(\omega)}_{i/n}\left(Q_n\right)&\equiv\frac{\partial^{\omega}}{\partial (Q_n)^{\omega}}\left[\frac{f^{(\alpha_n)}_{i/{N}}\left({ Q_n}/{\sqrt{s}}\right)}{ (Q_n)^{\beta_n}}\right]\,, % \quad\quad %{F}^{\{\alpha\},(\omega)}_{j/\nbar}\left( Q_\nbar\right)\equiv\frac{\partial^{\omega}}{\partial (Q_\nbar)^{\omega}}\left[\frac{f^{(\alpha_\nbar)}_{j/{\bar{N}}}\left( Q_\nbar/{\sqrt{s}}\right)}{ (Q_\nbar)^{\beta_\nbar}}\right]\,. %\end{align} %It is worth noting that in eq.~\eqref{eq:def:asyexp:c:mom}, since the cutoff parameter $\nu_n$ is chosen to be of the hard scale, i.e., $m_H e^{-Y_H}\gtrsim\nu_n\sim \mathcal{O}(\lambda^0_{\mathrm{T}})$, the integration in $\widetilde{I}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }$ does not come across any soft scale such as $\qT$ along the integration path, and its power precision is thus entirely governed by the prefactor $(\qT^2)^{\omega}$. This is also in agreement with the result estimated through the collinear scaling $k^{\mu}\sim m_H [\mathcal{O}(\lambda_{\mathrm{T}}^2),\mathcal{O}(\lambda_{\mathrm{T}}^0),\mathcal{O}(\lambda_{\mathrm{T}})]$. To this end, we are able to regard the series in eq.~\eqref{eq:def:asyexp:c:mom} as a homogeneous expansion of $\widetilde{I}^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\} }$ within the $n$-collinear regime. % %The analogous circumstance can also be found in the expansion within the $\nbar-$collinear domain, in which $k_-\sim m_He^{\pm Y_H}\sim \mathcal{O}(\lambda^0_{\mathrm{T}})\gg k_+\sim \mathcal{O}(\lambda^2_{\mathrm{T}})$ and one is thus capable of expanding the function ${F}^{\{\beta \} }_{i/n}$ around $m_H e^{-Y_H}$. The result reads, %\begin{align}\label{eq:def:asyexp:cbar:mom} %&\widetilde{I}^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\} }\Bigg|_{c_{\nbar}} %= %\sum_{\omega}\,\widetilde{I}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|_{c_{\nbar}}\nonumber\\ %= %& %\sum_{\omega}\, %(\qT^2)^{ %%\sigma+\eta %\omega}\, % \int^{\frac{\qT^2}{\tilde{k}^{\mathrm{min}}_+}}_{\nu_{\nbar}}\, % \frac{\done k_-}{k_-}\, % \frac{ (k_-)^{\rho-\omega}}{(\omega-\sigma)!} \, % {F}^{\{\beta \},(\omega-\sigma)}_{i/n}\left( m_H e^{-Y_H}\right)\, % {F}^{\{\alpha \},(0)}_{j/\nbar}\left(k_-+m_H e^{+Y_H}\right)\, % \theta(\omega-\sigma). %\end{align} This leaves the transitional domain, as defined in Eq.~\eqref{eq:def:col-n:soft:col-nbar:cutoff}, to be calculated. In light of the scaling rules of Eq.~\eqref{eq:def:scaling:nun:nunbar}, we can expand both ${F}^{(\alpha_n)}_{i/n,\beta_n}$ and ${F}^{(\alpha_\nbar)}_{j/\nbar,\beta_\nbar}$ around the scales $m_H e^{\pm Y_H}$, more specifically, \begin{equation}\label{eq:def:asyexp:s:mom1} \begin{split} \widetilde{\mathcal{I}}^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\}}\Bigg|_{t}\, =\,& \sum_{\lambda,\eta=0}^{\infty}\, \int^{\nu_n}_{\frac{\qT^2}{\nu_{\nbar}}}\, \frac{\done k_+}{k_+}\, \frac{(k_-)^{\rho+\lambda}\,(k_+)^{\sigma+\eta}}{\lambda!\,\eta!} \, {F}^{(\alpha_n+\eta)}_{i/n,\beta_n}\left(m_H e^{-Y_H}\right)\, {F}^{(\alpha_\nbar+\lambda)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right) \,\\ =\,& \sum_{\lambda,\eta=0}^{\infty}\, \frac{{F}^{(\alpha_n+\eta)}_{i/n,\beta_n}\left(m_H e^{-Y_H}\right)\, {F}^{(\alpha_\nbar+\lambda)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)} {\lambda!\,\eta!} \,\\ &\hspace*{8mm}\times\, \Bigg\{ \underbrace{ \frac{(\qT^2)^{\rho+\lambda}\,\nu_n^{\sigma+\eta-\rho-\lambda}} {\sigma+\eta-\rho-\lambda}\, \bar{\delta}^{\sigma+\eta}_{\rho+\lambda} }_{n\text{-col}} +\underbrace{ \frac{(\qT^2)^{\sigma+\eta }\,\nu_{\nbar}^{\rho+\lambda-\sigma-\eta}} {\rho+\lambda-\sigma-\eta}\, \bar{\delta}^{\sigma+\eta}_{\rho+\lambda} }_{\nbar\text{-col}} +\underbrace{ (\qT^2)^{\sigma+\eta}\, \ln\left[\frac{\nu_n\nu_{\nbar}}{\qT^2}\right]\, {\delta}^{\sigma+\eta}_{\rho+\lambda} }_{n\text{-col}\,,~\nbar\text{-col}\,,~\text{s}}\, \Bigg\}\,,\hspace*{-10mm} \end{split} \end{equation} where we have already grouped the expression according to their powers in $\nu_n$ and $\nu_{\nbar}$. $\delta^{\alpha}_{\beta}$ is the Kronecker Delta, $\delta^{\alpha}_{\beta}=1$ if $\alpha=\beta$ and zero otherwise, $\bar{\delta}^{\alpha}_{\beta}\equiv1-\delta^{\alpha}_{\beta}$ is its complement. We note that even for fixed values of $\lambda$ and $\eta$, the phase space integral results in terms with a variety of power accuracies. For instance, in the first term on r.h.s.\ the power precision is determined by the exponent of $\qT$, which is identical to that of $k_-$ in the integrand. Hence, the scaling of the emitted momentum $k^{\mu}$ here is determined by the $n$-collinear mode $k_-\sim\mathcal{O}(\qT^2/m_H)$ and $k_+\sim\mathcal{O}(m_H)$. Similarly, applying this scaling analysis to the second term, its power precision is given by the exponent of $k_+$ and the $\nbar$-collinear mode with $k_-\sim\mathcal{O}(m_H)$ and $k_+\sim\mathcal{O}(\qT^2/m_H)$. The interpretation of the scaling of the integration variable of the last term of Eq.~\eqref{eq:def:asyexp:s:mom1} is more flexible due to the presence of the constraint $\rho+\lambda=\sigma+\eta$. Hence, the emitted parton can be constituted of either the $n(\nbar)$-collinear particle or the soft one $k_-\sim k_+\sim\mathcal{O}(\qT)$. % This inhomogeneity stems from our choice of the momentum cutoffs $\nu_n$ and $\nu_{\nbar}$ in Eq.~\eqref{eq:def:scaling:nun:nunbar}, from which multiple dynamic modes are allowed to participate in the transitional area, such as the $n$-collinear one, $\nbar$-collinear one, or the soft one. In principle, reducing $\nu_n$ and $\nu_{\nbar}$ down to $\mathcal{O}(\qT)$ will filter out the collinear modes in the transitional domain rendering it homogeneous again, at the price of additional soft scales in both collinear sectors through the boundary condition, necessitating a second expansion in the small parameters $\nu_n/m_H$ and $\nu_\nbar/m_H$ within there. It remains to be noted, while alternative choices of $\nu_n$ and $\nu_{\nbar}$ may modify the dynamics in each sector, their combined power series is invariant under this choice. Hence, in this work we choose the prescription of Eq.~\eqref{eq:def:scaling:nun:nunbar}, i.e.\ homogenous collinear sectors, for simplicity. By collecting and refactoring terms of a common power in \qT\ we can recast Eq.~\eqref{eq:def:asyexp:s:mom1} as \begin{align}\label{eq:def:asyexp:s:mom2} \widetilde{\mathcal{I}}^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\} }\Bigg|_{t}\, =\, \left( \sum_{\omega=\rho}^{\infty}\, (\qT^2)^{\omega}\, \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}} \Bigg|_{ cs}\, \right) + \left( \sum_{\omega=\sigma}^{\infty}\, (\qT^2)^{\omega}\, \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}} \Bigg|_{ \bar{c}s}\, \right)\,, \end{align} where \begin{equation}\label{eq:def:asyexp:cs:mom} \begin{split} &\widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}} \Bigg|_{cs} = \sum_{\eta=0}^{\infty} \frac{{F}^{(\eta+\alpha_n)}_{i/n,\beta_n}\left(m_H e^{-Y_H}\right) {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)\,} {(\omega-\rho)!\,\eta!} \Bigg\{ \frac{\nu_n^{\sigma+\eta-\omega}}{\sigma+\eta-\omega} \bar{\delta}^{\sigma+\eta}_{\omega} +\ln\left[\frac{\nu_n}{\qT}\right]{\delta}^{\sigma+\eta}_{\omega}\, \Bigg\}\,, \\ &\widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}} \Bigg|_{\bar{c}s} = \sum_{\lambda=0}^{\infty} \frac{{F}^{(\alpha_n+\omega-\sigma)}_{i/n,\beta_n}\left(m_H e^{-Y_H}\right) {F}^{(\alpha_\nbar+\lambda)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)} {(\omega-\sigma)!\,\lambda!} \Bigg\{ \frac{\nu_{\nbar}^{\rho+\lambda-\omega}}{\rho+\lambda-\omega} \bar{\delta}^{\rho+\lambda}_{\omega} +\ln\left[\frac{\nu_{\nbar}}{\qT}\right]{\delta}^{\rho+\lambda}_{\omega} \Bigg\}\,. \end{split} \end{equation} Here we have re-organized the logarithmic terms in Eq.~\eqref{eq:def:asyexp:s:mom1} into the $n$-collinear-soft ($cs$) and $\nbar$-collinear-soft ($\bar{c}s$) sectors based on their scale dependences. At variance from the results in Eq.~\eqref{eq:def:asyexp:c:mom:at:omega} and Eq.~\eqref{eq:def:asyexp:cbar:mom:at:omega} in the $n$- and $\nbar$-collinear sectors, where the coefficients at each power consist of only the hard scales $k_\pm$, respectively, Eq.~\eqref{eq:def:asyexp:cs:mom} here introduces an additional dependence on $\ln\left({\nu_{n(\nbar)}}/{\qT}\right)$. % In order to facilitate numerical calculations of these coefficients, we rewrite the infinite series in Eq.~\eqref{eq:def:asyexp:cs:mom} in terms of the integrals over $k_\pm$, in analogy to Eqs.~\eqref{eq:def:asyexp:c:mom:at:omega} and \eqref{eq:def:asyexp:cbar:mom:at:omega}. If $\omega<\sigma$ in Eq.~\eqref{eq:def:asyexp:cs:mom}, this transformation is immediate, \begin{equation}\label{eq:def:asyexp:cs:mom:reg} \begin{split} & \bar{\theta}(\omega-\sigma)\, \sum_{ \eta =0}^{\infty}\, \frac{{F}^{(\eta+\alpha_n)}_{i/n,\beta_n}\left(m_H e^{-Y_H}\right)\, {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)\,} {(\omega-\rho)!\,\eta!} \, \frac{\nu_n^{\sigma+\eta-\omega}}{\sigma+\eta-\omega}\,\\ &\qquad\qquad\qquad \Longrightarrow\, \frac{\bar{\theta}(\omega-\sigma)}{(\omega-\rho)!}\, \int^{\nu_n}_0\,\frac{\done k_+}{k_+}\, k_+^{\sigma-\omega}\, {F}^{(\alpha_n)}_{i/n,\beta_n}\left(k_++m_H e^{-Y_H}\right)\, {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right) \,. \end{split} \end{equation} Here we have removed $\bar{\delta}^{\sigma+\eta}_{\omega}$ from the expressions since it always equals unity while $\omega<\sigma$ and $\eta\ge0$. The same reasoning can also be used to neglect the logarithmic contributions in Eq.~\eqref{eq:def:asyexp:cs:mom}. However, it is not straightforward to apply Eq.~\eqref{eq:def:asyexp:cs:mom:reg} in the remaining space with $\omega\ge\sigma$ as the integrand is singular in the limit $k_+\to0$. To this end, we make use of the higher-ranked star distribution, \begin{align}\label{eq:def:sDist} \int_0^{\Lambda}\,\done x\, \left[\frac{1}{x^m}\right]^{\nu}_{*}\,f(x) \equiv \int_{\nu}^{\Lambda}\,\done x\,\frac{f(x)}{x^m} + \int_0^{\nu}\,\done x\,\frac{1}{x^m}\, \left[f(x)-\sum_{n=0}^{m-1}\frac{x^n}{n!}f^{(n)}(0)\right]\,, \end{align} to maintain the end point analyticity. Therein, $f(x)$ is assumed to be always differentiable at $x=0$. With $m=1$, Eq.~\eqref{eq:def:sDist} reduces to the customary star distribution proposed in \cite{DeFazio:1999ptt,Bosch:2004th}. Equipped with eq.~\eqref{eq:def:sDist}, we are now able to convert the $n$-collinear-soft contribution in the case $\omega\ge\sigma$ and $\eta> \omega-\sigma$, \begin{equation}\label{eq:def:asyexp:cs:mom:dist} \begin{split} &{\theta}( \omega-\sigma)\, \sum_{\eta =\omega-\sigma+1}^{\infty}\, \frac{{F}^{(\eta+\alpha_n)}_{i/n,\beta_n}\left(m_H e^{-Y_H}\right)\, {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)\,}{(\omega-\rho)!\,\eta!}\, \frac{\nu_n^{\sigma+\eta-\omega}}{\sigma+\eta-\omega}\,\\ & \qquad\qquad\Longrightarrow\, \frac{{\theta}(\omega-\sigma)}{(\omega-\rho)!}\, \int^{\nu_n}_0\,\done k_+\, \left[\frac{1}{k_+^{\omega-\sigma+1}}\right]^{\nu_n}_{*}\, {F}^{(\alpha_n)}_{i/n,\beta_n}\left( k_++m_H e^{-Y_H}\right)\, {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)\,. \end{split} \end{equation} The remaining contributions in Eq.~\eqref{eq:def:asyexp:cs:mom} include the logarithms $\ln\left({\nu_{n}}/{\qT}\right)$ as well as the first $(\omega-\sigma)$ terms of the Taylor series. We will refrain from transforming those contributions here since, at a given power precision, the number of remaining terms are always finite. Combining above results we can recast the $n$-collinear-soft contribution of Eq.~\eqref{eq:def:asyexp:cs:mom} as follows \begin{equation}\label{eq:def:asyexp:cs:mom:int} \begin{split} \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|_{cs} = &\phantom{{}+} \frac{\bar{\theta}( \omega-\sigma)}{(\omega-\rho)!}\, \int^{\nu_n}_0\,\frac{\done k_+}{k_+}\,k_+^{\sigma-\omega}\, {F}^{(\alpha_n)}_{i/n,\beta_n}\left(k_++m_H e^{-Y_H}\right)\, {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right) \,\\ &{}+ \frac{{\theta}(\omega-\sigma)}{(\omega-\rho)!}\, \int^{\nu_n}_0\,\done k_+\, \left[\frac{1}{k_+^{\omega-\sigma+1}}\right]^{\nu_n}_{*}\, {F}^{(\alpha_n)}_{i/n,\beta_n}\left(k_++m_H e^{-Y_H}\right)\, {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)\,\\ &{}+ \frac{{\theta}(\omega-\sigma-1)}{(\omega-\rho)!}\, \sum_{\eta=0}^{\omega-\sigma-1}\, \frac{{F}^{(\alpha_n+\eta)}_{i/n,\beta_n}\left(m_H e^{-Y_H}\right)\, {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)\,} {\eta!} \, \frac{\nu_n^{\sigma+\eta-\omega}}{\sigma+\eta-\omega}\,\\ &{}+ \frac{{\theta}(\omega-\sigma)}{(\omega-\rho)!}\, \ln\left[\frac{\nu_n}{\qT}\right]\, \frac{{F}^{(\alpha_n+\omega-\sigma)}_{i/n,\beta_n}\left(m_H e^{-Y_H}\right)\, {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)\,}{(\omega-\sigma)!} \,. \end{split} \end{equation} By analogy, the contribution of the $\nbar$-collinear-soft sector in Eq.~\eqref{eq:def:asyexp:cs:mom} can be transformed to finite integrals following an analogous path, giving \begin{equation}\label{eq:def:asyexp:cbars:mom:int} \begin{split} \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|_{\bar{c}s} = &\phantom{{}+} \frac{\bar{\theta}(\omega-\rho)}{(\omega-\sigma)!}\, \int^{\nu_{\nbar} }_0\,\frac{\done k_-}{k_-}\,k_-^{\rho-\omega}\, {F}^{(\alpha_n+\omega-\sigma)}_{i/n,\beta_n}\left(m_H e^{-Y_H}\right)\, {F}^{(\alpha_\nbar)}_{j/\nbar,\beta_\nbar}\left(k_-+m_H e^{+Y_H}\right)\,\\ &{}+ \frac{{\theta}(\omega-\rho)}{(\omega-\sigma)!}\, \int^{\nu_{\nbar}}_0\,\done k_-\, \left[\frac{1}{k_-^{\omega-\rho+1}}\right]^{\nu_{\nbar}}_{*}\, {F}^{(\alpha_n+\omega-\sigma)}_{i/n,\beta_n}\left(m_H e^{-Y_H}\right)\, {F}^{(\alpha_\nbar)}_{j/\nbar,\beta_\nbar}\left(k_-+m_H e^{+Y_H}\right)\,\\ &{}+ \frac{{\theta}(\omega-\rho-1)}{(\omega-\sigma)!}\, \sum_{\lambda=0}^{\omega-\rho-1}\, \frac{{F}^{(\alpha_n+\omega-\sigma)}_{i/n,\beta_n}\left(m_H e^{-Y_H}\right)\, {F}^{(\alpha_\nbar+\lambda)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)\,}{\lambda!} \, \frac{\nu_{\nbar}^{\rho+\lambda-\omega}}{\rho+\lambda-\omega}\,\\ &{}+ \frac{{\theta}(\omega-\rho)}{(\omega-\sigma)!}\, \ln\left[\frac{\nu_{\nbar}}{\qT}\right]\, \frac{{F}^{(\alpha_n+\omega-\sigma)}_{i/n,\beta_n}\left(m_H e^{-Y_H}\right)\, {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)\,}{(\omega-\rho)!}\,. \end{split} \end{equation} Using the above result we can now combine the $n$-collinear sector of Eq.~\eqref{eq:def:asyexp:c:mom}, the $\nbar$-collinear sector of Eq.~\eqref{eq:def:asyexp:cbar:mom}, and the transitional sector of Eqs.~\eqref{eq:def:asyexp:cs:mom:int} and \eqref{eq:def:asyexp:cbars:mom:int}, arriving at the expansion of $\widetilde{\mathcal{I}}^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\}}$ of Eq.~\eqref{eq:def:I:central} in powers of $\qT^2$ in the small \qT~domain, \begin{align}\label{eq:def:asyexp:central:power:omega} \widetilde{\mathcal{I}}^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\} } = \sum_{\omega}(\qT^2)^{\omega}\, \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}} \equiv \sum_{\omega}(\qT^2)^{\omega} \Bigg\{ \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|_{c} + \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|_{\bar{c}} + \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|_{cs} + \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|_{\bar{c}s} \Bigg\}\,. \end{align} At this point it merits reminding that the pair of auxiliary scales, $\nu_n$ and $\nu_{\nbar}$, that we have employed to define and separate the dynamic regions in Eq.~\eqref{eq:def:col-n:soft:col-nbar:cutoff} appear explicitly in the expressions of all three individual domains. For consistency's sake, it is of the essence to examine whether the combination of all domains also exhibits such a dependence, or whether this dependence, in fact, vanishes after summing over all the ingredients. To this end, we take the derivatives of the r.h.s.\ of Eq.~\eqref{eq:def:asyexp:central:power:omega} with respect to $\nu_n$, and it evaluates to \begin{equation}\label{eq:def:asyexp:central:power:omega:nundiff} \begin{split} & \frac{\partial}{\partial \nu_n} \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|_{c} = -\,\frac{\partial }{\partial \nu_n} \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|_{cs} = -\frac{(\nu_n)^{\sigma-\omega-1}}{(\omega-\rho)} {F}^{(\alpha_n)}_{i/n,\beta_n}\left(\nu_n+m_H e^{-Y_H}\right) {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right),\\ & \frac{\partial}{\partial \nu_n} \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|_{\bar{c}} = \frac{\partial}{\partial \nu_n} \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|_{\bar{c}s} =0\,, \end{split} \end{equation} where the results of Eqs.~\eqref{eq:def:asyexp:c:mom:at:omega} and \eqref{eq:def:asyexp:cs:mom:int} are utilised to derive the r.h.s.\ of Eq.~\eqref{eq:def:asyexp:central:power:omega:nundiff}. In addition, the terms arising from the derivative of the star distribution, defined in Eq.~\eqref{eq:def:sDist}, have been cancelled against the $\nu_n$ dependences arising from the logarithmic term and the truncated Taylor polynomials in Eq.~\eqref{eq:def:asyexp:cs:mom:int}. A similar result can also be found for the $\nu_\nbar$ dependence of Eq.~\eqref{eq:def:asyexp:central:power:omega}, giving \begin{equation}\label{eq:def:asyexp:central:power:omega:nunbardiff} \begin{split} & \frac{\partial}{\partial \nu_\nbar} \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|_{c} = \frac{\partial}{\partial \nu_\nbar} \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|_{cs} = 0\,,\\ & \frac{\partial}{\partial \nu_\nbar} \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|_{\bar{c}} = -\frac{\partial}{\partial \nu_\nbar} \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|_{\bar{c}s} =- \frac{(\nu_\nbar)^{\rho-\omega-1}}{(\omega-\sigma)!} {F}^{(\alpha_n+\omega-\sigma)}_{i/n,\beta_n}\left(m_H e^{-Y_H}\right) {F}^{(\alpha_\nbar)}_{j/\nbar,\beta_\nbar}\left(\nu_\nbar+m_H e^{+Y_H}\right) . \end{split} \end{equation} Combining the results of Eqs.~\eqref{eq:def:asyexp:central:power:omega:nundiff} and \eqref{eq:def:asyexp:central:power:omega:nunbardiff}, respectively, we can conclude that the coefficient $\widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}$ in Eq.~\eqref{eq:def:asyexp:central:power:omega} is indeed independent of the choice of the separators $\nu_n$ and $\nu_\nbar$ at each power. This agrees with the expectation from a direct expansion of $\widetilde{\mathcal{I}}^{\rho,\sigma }_{[\kappa],\{\alpha,\beta\}}$, currently beyond our capabilities as the PDFs are not rigorously known analytically, that it should be a function of $\qT$, $s$, and $m_H$ only and independent of $\nu_n$ or $\nu_\nbar$. \subsubsection{Rapidity regularisation and zero-bin subtraction}\label{sec:asyexp:qT:extrapl} In the previous section, with the help of the auxiliary scales $\nu_n$ and $\nu_\nbar$, we have derived the power series for $\widetilde{\mathcal{I}}^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\}}$ in Eq.~\eqref{eq:def:asyexp:central:power:omega} in the vicinity $\qT=0$ at central rapidities, $e^{\pm Y_H}\sim\mathcal{O}(1)$. Even though this strategy has accomplished an asymptotic expansion of $\widetilde{\mathcal{I}}^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\}}$, and in turn the \qT~distribution, at NLO, it is not straightforward to generalise this method to higher perturbative orders. The presence of subdivisions of phase space through the auxiliary scales $\nu_n$ and $\nu_\nbar$, generally inducing additional scales to phase space and loop integrals, complicates the calculations substantially. Further, the absence of additional constraints on the integration paths is also one of prerequisites to establish the factorisation in a SCET-based analysis. To this end, we will discuss the rearrangement of the ingredients defined in Eqs.~\eqref{eq:def:asyexp:c:mom:at:omega} and \eqref{eq:def:asyexp:cbar:mom:at:omega} as well as Eqs.~\eqref{eq:def:asyexp:cs:mom:int} and \eqref{eq:def:asyexp:cbars:mom:int} such that the dependence on the auxiliary scales to subdivide the phase space is removed. In particular, recalling our findings regarding the $\nu_{n(\nbar)}$-independence of $\widetilde{\mathcal{I}}^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\}}$, but not its components in Eqs.~\eqref{eq:def:asyexp:central:power:omega:nundiff} and \eqref{eq:def:asyexp:central:power:omega:nunbardiff}, such a rearrangement is warranted. Although in the discussion below, we will still restrict ourselves to the NLO constituent $\widetilde{\mathcal{I}}^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\}}$ extracted from Eq.~\eqref{eq:msq} as an illustrative example, it is expected that the conclusion here can provide the theoretical baseline for an analysis in more general situations. We start by examining the collinear sectors. Here, eliminating the dependences of the auxiliary scales $\nu_n$ and $\nu_\nbar$ amounts to reducing the lower boundaries in Eq.~\eqref{eq:def:asyexp:c:mom:at:omega} and Eq.~\eqref{eq:def:asyexp:cbar:mom:at:omega} from their intrinsic domains defined in Eq.~\eqref{eq:def:scaling:nun:nunbar} to the origin. To be precise, we split \begin{align}\label{eq:def:asyexp:c:cbar:diff} \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|_{c} \, =\, \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|_{c} \, -\, \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|_{c0} \,, \qquad\quad \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|_{\bar{c}}\, =\, \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|_{\bar{c}}\, -\, \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|_{\bar{c}0}\,, \end{align} where $\widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\big|_{c}$ and $\widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\big|_{\bar{c}}$ collect the collinear contributions, integrating the light-cone momentum over the entire range. Their expressions read \begin{equation}\label{eq:def:asyexp:c:at:omega:nured} \begin{split} \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|_{c} &\equiv \lim_{\tau\to0}\int^{\tilde{k}^{\mathrm{max}}_+}_{0} \frac{\done k_+}{k_+} \mathcal{R}(k_-,k_+,\tau) \frac{(k_+)^{\sigma-\omega}}{(\omega-\rho)!} {F}^{(\alpha_n)}_{i/n,\beta_n}\left(k_++m_H e^{-Y_H}\right) {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right), \\ \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|_{\bar{c}} &\equiv \lim_{\tau\to0}\int^{\frac{\qT^2}{\tilde{k}^{\mathrm{min}}_+}}_{0} \frac{\done k_-}{k_-} \mathcal{R}(k_-,k_+,\tau) \frac{(k_-)^{\rho-\omega}}{(\omega-\sigma)!} {F}^{(\alpha_n+\omega-\sigma)}_{i/n,\beta_n}\left( m_H e^{-Y_H}\right) {F}^{(\alpha_\nbar)}_{j/\nbar,\beta_\nbar}\left(k_-+m_H e^{+Y_H}\right). \end{split} \end{equation} Therein, in order to regularise the rapidity divergence in the limit $k_{\pm}\to0$, we multiply the original integrand by $\mathcal{R}(k_-,k_+,\tau)$, which is a function of the light-cone momenta $k_{\pm}$ and a real parameter $\tau$, satisfying, \begin{align}\label{rap:def:feat} \lim_{\tau\to0}\, \mathcal{R}(k_-,k_+,\tau)\, =\, \left\{ \begin{matrix} 1 & \text{$k_{\pm}\neq 0$}\,,\\ 0 & \text{$k_{+}=0$~or~$k_{-}=0$}\,. \end{matrix} \right. \end{align} For the regions $k_{\pm}\neq 0$, the integrands in Eq.~\eqref{eq:def:asyexp:c:at:omega:nured} are uniformly convergent, which permits reducing the rapidity regulator $\mathcal{R}(k_-,k_+,\tau)$ in the limit $\tau\to0$ and restoring the integrands to their original forms. Nevertheless, in the asymptotic area $k_{+}=0$~or~$k_{-}=0$, the role of the rapidity regulator becomes indispensable, ensuring that the phase space integrals in Eq.~\eqref{eq:def:asyexp:c:at:omega:nured} are always well defined. The discussion in this section will emphasise rapidity regulators that are able to preserve their expressions in both the $n$-collinear and $\nbar$-collinear sectors for all powers, such as the analytic regulator of \cite{Becher:2010tm,Becher:2011dz}, the exponential regulator of \cite{Li:2016axz,Li:2016ctv}, and the pure rapidity regulator of \cite{Ebert:2018gsn,Moult:2019vou}. We will dub them the conservative rapidity regulator or conservative regularisation scheme (CRa) hereafter. Other than that, there are also alternative proposals, including the $\Delta$-regulator \cite{Chiu:2009yx, Echevarria:2011epo,Echevarria:2015usa,Echevarria:2015byo, Echevarria:2016scs} and the $\eta$-regulator \cite{Chiu:2011qc,Chiu:2012ir}. At this point, either the rapidity regulators themselves or the regulator-dressed propagators will participate in the power expansion such that in practice the rapidity divergences can be regularised in varying strategies in different ingredients from power to power. They will be called dissipative rapidity regulator (DRa) in this work. We will postpone their investigation for now but discuss the possible prescriptions in App.~\ref{sec:dis:reg}. In Eq.\ \eqref{eq:def:asyexp:c:cbar:diff}, we have also introduced $\widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\big|_{c0}$ and $\widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\big|_{\bar{c}0}$ in order to restore the equality after. Their expressions read, \begin{equation}\label{eq:def:asyexp:c:at:omega:nured:diff} \begin{split} &\widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|_{c0} = \lim_{\tau\to0}\int^{\nu_n}_{0} \frac{\done k_+}{k_+} \mathcal{R}(k_-,k_+,\tau) \frac{(k_+)^{\sigma-\omega}}{(\omega-\rho)!} {F}^{(\alpha_n)}_{i/n,\beta_n}\left(k_++m_H e^{-Y_H}\right) {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right), \\ &\widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|_{\bar{c}0} = \lim_{\tau\to0}\int^{\nu_{\nbar}}_{0} \frac{\done k_-}{k_-} \mathcal{R}(k_-,k_+,\tau) \frac{(k_-)^{\rho-\omega}}{(\omega-\sigma)!} {F}^{(\alpha_n+\omega-\sigma)}_{i/n,\beta_n}\left( m_H e^{-Y_H}\right) {F}^{(\alpha_\nbar)}_{j/\nbar,\beta_\nbar}\left(k_-+m_H e^{+Y_H}\right). \end{split} \end{equation} Since these functions are always associated with the $k_{\pm}$ integrals from the origin point up to the cutoffs $\nu_{n(\nbar)}$, we will make use of the subscripts $``c0"$ $(``\bar{c}0")$ to represent them hereafter. From Eq.~\eqref{eq:def:asyexp:c:at:omega:nured:diff}, noting that the integration variables $k_{\pm}$ are both well situated within the convergence radii of ${F}_{i/n,\beta_n}$ and ${F}_{j/\nbar,\beta_\nbar}$, according to Sec.~\ref{sec:setups}, we can now perform the power expansion in $k_{\pm}$. We then have, \begin{equation}\label{eq:def:asyexp:c0:at:omega:nured:diff:decomp} \begin{split} &\widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|_{c0}\, =\, \frac{{F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)}{(\omega-\rho)!}\, \left\{ \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|_{c0r}\, +\, \theta\left(\omega-\sigma\right)\, \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|_{c0d}\, \right\}\,,\\ &\widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|_{\bar{c}0}\, =\, \frac{{F}^{(\alpha_n+\omega-\sigma)}_{i/n,\beta_n}\left( m_H e^{-Y_H}\right)}{(\omega-\sigma)!}\, \left\{ \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|_{\bar{c}0r}\, +\, \theta\left(\omega-\rho\right)\, \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|_{\bar{c}0d}\, \right\}\,, \end{split} \end{equation} where \begin{equation}\label{eq:def:asyexp:c0r:at:omega:nured:diff} \begin{split} \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|_{c0r} &=\, \sum^{\infty}_{\eta=\mathrm{max}\{0,(\omega-\sigma+1)\}} \frac{\nu^{\sigma-\omega+\eta}_n}{\sigma-\omega+\eta} \frac{{F}^{(\alpha_n+\eta)}_{i/n,\beta_n}\left(m_H e^{-Y_H}\right)}{\eta!}\,, \\ \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|_{\bar{c}0r} &=\, \sum^{\infty}_{\lambda=\mathrm{max}\{0,(\omega-\rho+1)\}} \frac{\nu^{\rho-\omega+\lambda}_\nbar}{\rho-\omega+\lambda} \frac{{F}^{(\alpha_\nbar+\lambda)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)}{\lambda!}\,, \\ \end{split} \end{equation} are the regular components, where the regulator could be safely removed by the means of Eq.\ \eqref{rap:def:feat}, and \begin{equation}\label{eq:def:asyexp:c0d:at:omega:nured:diff} \begin{split} \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|_{c0d} &=\, \sum_{\eta=0}^{\omega-\sigma}\, \frac{{F}^{(\alpha_n+\eta)}_{i/n,\beta_n}\left(m_H e^{-Y_H}\right)}{\eta!}\, \left\{ \lim_{\tau\to0}\int^{\nu_n}_{0} \frac{\done k_+}{k_+} \mathcal{R}(k_-,k_+,\tau) (k_+)^{\sigma-\omega+\eta} \right\}\,, \\ \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|_{\bar{c}0d} &=\, \sum_{\lambda=0}^{\omega-\rho}\, \frac{{F}^{(\alpha_\nbar+\lambda)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)}{\lambda!}\, \left\{ \lim_{\tau\to0}\int^{\nu_\nbar}_{0} \frac{\done k_-}{k_-} \mathcal{R}(k_-,k_+,\tau) (k_-)^{\rho-\omega+\lambda} \right\}\,. \end{split} \end{equation} contain the (regulated) rapidity divergences at $k_{\pm}\to0$. Here, the regulator $\mathcal{R}(k_-,k_+,\tau)$ is essential and the respective integrals are therefore dependent on the choice of the regularisation scheme. Substituting Eq.~\eqref{eq:def:asyexp:c0r:at:omega:nured:diff} into Eq.~\eqref{eq:def:asyexp:c0:at:omega:nured:diff:decomp}, we observe that the results for $\widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\big|_{c0}$ and $\widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\big|_{c0}$ still explicitly depend on the auxiliary scales $\nu_{n(\nbar)}$. However, according to Eq.~\eqref{eq:def:asyexp:central:power:omega:nundiff}, all those dependences will drop out upon combining them with the contributions from the transitional region of Eq.~\eqref{eq:def:asyexp:cs:mom}, and it follows that \begin{align}\label{eq:id:mom:rsp} \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|_{ cs} + \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|_{\bar{c}s} - \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|_{c0} - \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|_{\bar{c}0} = \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|_{comb}, \end{align} where on the r.h.s., $\widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\big|_{comb}$, comprises a set of one-fold integrals of $k_+$ or $k_-$ over the range $[0,+\infty]$. Its precise form will be specified below. In the literature, there are two preferences for expressing this combined result. The first one, used extensively when using the method of expansion by regions \cite{Beneke:1997zp, Smirnov:1998vk,Smirnov:1999bza,Smirnov:2002pj, Jantzen:2011nz} and SCET~\cite{Bauer:2001yt,Bauer:2001ct,Bauer:2000yr, Bauer:2000ew,Bauer:2002nz,Beneke:2002ph,Beneke:2002ni, Bauer:2002aj,Lange:2003pk,Beneke:2003pa}, comprises the soft interaction $k_{\pm}\sim\mathcal{O}(\qT)$ in full as well as the subtraction terms to remove the overlap with the collinear regions. Hereafter, we will refer to the results from this formulation as the full soft \FSmeth prescription. It yields that \begin{align}\label{eq:def:s:ccs:fs:rap} \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|_{comb}\, =\, \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|^{\FSmeth}_{s}\, -\, \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|^{\FSmeth}_{c\bar{c}s}\,. \end{align} Here $\widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\big|^{\FSmeth}_{s}$ stands for the soft contribution, derived by expanding the integrand in Eq.~\eqref{eq:def:I:central} in accordance with the soft scaling $k_{\pm}\sim\mathcal{O}(\qT)$. At the $\omega$th-power, the result reads, \begin{align}\label{eq:def:s:fs:rap} \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|^{\FSmeth}_{s}\, =&\, \theta(\omega-\rho-\sigma)\, \sum_{\eta=0}^{(\omega-\rho-\sigma)}\, {F}^{(\alpha_n+\omega-\rho-\sigma-\eta)}_{i/n,\beta_n}\left(m_He^{-Y_H}\right)\, {F}^{(\alpha_\nbar +\eta)}_{j/\nbar,\beta_\nbar}\left(m_He^{+Y_H}\right)\, \lim_{\tau\to0}\, \int^{\infty}_{0}\, \frac{\done k_+}{k_+} \, \nnb\\ &\times \mathcal{R}(k_-,k_+,\tau) \, \frac{(k_-)^{\rho+\eta-\omega}}{\eta !} \, \frac{ (k_+)^{ -\rho -\eta }}{(\omega-\rho-\sigma-\eta)!}\,, \end{align} where we have extracted the factor of $(\qT^{2})^{\omega}$ from the integrals in Eq.~\eqref{eq:def:s:fs:rap}, in line with the definition of the power series in Eq.~\eqref{eq:def:asyexp:central:power:omega}. Given the expression in Eq.~\eqref{eq:def:s:fs:rap}, we can obtain an expression for $\widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\big|^{\FSmeth}_{c\bar{c}s}$ by comparing Eq.~\eqref{eq:def:s:ccs:fs:rap} with Eq.~\eqref{eq:id:mom:rsp}. As this subtrahend at LP is intimately associated with the soft limit of the collinear functions and thus the zeroth-bin of the label momentum within the position-momentum space hybrid representation, $\widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\big|^{\FSmeth}_{c\bar{c}s}$ is frequently dubbed the zero-bin contribution \cite{Manohar:2006nz,Idilbi:2007yi,Idilbi:2007ff,Chiu:2009yx} or the soft subtraction term \cite{Ji:2004xq,Ji:2004wu, Idilbi:2007yi,Idilbi:2007ff,Echevarria:2011epo}. On the other hand, there are also alternative proposals in the literature~\cite{Vladimirov:2021hdn,Vladimirov:2023aot, Goerke:2017ioi,Inglis-Whalen:2020rpi,Inglis-Whalen:2021bea}. There, a decomposition of Eq.~\eqref{eq:id:mom:rsp} without an explicit soft sector is chosen. The virtue of such a scheme is that in absence of the soft contribution the soft-collinear interaction vertices do not need to be expanded using multiple scaling regimes, and the factorisation of the distinct dynamic modes is thus considerably simplified. In this work, we will dub this approach the one in the non-soft \NSmeth prescription. It follows that, \begin{align} \label{eq:def:s:ccs:ns:rap} \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|_{comb}\, =\, -\, \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|^{\NSmeth}_{c\bar{c}}\,. \end{align} Hence, the interior contribution $\widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}$ in Eq.~\eqref{eq:def:I:central} consists of only the collinear sectors in Eq.~\eqref{eq:def:asyexp:c:at:omega:nured} as well as $\widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\big|^{\NSmeth}_{c\bar{c}}$. Since $\widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\big|^{\NSmeth}_{c\bar{c}}$ here effectively removes the overlap between the $n$-collinear and $\nbar$-collinear contributions, it is also named the overlap subtraction term in \cite{Goerke:2017ioi,Inglis-Whalen:2020rpi,Inglis-Whalen:2021bea}. Notwithstanding, in view of the functional similarity of $\widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\big|^{\NSmeth}_{c\bar{c}}$ and $\widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\big|^{\FSmeth}_{c\bar{c}s}$, we will not further distinguish the terminologies in this paper, such as the overlapping subtraction, the zero-bin contribution, or the soft remover. Instead, they will be all regarded to be conceptually equivalent but evaluated within different prescriptions. Comparing Eq.~\eqref{eq:def:s:ccs:ns:rap} with Eq.~\eqref{eq:def:s:ccs:fs:rap}, we note that the subtraction terms in those two schemes possess the following relation, \begin{align}\label{eq:def:ns:fs:trans} \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|^{\NSmeth}_{c\bar{c}}\, =\, \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|^{\FSmeth}_{c\bar{c}s}\, -\, \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|^{\FSmeth}_{s}\,. \end{align} In the following, we will be focused on the derivation of $\widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\big|^{\NSmeth}_{c\bar{c}}$. The expressions within the \FSmeth prescription can be obtained by means of the relationship above. %\commentWJ{seems to that the soft function is artificial and one in principle could totally live in a world with only collinear modes.} We begin with the transformation of $\widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\big|_{cs}$ and $\widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\big|_{ \bar{c}s}$. As illustrated in Eq.~\eqref{eq:def:asyexp:cs:mom}, $\widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\big|_{cs}$ comprises the logarithmic terms in the case of ${\omega}={(\sigma+\eta)}$ and powers of the auxiliary scales $\nu_{n(\nbar)}$ otherwise. The latter contribution can be further categorised based on the relation between $\omega$ and $(\sigma+\eta)$, more specifically, \begin{equation}\label{eq:reexp:sc1} \begin{split} &\hspace*{-5mm}\sum_{\eta =0}^{\infty} \frac{{F}^{(\eta+\alpha_n)}_{i/n,\beta_n}\left( m_H e^{-Y_H}\right) {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)\,} {(\omega-\rho)!\,\eta!} \frac{\nu_n^{\sigma+\eta-\omega}}{\sigma+\eta-\omega} \bar{\delta}^{\sigma+\eta}_{\omega}\\ =\,& \frac{{F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)}{(\omega-\rho)!} \Bigg\{ \sum_{\eta=\mathrm{max}\{0,(\omega-\sigma+1)\}}^{\infty} \frac{{F}^{(\alpha_n+\eta)}_{i/n,\beta_n}\left( m_H e^{-Y_H}\right)} {\eta!} \frac{\nu_n^{\sigma+\eta-\omega}}{\sigma+\eta-\omega}\\ &\hspace*{30mm}{} -\theta(\omega-\sigma-1)\sum_{\eta=0}^{\omega-\sigma-1} \frac{{F}^{(\alpha_n+\eta)}_{i/n,\beta_n}\left(m_H e^{-Y_H}\right)} {\eta!\,} \lim_{\tau\to0}\int^{\infty}_{\nu_n}\frac{\done k_+}{k_+} \mathcal{R}(k_-,k_+,\tau)(k_+)^{\sigma-\omega+\eta} \Bigg\}\,.\hspace*{-20mm} \end{split} \end{equation} Therein, within the curly brackets, the first term collects all the contributions with $\omega<(\sigma+\eta)$, whilst the second term collects all contributions with $\omega>(\sigma+\eta)$ and has been transformed into its integral form. Aiming at a representation for $\widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\big|_{cs}$ that can manifestly cancel against the $\nu_n$ dependences in Eq.~\eqref{eq:def:asyexp:c0r:at:omega:nured:diff} and Eq.~\eqref{eq:def:asyexp:c0d:at:omega:nured:diff}, the rapidity regulator $\mathcal{R}(k_-,k_+,\tau)$ is introduced here for bookkeeping purposes. Once the relationship $\omega<(\sigma+\eta)$ is satisfied, $\mathcal{R}(k_-,k_+,\tau)$ always stays inactive in the limit $\tau\to0$. An analogous rearrangement is also applicable to $\widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\big|_{ \bar{c}s}$ in Eq.~\eqref{eq:def:asyexp:cs:mom}. It yields that \begin{equation}\label{eq:reexp:scbar1} \begin{split} &\hspace*{-5mm}\sum_{\lambda =0}^{\infty} \frac{{F}^{(\alpha_n+\omega-\sigma)}_{i/n,\beta_n}\left( m_H e^{-Y_H}\right) {F}^{(\alpha_\nbar+\lambda)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)} {(\omega-\sigma)!\,\lambda!} \frac{\nu_{\nbar}^{\rho+\lambda-\omega}}{\rho+\lambda-\omega} \bar{\delta}^{\rho+\lambda}_{\omega}\\ =\,& \frac{{F}^{(\alpha_n+\omega-\sigma)}_{i/n,\beta_n}\left( m_H e^{-Y_H}\right)}{(\omega-\sigma)!}\, \Bigg\{ \sum_{\lambda=\mathrm{max}\{0,(\omega-\rho+1)\}}^{\infty} \frac{{F}^{(\alpha_\nbar+\lambda)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)} {\lambda!} \frac{\nu_{\nbar}^{\rho+\lambda-\omega}}{\rho+\lambda-\omega}\\ &\hspace*{30mm}{} -\theta(\omega-\rho-1)\sum_{\lambda=0}^{\omega-\rho-1}\, \frac{{F}^{(\alpha_\nbar+\lambda)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)} {\lambda!} \lim_{\tau\to0}\int^{\infty}_{\nu_\nbar}\frac{\done k_-}{k_-} \mathcal{R}(k_-,k_+,\tau)(k_-)^{\rho+\lambda-\omega} \Bigg\}\,.\hspace*{-20mm} \end{split} \end{equation} We can now recast the logarithmic contributions of $\widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\big|_{cs}$ and $\widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\big|_{\bar{c}s}$ in integral form, as presented in Eqs.~\eqref{eq:def:asyexp:s:mom2} and \eqref{eq:def:asyexp:cs:mom}. It is worth noting at this point that the logarithmic terms from both sectors always and only appear together once $\omega\ge\rho$ and $\omega\ge\sigma$ simultaneously. Therefore, in the following, we cope with them simultaneously, i.e., \begin{equation}\label{eq:reexp:sc:scbar:log} \begin{split} &\hspace*{-5mm} \frac{{F}^{(\alpha_n+\omega-\sigma)}_{i/n,\beta_n}\left(m_H e^{-Y_H}\right) {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)\,}{(\omega-\rho)!\,(\omega-\sigma)!} \Bigg\{ \ln\left[\frac{\nu_n}{\qT}\right]\, +\, \ln\left[\frac{\nu_{\nbar}}{\qT}\right] \Bigg\} \\ =\,& \frac{{F}^{(\alpha_n+\omega-\sigma)}_{i/n,\beta_n}\left(m_H e^{-Y_H}\right) {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)\,}{(\omega-\rho)!\,(\omega-\sigma)!}\\ &\times\; \Bigg\{ -\lim_{\tau\to0}\int^{\infty}_{\nu_n}\frac{\done k_+}{k_+}\, \mathcal{R}(k_-,k_+,\tau) +\lim_{\tau\to0}\int^{\infty}_{0}\frac{\done k_+}{k_+}\, \mathcal{R}(k_-,k_+,\tau) -\lim_{\tau\to0}\int^{\infty}_{\nu_\nbar}\frac{\done k_-}{k_-}\, \mathcal{R}(k_-,k_+,\tau) \Bigg\}\,, \end{split} \end{equation} where in the last step we reconvert the logarithms into their integral form and employ $\mathcal{R}(k_-,k_+,\tau)$ to regulate their possibly singular behaviour in the limit $k_{\pm}\to 0$. Comparing the above expressions with Eq.~\eqref{eq:def:asyexp:c0r:at:omega:nured:diff}, we observe that terms containing powers of the auxiliary scale $\nu_{n(\nbar)}$ take the same form in Eqs.~\eqref{eq:reexp:sc1} and \eqref{eq:reexp:scbar1} and Eq.~\eqref{eq:def:asyexp:c0r:at:omega:nured:diff}, and hence cancel upon combination. Similarly, the dependences of the integral on the auxiliary scales through their boundaries in Eqs.~\eqref{eq:reexp:sc1}-\eqref{eq:reexp:sc:scbar:log} can be assimilated in their entirety by combining them with the corresponding integrals in Eq.~\eqref{eq:def:asyexp:c0d:at:omega:nured:diff}. Therefore, we arrive at, \begin{align}\label{eq:def:c0:cbar0:ns} \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|^{\NSmeth}_{c\bar{c}}\, =\, \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|^{\NSmeth}_{c0}\, +\, \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|^{\NSmeth}_{\bar{c}0}\,, \end{align} where % \begin{align} % \label{eq:def:c0:ns} % \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|^{\NSmeth}_{c0}\, % =\,& % \theta\left(\omega-\sigma \right)\, %\sum_{\eta=0}^{\omega-\sigma }\, %\frac{{F}^{(\alpha_n+\eta)}_{i/n,\beta_n}\left(m_H e^{-Y_H}\right)\,{F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)}{\eta!\, (\omega-\rho)!}\, %\lim_{\tau\to0} % \int^{\infty}_{0} % \frac{\done k_+}{k_+} % \left(1-\frac{\delta_{\omega}^{\sigma+\eta}}{2}\right) % \, %\nonumber\\ %&\times %\mathcal{R}(k_-,k_+,\tau)\, % (k_+)^{\sigma-\omega+\eta} \, % ,\\ % \label{eq:def:cbar0:ns} % \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|^{\NSmeth}_{\bar{c}0}\, % =\,& %\theta\left(\omega-\rho\right)\, % \sum_{\lambda=0}^{\omega-\rho}\, %\frac{{F}^{(\alpha_n+\omega-\sigma)}_{i/n,\beta_n}\left( m_H e^{-Y_H}\right) {F}^{(\alpha_\nbar+\lambda)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)}{\lambda!(\omega-\sigma)! }\, %\lim_{\tau\to0}\, % \int^{\infty}_{0}\, % \frac{\done k_-}{k_-}\, % \left(1-\frac{\delta_{\omega}^{\rho+\lambda}}{2}\right)\, % \nonumber\\ %&\times %\mathcal{R}(k_-,k_+,\tau)\, % (k_-)^{\rho-\omega+\lambda}\,. %\end{align} \begin{equation}\label{eq:def:c0:ns} \begin{split} \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|^{\NSmeth}_{c0}\, =\,& \theta\left(\omega-\sigma\right)\, \sum_{\eta=0}^{\omega-\sigma}\, \sum_{\lambda=0}^{\omega-\rho}\, \frac{{F}^{(\alpha_n+\eta)}_{i/n,\beta_n}\left(m_H e^{-Y_H}\right)\, {F}^{(\alpha_\nbar+\lambda)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)} {\eta!\,\lambda!}\\ &\hspace*{30mm}\times\, \lim_{\tau\to0}\int^{\infty}_{0}\frac{\done k_+}{k_+} \left(1-\frac{\delta_{\omega}^{\sigma+\eta}}{2}\right)\, \mathcal{R}(k_-,k_+,\tau)\,(k_+)^{\sigma-\omega+\eta}\, \delta^{\omega}_{\lambda+\rho}\,,\\ \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|^{\NSmeth}_{\bar{c}0}\, =\,& \theta\left(\omega-\rho\right)\, \sum_{\eta=0}^{\omega-\sigma}\, \sum_{\lambda=0}^{\omega-\rho}\, \frac{{F}^{(\alpha_n+\eta)}_{i/n,\beta_n}\left( m_H e^{-Y_H}\right) {F}^{(\alpha_\nbar+\lambda)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)} {\eta!\,\lambda!}\\ &\hspace*{30mm}\times\, \lim_{\tau\to0}\int^{\infty}_{0}\frac{\done k_-}{k_-} \left(1-\frac{\delta_{\omega}^{\rho+\lambda}}{2}\right)\, \mathcal{R}(k_-,k_+,\tau)\,(k_-)^{\rho-\omega+\lambda}\, \delta^{\omega}_{\eta+\sigma}\,. \end{split} \end{equation} Here, we have divided $\widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\big|^{\NSmeth}_{c\bar{c}}$ into two pieces, $\widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\big|^{\NSmeth}_{c0}$ and $\widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\big|^{\NSmeth}_{\bar{c}0}$, inheriting the structure from Eq.~\eqref{eq:def:asyexp:c0d:at:omega:nured:diff}. At variance with Eq.~\eqref{eq:def:asyexp:c0d:at:omega:nured:diff}, however, additional factors $\delta_{\omega}^{\sigma+\eta}$ and $\delta_{\omega}^{\rho+\lambda}$ are present in the integrands now, induced by the unbounded integrals of Eq.~\eqref{eq:reexp:sc:scbar:log}. During the derivation, we have evenly distributed these terms into the $n$-collinear and $\nbar$-collinear sectors symmetrically, incurring a factor $\tfrac{1}{2}$ in Eq.~\eqref{eq:def:c0:ns}. Alternative assignments are in principle possible, which may impact the expressions in the individual sectors but will leave the sum in Eq.~\eqref{eq:def:c0:cbar0:ns} invariant. Equipped with the collinear functions of Eq.~\eqref{eq:def:asyexp:c:at:omega:nured} and the subtrahends of Eq.~\eqref{eq:def:c0:ns}, we are now able to re-express the interior contribution $\widetilde{\mathcal{I}}^{\rho,\sigma }_{[\kappa],\{\alpha,\beta\} }$ as follows, \begin{align} \label{eq:def:asyexp:central:power:omega:rap} \widetilde{\mathcal{I}}^{\rho,\sigma }_{[\kappa],\{\alpha,\beta\}} =\, \sum^{\infty}_{\omega=\rho} \left(\qT^2\right)^{\omega} \left[\widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|_{c} - \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|^{\NSmeth}_{c0}\right] + \sum^{\infty}_{\omega=\sigma} \left(\qT^2\right)^{\omega} \left[\widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|_{\bar{c}} - \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|^{\NSmeth}_{\bar{c}0}\right]. \end{align} Herein, we only show the expressions in the NS scheme for brevity, which can be straightforwardly converted into the FS ones through Eq.~\eqref{eq:def:ns:fs:trans}. Referring back to Eq.~\eqref{eq:def:asyexp:central:power:omega}, we have now found a formulation in which the individual terms on the r.h.s.\ of Eq.~\eqref{eq:def:asyexp:central:power:omega:rap} are free of any dependence on the auxiliary scales $\nu_{n(\nbar)}$ along the integration path. However, in return, they are now subject to the choice of rapidity regularisation scheme implemented through $\mathcal{R}(k_-,k_+,\tau)$. As will be discussed in Secs.~\ref{sec:app:prap} and \ref{sec:app:exp}, the regulator $\mathcal{R}(k_-,k_+,\tau)$ also depends on scales $\tilde{\nu}_n$ and $\tilde{\nu}_\nbar$ in practice, which bears resemblance to those in Eq.~\eqref{eq:def:col-n:soft:col-nbar:cutoff} and can effectively concentrate the integrand in each sector onto its intrinsic domain, akin to the conventional dimensional regularisation~\cite{tHooft:1972tcz}. % %<backup> %Furthermore, in eq.~\eqref{eq:def:asyexp:central:power:omega:rap}, only the collinear sectors together with their overlapping subtrahends are present. Nevertheless, this paper avoids concluding the complete irrelevance of the soft contributions during the decomposition of $ \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }$. At this point, it merits reminding that during the analysis of the momentum space expansion in Sec.~\ref{sec:asyexp:qT:mom}, the soft mode is related to the transitional region in terms of the logarithmic terms in eq.~\eqref{eq:def:asyexp:s:mom1}, which afterwards conducts the transformation in eq.~\eqref{eq:reexp:sc:scbar:log} and in turn leads to the appearance of the factors $(\delta_{\omega}^{\sigma+\eta}/2)$ and $(\delta_{\omega}^{\rho+\lambda}/2)$ in eq.~\eqref{eq:def:c0:ns}. Those two factors differ the integrands in the subtraction sectors from those of the collinear functions in the soft limit and thus indicate the existence of a type of standalone contribution stemming from the moderate rapidity area. However, it is worth noting that, as characterised by $(\delta_{\omega}^{\sigma+\eta}/2)$ and $(\delta_{\omega}^{\rho+\lambda}/2)$, this kind of contribution can survive only if the $k_{\pm}$-integrals in eqs.~\eqref{eq:def:c0:ns} become dimensionless, which overlaps with the soft function of eq.~\eqref{eq:def:s:fs:rap} in part but omits those with the non-vanishing mass dimensions. % % Finally, we can now analyse the scaling of $k_{\pm}$ in each sector on the r.h.s.\ of Eq.~\eqref{eq:def:asyexp:central:power:omega:rap}. Since the collinear functions here are derived by extrapolating the lower boundaries of Eq.~\eqref{eq:def:asyexp:c:mom:at:omega} and Eq.~\eqref{eq:def:asyexp:cbar:mom:at:omega}, the integration variables in Eq.~\eqref{eq:def:asyexp:c:at:omega:nured} observe the same scaling rule as those in momentum space. More explicitly, we have $k_+\sim\mathcal{O}(1)$ and $k_-\sim\mathcal{O}(\qT^2/m_H)$ for the $n$-collinear element and $k_+\sim\mathcal{O}(\qT^2/m_H)$ and $k_-\sim\mathcal{O}(1)$ in the $\nbar$-collinear case. \changed{ To determine the scaling in the subtraction terms of Eq.~\eqref{eq:def:c0:ns}, it merits noting that the integration variables $k_{\pm}$ therein have been both expanded in the arguments of ${F}_{i/n,\beta_n}$ and ${F}_{j/\nbar,\beta_\nbar}$ and also that the function ${F}_{j/\nbar,\beta_\nbar}$ (${F}_{i/n,\beta_n}$) in the ``$c0$" (``$\bar{c}0$") sector observes the same pattern as that in the $n$-($\nbar$-)collinear contribution of Eq.~\eqref{eq:def:asyexp:c:at:omega:nured}. Therefore, we are capable of interpreting the variables $k_{\pm}$ in Eq.~\eqref{eq:def:c0:ns} from the dual scaling---one first of all expands the integrand with the collinear scaling and fixes the $\omega$th-power correction, and then apply a second power expansion in line with soft scaling $k_{\pm}\sim\mathcal{O}(\qT)$, retaining all contributions below or equal to the $(2\omega)$th-power. } %The subtraction terms in Eq.~\eqref{eq:def:c0:ns}, %due to the facts that the integration variables $k_{\pm}$ therein %have been both expanded in the arguments of %${F}_{i/n,\beta_n}$ and ${F}_{j/\nbar,\beta_\nbar}$ %and also that either ${F}_{i/n,\beta_n}$ or %${F}_{j/\nbar,\beta_\nbar}$, respectively, is always synchronised %with that in the collinear function, %on the other hand, allows to interpret the variables $k_{\pm}$ in %the dual scaling---one first of all expands the integrand with %the collinear scaling and fixes the $\omega$th-power correction, %which is followed by a posterior power expansion in accordance %with the soft scaling $k_{\pm}\sim\mathcal{O}(\qT)$ and the retention %of all contributions below or equal to the $(2\omega)$th-power. \begin{figure}[h!] \centering \begin{subfigure}{0.49\textwidth} \centering \includegraphics[width=.6\linewidth, height=0.4\linewidth]{Plots/Soft_PowerCounting_At_NkLP_Naive.pdf} \caption{Subtrahends in the soft scaling} \label{fig:zbsub:soft} \end{subfigure} \begin{subfigure}{0.49\textwidth} \centering \includegraphics[width=.6\linewidth, height=0.4\linewidth]{Plots/Soft_PowerCounting_At_NkLP_Generic.pdf} \caption{Subtrahends in the dual scaling} \label{fig:zbsub:duo} \end{subfigure} \caption{ Organisation of zero-bin subtrahends in different scalings. Every point in the map stands for a index-pair $(\lambda,\eta)$ in Eq.~\eqref{eq:def:c0:ns} which characterises the subtraction procedure entailed by the expansion of $\widetilde{\mathcal{I}}^{\lambda,\eta}_{[\kappa],\{\alpha,\beta\}}$ with integer $\lambda,\eta\ge -1$ in the small \qT~domain. As examples, the red stars highlight the subleading (\NLP) power corrections, the blue triangles represent the sub-subleading (\NNLP) ones, and the green dots indicate the sub-sub-subleading (\NNNLP) ones. } \label{fig:zbsub:scalings} \end{figure} It should be emphasised that at a lower power accuracy, the dual scaling can be reduced to the soft-only one especially in the case $\rho=\sigma=\chi$ with integer $\chi\ge -1$, which however does not hold in general. As an example, Fig.\ 1 illustrates the case $\chi=-1$, which is the minimum of $\chi$ allowed by the squared amplitudes in Eq.~\eqref{eq:msq} and thus concerns the leading power approximation in the small \qT~domain. We observe that, on the lowest level, both of schemes consist of the origin $\lambda=\eta=-1$ and thus can be considered to be equivalent here. However, with the power accuracy growing, the soft scaling forces the indices $\lambda$ and $\eta$ to align along the diagonals, whereas the dual scaling organises the indices of the zero-bin subtrahend along rectangular edges, clearly separating the two. Those distinct patterns can subsequently evaluate to different zero-bin subtrahends for general choices of rapidity regulators, which therefore defies our interpretation of the integration variables of Eq.~\eqref{eq:def:c0:ns} in a purely soft scaling prescription. In order to systematically implement these scaling rules, we introduce the power expansion operator $\widehat{\mathbf{T}}_{i}^{(\omega)}$, with the subscript $i$ running over the sectors $\{c,\bar{c},s\}$, acting on the object following it and projecting out the contribution at the $\omega$th-power in line with the scalings indicated by $i$. In this way, the components of Eq.~\eqref{eq:def:asyexp:central:power:omega:rap} can be recast into, \begin{equation}\label{eq:def:asyexp:c:at:omega:nured:Texp} \begin{split} \left(\qT^2\right)^{\omega}\, \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|_{c} \, &=\, \lim_{\tau\to0}\,\int^{\tilde{k}^{\mathrm{max}}_+}_{0}\, \frac{\done k_+}{k_+}\, \mathcal{R}(k_-,k_+,\tau)\, \widehat{\mathbf{T}}_{c}^{(\omega)}\, I^{ \rho,\sigma}_{[\kappa],\{\alpha,\beta\}}\,, \\ \left(\qT^2\right)^{\omega}\, \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|_{\bar{c}} \, &=\, \lim_{\tau\to0}\,\int^{\frac{\qT^2}{\tilde{k}^{\mathrm{min}}_+}}_{0}\, \frac{\done k_-}{k_-}\, \mathcal{R}(k_-,k_+,\tau)\, \widehat{\mathbf{T}}_{\bar{c}}^{(\omega)}\, I^{ \rho,\sigma}_{[\kappa],\{\alpha,\beta\}}\,, \end{split} \end{equation} and \begin{equation}\label{eq:def:c0:ns:Texp} \begin{split} \left(\qT^2\right)^{\omega}\, \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|_{c0} \, & =\, \theta\left(\omega-\sigma \right) \lim_{\tau\to0}\int^{\infty}_{0} \frac{\done k_+}{k_+}\; \mathcal{R}(k_-,k_+,\tau) \sum_{\overline{\omega}=(\rho+\sigma) }^{2\omega} \left(1-\frac{\delta_{\overline{\omega}}^{2\omega}}{2}\right) \widehat{\mathbf{T}}_{s}^{(\overline{\omega})} \widehat{\mathbf{T}}_{c}^{(\omega)} I^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\}}\,,\\ \left(\qT^2\right)^{\omega}\, \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|_{\bar{c}0} \, & =\, \theta\left(\omega-\rho \right) \lim_{\tau\to0}\int^{\infty}_{0} \frac{\done k_-}{k_-}\; \mathcal{R}(k_-,k_+,\tau) \sum_{\overline{\omega}=(\rho+\sigma) }^{2\omega} \left(1-\frac{\delta_{\overline{\omega}}^{2\omega}}{2}\right) \widehat{\mathbf{T}}_{s}^{(\overline{\omega})} \widehat{\mathbf{T}}_{\bar{c}}^{(\omega)} I^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\}}\,, \end{split} \end{equation} where $I^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\}}$ is the integrand of $\widetilde{\mathcal{I}}^{ \rho,\sigma}_{[\kappa],\{\alpha,\beta\}}$ defined in Eq.~\eqref{eq:def:I:central}, \begin{align}\label{eq:def:subjt} I^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\}}\equiv\, (k_-)^{\rho}\,(k_+)^{\sigma}\, {F}^{(\alpha_n)}_{i/n,\beta_n}\left(k_++m_He^{-Y_H}\right)\, {F}^{(\alpha_\nbar)}_{j/\nbar,\beta_\nbar}\left(k_-+m_He^{+Y_H}\right)\,. \end{align} We note that after the re-arrangements of Eqs.~\eqref{eq:def:asyexp:c:at:omega:nured:diff}-\eqref{eq:id:mom:rsp} and Eqs.~\eqref{eq:reexp:sc1}-\eqref{eq:reexp:sc:scbar:log}, the results in Eqs.~\eqref{eq:def:asyexp:c:at:omega:nured:Texp}-\eqref{eq:def:c0:ns:Texp} present a form that is distinct from that observed Eqs.~\eqref{eq:def:asyexp:c:mom:at:omega}-\eqref{eq:def:asyexp:cbar:mom:at:omega} as well as Eqs.~\eqref{eq:def:asyexp:cs:mom:int}-\eqref{eq:def:asyexp:cbars:mom:int} obtained via the momentum cutoffs $\nu_n$ and $\nu_\nbar$. This is relevant in particular for the ``$sc$" and ``$s\bar{c}$" sectors in Eqs.~\eqref{eq:def:asyexp:cs:mom:int}-\eqref{eq:def:asyexp:cbars:mom:int}, despite hybrid scaling having been used in the transitional range. As illustrated in Eq.~\eqref{eq:def:asyexp:s:mom1}, the resulting coefficient $\widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\big|_{t}$ invokes only the integrands at the same power accuracy once the scaling for the integration variable is given. Contrarily, the situation in Eq.~\eqref{eq:def:c0:ns:Texp} is quite different, where, after applying the soft scaling, the results $\widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\big|_{c0}$ and $\widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\big|_{\bar{c}0}$ comprise not only corrections at the $\omega$th-power, but also those on a lower level. In order to interpret this structural difference, it merits recalling that in deriving Eqs.~\eqref{eq:def:asyexp:c:mom:at:omega} and \eqref{eq:def:asyexp:cbar:mom:at:omega} as well as Eqs.~\eqref{eq:def:asyexp:cs:mom:int} and \eqref{eq:def:asyexp:cbars:mom:int} we have introduced a set of dynamic regions, see Eq.~\eqref{eq:def:col-n:soft:col-nbar:cutoff}, such that within these restricted phase space domains the assigned scalings are always effective before and after the phase space integration. However, in calculating the subtrahends in Eq.~\eqref{eq:def:c0:ns:Texp}, in particular after the combination with Eqs.~\eqref{eq:reexp:sc1}-\eqref{eq:reexp:sc:scbar:log}, all boundaries that separate the different scalings of the integration variables cancel out. As a result, the ``$c0$" and ``$ \bar{c}0$" expressions of Eq.~\eqref{eq:def:c0:ns:Texp} mainly comprise contributions from the rapidity extremities $k_{\pm}\to\pm0$, correlated to the same positions of the collinear functions in Eq.~\eqref{eq:def:asyexp:c:at:omega:nured:Texp}, rather than emphasising any integration segments in the physical domain. In light of this, the scaling laws implemented in Eq.~\eqref{eq:def:c0:ns:Texp} should be conceived more of a prescription guiding us to organise the zero-bin subtrahends in order to subdue any unphysical asymptotic behaviour in the collinear sectors and averting the possibility of these sectors generating any non-trivial remainders for the resulting power series. It is worth noting that the integrands in Eq.~\eqref{eq:def:c0:ns:Texp} appear to contradict the homogeneity condition from the method of expansion by regions~\cite{Beneke:1997zp,Smirnov:1998vk,Smirnov:1999bza, Smirnov:2002pj,Jantzen:2011nz}. In this method, the asymptotic behaviour of the Feynman or phase space integrals is associated with a set of regions along the integration path. From this one is able to expand the integrands before completing the integration and at a given power precision, the resulting power coefficients only concern the expanded integrands of the same power accuracy, more specifically, \begin{align}\label{eq:def:asyexp:homoexp} \widetilde{\mathcal{F}}^{(\omega)}\sim \sum_{i}\int\done\Phi\, \widehat{\mathbf{T}}_{i}^{(\omega)}\,f\,, \end{align} where $\widetilde{\mathcal{F}}^{(\omega)}$ denotes the $\omega$th term in the power series, with $f$ standing for a given integrand and $\Phi$ encoding a group of integration variables. In this paper, such a one-to-one correspondence between the power accuracy of the integrands and that of $\widetilde{\mathcal{F}}^{(\omega)}$ will be referred to as the homogeneity of the asymptotic expansion hereafter. On the contrary, a region analysis where the dimensional regulator uniquely governs the divergences incurred by the reduced integrands, such homogeneity is found to generally hold in a variety of kinematical limits, such as the off-shell large-momentum expansion and the large-mass limits with either an internal or external heavy parton~\cite{Smirnov:2002pj}. The reason comes in part from the fact that the overlapping sectors for those asymptotic regimes, according to \cite{Jantzen:2011nz}, admit the unbounded integrals over the multiple-expanded integrands, which, using dimensional regularisation, are all scaleless and thus vanish. In principle, if the homogeneity is also desired for the small~\qT\ expansion, one can embed a special group of rapidity operators into Eq.~\eqref{eq:def:c0:ns:Texp}, such as the analytic \cite{Becher:2010tm,Becher:2011dz} and pure rapidity \cite{Ebert:2018gsn,Moult:2019vou} cases, from which, mimicking the dimensional regulator, the integrals in the zero-bin subtrahends of Eq.~\eqref{eq:def:c0:ns:Texp} become scaleless and are thus eliminated. Subsequently, homogeneity is restored in the small~\qT\ expansion and the power coefficients are thereby recast as, \begin{align} \label{eq:def:asyexp:central:power:omega:rap:hom} \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\, =\, \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|^{\langle\mathrm{hom.rap.}\rangle}_{c}\, +\, \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}} \Bigg|^{\langle\mathrm{hom.rap.}\rangle}_{\bar{c}}\,. \end{align} This work will dub this set of rapidity regulators the homogeneous ones, as labeled in the superscripts above. However, the above form is not generic. For instance, once the exponential regulator \cite{Li:2016axz,Li:2016ctv} is put in place, both the ``$c0$" and ``$\bar{c}0$" sectors in Eq.~\eqref{eq:def:c0:ns:Texp} will make non-trivial and indispensable contributions, from which all unphysical singularities generated in the collinear sectors of Eq.~\eqref{eq:def:asyexp:c:at:omega:nured:Texp} can be eliminated at each power, according to Eq.~\eqref{eq:def:asyexp:c:cbar:diff}. In this sense, the decomposition in Eqs.~\eqref{eq:def:asyexp:central:power:omega:rap:hom} can only be appropriate for the asymptotic expansion with a homogeneous regulator, while the generalised recipe, that will hold on a generic choice of rapidity regulators, is presented in Eq.~\eqref{eq:def:asyexp:central:power:omega:rap}. \subsubsection{Comparison with existing results} \label{sec:asyexp:comp} We will now confront the zero-bin subtrahend derived in Eqs.~\eqref{eq:def:asyexp:central:power:omega:rap}-\eqref{eq:def:c0:ns:Texp} with those proposed in the literature. At \LP, the zero-bin contribution at NLO involves only the master integral $\widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}$ with $\rho=\sigma=\omega=-1$ in the process $pp\to H+X$, and it has been demonstrated in~\cite{Manohar:2006nz,Idilbi:2007yi, Idilbi:2007ff,Chiu:2009yx,Echevarria:2011epo} that the zero-bin subtrahend can be constructed by taking the soft limit of the integrand. It follows that, \begin{align}\label{eq:def:c0:cbar0:ns:lp} \frac{1}{\qT^2} \widetilde{\mathcal{G}}^{-1,-1,(-1)}_{[\kappa],\{\alpha,\beta\} }\Bigg|^{\NSmeth}_{c\bar{c}} \xRightarrow[]{\text{~~soft~~}} \lim_{\tau\to0}\,\int^{\infty}_{0}\, \frac{\done k_-}{k_-}\,\mathcal{R}(k_-,k_+,\tau)\, \frac{ {F}^{(\alpha_n)}_{i/n,\beta_n}\left(m_He^{-Y_H}\right) {F}^{(\alpha_\nbar)}_{j/\nbar,\beta_\nbar}\left(m_He^{+Y_H} \right) } {k_-\,k_+}\,. \end{align} This result can also be reproduced from Eq.~\eqref{eq:def:c0:ns:Texp}. At \LP, the repeated application of the expansion operators in Eq.~\eqref{eq:def:c0:ns:Texp} does not produce any power of the integration variables $k_{\pm}$ and therefore yields the same powers of $k_\pm$ as that in Eq.~\eqref{eq:def:c0:cbar0:ns:lp}. Moreover, owing to the relation $2\omega=\overline{\omega}=-2$, the $\delta$-functions in Eq.~\eqref{eq:def:c0:ns:Texp} are both contributing a factor of $(1/2)$ from each sector, which add up to unity after combining the results. This thus leads to the exact same expression of Eq.~\eqref{eq:def:c0:cbar0:ns:lp}. An alternative scheme to calculate the zero-bin subtraction up to \NLP was proposed in \cite{Inglis-Whalen:2022vyn, Inglis-Whalen:2021bea}. In this method, the asymptotic behaviour of the small \qT~regime is assumed to be entirely governed by the $n$- and $\nbar$-collinear momenta. Subsequently, in order to remove the redundant overlapping contributions, each collinear ingredient is expanded in accordance with the scaling of the other one in the opposite direction and then their sum is averaged, more specifically, \begin{equation}\label{eq:def:c0:cbar0:ns:oppcol} \begin{split} \left(\qT^2\right)^{\omega}\, \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|^{\NSmeth}_{c\bar{c}}\, &\xRightarrow[]{\text{~~opp.col.~~}}\, \frac{\theta\left(\omega-\rho \right)\theta\left(\omega-\sigma\right)}{2}\, \lim_{\tau\to0}\,\int^{\infty}_{0}\, \frac{\done k_+}{k_+}\,\mathcal{R}(k_-,k_+,\tau)\, \\ &\hspace*{20mm}\times\; \Bigg\{ \left( \sum_{\overline{\omega}=\sigma}^{\omega}\, \widehat{\mathbf{T}}_{\bar{c}}^{(\overline{\omega})} \right) \widehat{\mathbf{T}}_{c}^{(\omega)} + \left( \sum_{\overline{\omega}=\rho}^{\omega}\, \widehat{\mathbf{T}}_{c}^{(\overline{\omega})} \right) \widehat{\mathbf{T}}_{\bar{c}}^{(\omega)} \\ &\hspace*{28mm}{} + \widehat{\mathbf{T}}_{c}^{(\omega)}\, \left( \sum_{\overline{\omega}=\sigma}^{\omega-1} \widehat{\mathbf{T}}_{\bar{c}}^{(\overline{\omega})} \right) + \widehat{\mathbf{T}}_{\bar{c}}^{(\omega)} \left( \sum_{\overline{\omega}=\rho}^{\omega-1}\, \widehat{\mathbf{T}}_{c}^{(\overline{\omega})} \right) \Bigg\}\; I^{\rho,\sigma}_{[\kappa], \{\alpha,\beta\}} \,. \end{split} \end{equation} Using this result to calculate $I^{-1,-1 }_{[\kappa],\{\alpha,\beta\}}$, we observe that only the first two terms in the curly brackets can give non-vanishing contributions at \LP as the range of summation in the last two terms is more restricted. In addition, due to the fact that the product of two collinear expansion operators in the opposite collinear directions is equivalent to one single soft expansion operator in this case, Eq.~\eqref{eq:def:c0:cbar0:ns:oppcol} evaluates to the identical expression to that in Eq.~\eqref{eq:def:c0:cbar0:ns:lp}. % This can be shown explicitly by considering % \begin{align} % & \widehat{\mathbf{T}}_{c}^{(-1)} \frac{ {F}^{(\alpha_n)}_{i/n,\beta_n}\left(k_++m_H e^{-Y_H}\right) % {F}^{(\alpha_\nbar )}_{j/\nbar,\beta_\nbar}\left(k_-+m_H e^{+Y_H}\right)}{k_+ k_-}= \frac{ {F}^{(\alpha_n)}_{i/n,\beta_n}\left(k_++m_H e^{-Y_H}\right) % {F}^{(\alpha_\nbar )}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)}{k_+ k_-}+....\\ % & \widehat{\mathbf{T}}_{\bar{c}}^{(-1)} \frac{ {F}^{(\alpha_n)}_{i/n,\beta_n}\left(k_++m_H e^{-Y_H}\right) % {F}^{(\alpha_\nbar )}_{j/\nbar,\beta_\nbar}\left(k_-+m_H e^{+Y_H}\right)}{k_+ k_-}= \frac{ {F}^{(\alpha_n)}_{i/n,\beta_n}\left( m_H e^{-Y_H}\right) % {F}^{(\alpha_\nbar )}_{j/\nbar,\beta_\nbar}\left(k_-+m_H e^{+Y_H}\right)}{k_+ k_-}+....\\ % & \widehat{\mathbf{T}}_{s}^{(-1)} \frac{ {F}^{(\alpha_n)}_{i/n,\beta_n}\left(k_++m_H e^{-Y_H}\right) % {F}^{(\alpha_\nbar )}_{j/\nbar,\beta_\nbar}\left(k_-+m_H e^{+Y_H}\right)}{k_+ k_-}= \frac{ {F}^{(\alpha_n)}_{i/n,\beta_n}\left( m_H e^{-Y_H}\right) % {F}^{(\alpha_\nbar )}_{j/\nbar,\beta_\nbar}\left( m_H e^{+Y_H}\right)}{k_+ k_-}+.... % \end{align} At \NLP, all terms of Eq.~\eqref{eq:def:c0:cbar0:ns:oppcol} contribute to the zero-bin subtraction. While in the first two terms in the curly brackets the \NLP collinear sectors have been expanded in line with the counting rule in the opposite direction, the last two terms recover the power corrections that did not contribute to the \LP result, but re-enter the zero-bin subtraction procedure here. Thus, retaining all terms up to \NLP, this yields, \begin{equation}\label{eq:def:c0:cbar0:ns:nlp} \begin{split} \widetilde{\mathcal{G}}^{-1,-1,(0)}_{[\kappa],\{\alpha,\beta\}}\Bigg|^{\NSmeth}_{c\bar{c}}\, \xRightarrow[]{\text{~~opp.col.~~}} \,& \theta\left(\omega-\rho \right)\, \theta\left(\omega-\sigma \right)\, \lim_{\tau\to0}\,\int^{\infty}_{0}\, \frac{\done k_+}{k_+}\,\mathcal{R}(k_-,k_+,\tau)\, \bigg\{ 1\,+\,\frac{1}{k_-}\,+\frac{1}{k_+} \bigg\}\, \\ &\hspace*{40mm}\times\; {F}^{(\alpha_n)}_{i/n,\beta_n}\left(m_He^{-Y_H}\right)\, {F}^{(\alpha_\nbar)}_{j/\nbar,\beta_\nbar}\left( m_He^{+Y_H} \right)\,. \end{split} \end{equation} This result agrees with the expectation from the dual scaling. Please note, \LP-like terms have now entered the subtraction term at \NLP, constituting the inhomogeneity we alluded to earlier. More explicitly, substituting the integrand $I^{-1,-1 }_{[\kappa],\{\alpha,\beta\}}$ into Eq.~\eqref{eq:def:c0:ns:Texp}, we obtain, \begin{equation}\label{eq:def:c0:ns:Texp:nlp} \begin{split} \widetilde{\mathcal{G}}^{-1,-1,(0)}_{[\kappa],\{\alpha,\beta\}}\Bigg|_{c0} \, =\,& \theta\left(\omega-\sigma \right)\, \lim_{\tau\to0}\,\int^{\infty}_{0}\, \frac{\done k_+}{k_+}\,\mathcal{R}(k_-,k_+,\tau)\, \bigg\{ \frac{1}{2}\,+\,\frac{1}{k_+} \bigg\}\, {F}^{(\alpha_n)}_{i/n,\beta_n}\left(m_He^{-Y_H}\right)\, {F}^{(\alpha_\nbar)}_{j/\nbar,\beta_\nbar}\left( m_He^{+Y_H}\right), \\ \widetilde{\mathcal{G}}^{-1,-1,(0)}_{[\kappa],\{\alpha,\beta\}}\Bigg|_{\bar{c}0} \, =\,& \theta\left(\omega-\rho \right)\, \lim_{\tau\to0}\,\int^{\infty}_{0}\, \frac{\done k_-}{k_-}\,\mathcal{R}(k_-,k_+,\tau)\, \bigg\{ \frac{1}{2}\,+\,\frac{1}{k_-} \bigg\}\, {F}^{(\alpha_n)}_{i/n,\beta_n}\left(m_He^{-Y_H}\right)\, {F}^{(\alpha_\nbar)}_{j/\nbar,\beta_\nbar}\left( m_He^{+Y_H}\right). \end{split} \end{equation} Recalling that additional constraints on the exponents $\rho$ and $\sigma$ have already been imposed in the definition of the power series in Eq.~\eqref{eq:def:asyexp:central:power:omega:rap}, combining both contributions above precisely reproduces the results of Eq.~\eqref{eq:def:c0:cbar0:ns:nlp}. Furthermore, even though Eq.~\eqref{eq:def:c0:cbar0:ns:nlp} is obtained by summarising the asymptotic properties of the \NLP ingredients in \cite{Inglis-Whalen:2022vyn, Inglis-Whalen:2021bea}, it is very interesting to note that Eq.~\eqref{eq:def:c0:cbar0:ns:nlp} is in fact still useful in organising the overlap removal for N$^2$LP and beyond. To see this, we note that the collinear expansion operators $\widehat{\mathbf{T}}_{c} $ and $\widehat{\mathbf{T}}_{\bar{c}}$ commute. Hence, we can drop the factor of $\tfrac{1}{2}$ and recast the r.h.s.\ of Eq.~\eqref{eq:def:c0:cbar0:ns:nlp} below, \begin{equation}\label{eq:def:c0:cbar0:ns:oppcol2} \begin{split} \left(\qT^2\right)^{\omega}\, \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}}\Bigg|^{\NSmeth}_{c\bar{c}}\, \xRightarrow[]{\text{~~opp.col.~~}} &\, \theta\left(\omega-\rho \right)\theta\left(\omega-\sigma \right)\, \lim_{\tau\to0}\,\int^{\infty}_{0}\, \frac{\done k_+}{k_+}\,\mathcal{R}(k_-,k_+,\tau)\, \\ &\times \Bigg\{ \widehat{\mathbf{T}}_{\bar{c}}^{(\omega)} \widehat{\mathbf{T}}_{c}^{(\omega)} + \widehat{\mathbf{T}}_{c}^{(\omega)}\, \left( \sum_{\overline{\omega}=\sigma}^{\omega-1}\, \widehat{\mathbf{T}}_{\bar{c}}^{(\overline{\omega})}\, \right) + \widehat{\mathbf{T}}_{\bar{c}}^{(\omega)}\, \left( \sum_{\overline{\omega}=\rho}^{\omega-1}\, \widehat{\mathbf{T}}_{c}^{(\overline{\omega})}\, \right) \Bigg\} I^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\}} \,,\hspace*{-20mm} \end{split} \end{equation} Plugging the expressions of eq.~\eqref{eq:def:subjt} into eq.~\eqref{eq:def:c0:cbar0:ns:oppcol2}, we then obtain, \begin{equation}\label{eq:def:c0:cbar0:ns:oppcol3} \begin{split} \mathrm{r.h.s.~of~eq.~\eqref{eq:def:c0:cbar0:ns:oppcol2}} =&\; \theta\left(\omega-\rho \right) \theta\left(\omega-\sigma \right)\, \lim_{\tau\to0}\, \int^{\infty}_{0}\, \frac{\done k_+}{k_+}\, \mathcal{R}(k_-,k_+,\tau)\\ &\times \Bigg\{ k_-^{\omega}\, k_+^{\omega}\, \frac{ {F}^{(\alpha_n+\omega-\sigma)}_{i/n,\beta_n}\left(m_H e^{-Y_H}\right) }{(\omega-\sigma)!} \frac{ {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right) }{(\omega-\rho)!} \\ &\hspace*{6mm}{} + k_-^{\omega}\, \sum_{\eta=0}^{\omega-\sigma-1 }\, k_+^{\sigma+\eta}\, \frac{ {F}^{(\alpha_n+\eta)}_{i/n,\beta_n}\left(m_H e^{-Y_H}\right)\, {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)} {\eta!\,(\omega-\rho)!}\, \\ &\hspace*{6mm}{} + k_+^{\omega}\, \sum_{\eta=0}^{\omega-\sigma-1 }\, k_-^{\rho +\lambda}\, \frac{ {F}^{(\alpha_n+\omega-\sigma)}_{i/n,\beta_n}\left( m_H e^{-Y_H}\right) {F}^{(\alpha_\nbar+\lambda)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right) }{\lambda!(\omega-\sigma)!}\, \Bigg\}\,. \end{split} \end{equation} Extracting a common factor of $(\qT^2)^{\omega}$ from the curly bracket above, we observe its coincidence with the sum of Eq.~\eqref{eq:def:c0:ns} and thus the equivalence with Eq.~\eqref{eq:def:c0:ns:Texp:nlp}. We will now compare our results with the results obtained through employing the method of expansion by regions~\cite{Beneke:1997zp,Smirnov:1998vk, Smirnov:1999bza,Smirnov:2002pj,Jantzen:2011nz} and focus in particular on the formalism proposed in~\cite{Jantzen:2011nz}. Therein, the mathematical foundation behind the expansion by regions has been discussed via examples for the one-loop integrals in different kinematic limits. Of them, the analysis of the Feynman integrals in the Sudakov limit~\cite{Jantzen:2011nz} is intimately related to the \qT~spectra within the asymptotic regime. Therefore, after appropriate adaptations, the techniques proposed in~\cite{Jantzen:2011nz} can also be exploited to compute the zero-bin subtraction here. In the following, we will elucidate this application. The starting point of the formalism in~\cite{Jantzen:2011nz} is to work out a group of dynamic regions that are able to encompass the entire phase space and also separately accommodate the contributions from all involved scales. In our case, this goal can be accomplished by the dynamic modes presented in Eqs.~\eqref{eq:def:col-n:soft:col-nbar:cutoff}. The next task is to extrapolate the bounded integrals contained in each region so as to remove all auxiliary cutoff scales along the integration paths. This procedure can be illustrated by using the expansion operators introduced in Eqs.~\eqref{eq:def:asyexp:c:at:omega:nured:Texp} and \eqref{eq:def:c0:ns:Texp}, i.e.\ \begin{align} \widetilde{\mathcal{I}}^{\rho,\sigma }_{[\kappa],\{\alpha,\beta\} } = \sum_{\omega} \left[ \int^{\tilde{k}^{\mathrm{max}}_+}_{\nu_n} \widehat{\mathbf{T}}_{c}^{(\omega)}\, + \int^{\nu_n}_{\frac{\qT^2}{\nu_\nbar}}\, \widehat{\mathbf{T}}_{s}^{(\omega)}\, + \int^{\frac{\qT^2}{\nu_\nbar}}_{ \tilde{k}^{\mathrm{min}}_+ }\, \widehat{\mathbf{T}}_{\bar{c}}^{(\omega)} \right]\, \frac{\done k_+}{k_+}\, I^{\rho,\sigma }_{[\kappa],\{\alpha,\beta\} }\,, \end{align} and then extrapolating the integral boundaries $\nu_n$ and $\nu_\nbar$, \begin{equation}\label{eq:def:expbreg:c1} \begin{split} \sum_{\omega_c}\int^{\tilde{k}^{\mathrm{max}}_+}_{\nu_n} \widehat{\mathbf{T}}_{c}^{(\omega_c)} & \rightarrow \lim_{\tau\to0} \left[ \sum_{\omega_c}\int^{\tilde{k}^{\mathrm{max}}_+}_{0} \mathcal{R}\, \widehat{\mathbf{T}}_{c}^{(\omega_c)} - \sum_{\omega_c,\omega_s}\int^{\nu_n}_{\frac{\qT^2}{\nu_\nbar}} \mathcal{R}\, \widehat{\mathbf{T}}_{s}^{(\omega_s)} \widehat{\mathbf{T}}_{c}^{(\omega_c)} - \sum_{\omega_c,\omega_{\bar{c}}}\int^{\frac{\qT^2}{\nu_\nbar}}_{0} \mathcal{R}\, \widehat{\mathbf{T}}_{\bar{c}}^{(\omega_{\bar{c}})} \widehat{\mathbf{T}}_{c}^{(\omega_c)} \right], \\ \sum_{\omega_s}\int^{\nu_n}_{\frac{\qT^2}{\nu_\nbar}} \widehat{\mathbf{T}}_{s}^{(\omega_s)} & \rightarrow \lim_{\tau\to0} \left[ \sum_{\omega_s}\int^{\infty}_{0} \mathcal{R}\, \widehat{\mathbf{T}}_{s}^{(\omega_s)} - \sum_{\omega_c,\omega_s}\int^{\infty}_{\nu_n} \mathcal{R}\, \widehat{\mathbf{T}}_{c}^{(\omega_c)} \widehat{\mathbf{T}}_{s}^{(\omega_s)} - \sum_{\omega_s,\omega_{\bar{c}}}\int^{\frac{\qT^2}{\nu_\nbar}}_{0} \mathcal{R}\, \widehat{\mathbf{T}}_{\bar{c}}^{(\omega_{\bar{c}})} \widehat{\mathbf{T}}_{s}^{(\omega_s)} \right], \\ \sum_{\omega_{\bar{c}}}\int^{\frac{\qT^2}{\nu_\nbar}}_{\tilde{k}^{\mathrm{min}}_+ } \widehat{\mathbf{T}}_{\bar{c}}^{(\omega_{\bar{c}})} & \rightarrow \lim_{\tau\to0} \left[ \sum_{\omega_{\bar{c}}}\int^{\infty}_{ \tilde{k}^{\mathrm{min}}_+ } \mathcal{R}\, \widehat{\mathbf{T}}_{\bar{c}}^{(\omega_{\bar{c}})} - \sum_{\omega_{\bar{c}},\omega_s}\int^{\nu_n}_{\frac{\qT^2}{\nu_\nbar}} \mathcal{R}\, \widehat{\mathbf{T}}_{s}^{(\omega_s)} \widehat{\mathbf{T}}_{\bar{c}}^{(\omega_{\bar{c}})} - \sum_{\omega_c,\omega_{\bar{c}}}\int^{\infty}_{\nu_n} \mathcal{R}\, \widehat{\mathbf{T}}_c^{(\omega_{c})} \widehat{\mathbf{T}}_{\bar{c}}^{(\omega_{\bar{c}})} \right]. \end{split} \end{equation} Therein, in order to render the integrals still well-defined after extrapolating the boundaries, the rapidity regulator $\mathcal{R}$ has been put in place. Since the discussion here is focused on the conservative rapidity regularisation prescription that preserves the expression of $\mathcal{R}$ in all the involved sectors, in writing Eq.~\eqref{eq:def:expbreg:c1}, we pull all regulators $\mathcal{R}$ in front of the expansion operators. We note that the r.h.s.\ of Eq.~\eqref{eq:def:expbreg:c1} still depends on the cutoff scales $\nu_n$ and $\nu_\nbar$. This dependence can be eliminated through the following identity, \begin{equation}\label{eq:def:expbreg:rel:c:s:cbar} \begin{split} \sum_{\omega_c,\omega_{\bar{c}},\omega_s}\int^{\infty}_{0} \mathcal{R}\, \widehat{\mathbf{T}}_{c}^{(\omega_c)} \widehat{\mathbf{T}}_{s}^{(\omega_s)} \widehat{\mathbf{T}}_{\bar{c}}^{(\omega_{\bar{c}})} \rightarrow& \sum_{\omega_c,\omega_s}\int^{\frac{\qT^2}{\nu_\nbar}}_{0} \mathcal{R}\, \widehat{\mathbf{T}}_{s}^{(\omega_s)} \widehat{\mathbf{T}}_{c}^{(\omega_c)} + \sum_{\omega_c,\omega_{\bar{c}}}\int_{\frac{\qT^2}{\nu_\nbar}}^{ \nu_n} \mathcal{R}\, \widehat{\mathbf{T}}_{\bar{c}}^{(\omega_{\bar{c}})} \widehat{\mathbf{T}}_{c}^{(\omega_c)} \\ &{}+ \sum_{\omega_{\bar{c}},\omega_s}\int^{\infty}_{\nu_n} \mathcal{R}\, \widehat{\mathbf{T}}_{s}^{(\omega_s)} \widehat{\mathbf{T}}_{\bar{c}}^{(\omega_{\bar{c}})}\,. \end{split} \end{equation} In its derivation, we have used the commutativity of the power projection operators $\widehat{\mathbf{T}}_{c}$, $\widehat{\mathbf{T}}_{s}$, and $\widehat{\mathbf{T}}_{\bar{c}}$. Combining Eq.~\eqref{eq:def:expbreg:rel:c:s:cbar} with Eq.~\eqref{eq:def:expbreg:c1}, we have, %%%%%%%%% %\footnote{ % This result appears contradicting the calculation in~\cite{Jantzen:2011nz} on the Sudakov form factors, where the propagators in the ensuing Feynman integrals are raised by the power of $\tau$ and the expansion operators act on all those denominators dressed by analytic regulator. However, this kind of conflict is in fact spuriously. In our case, the factors in eq.~\eqref{eq:def:subjt} that are able to undertake the analytic regularization are the light-cone coordinates $k_{\pm}$, which stay still before and after the expansion and therefore permit us to freely move the rapidity regulator forward. } %%%%%%%% %%%%%%%% %%%%%%%% %%%%%%%% %%%%%%%% %%%%%%%% % memo: % If one insists to put the rapidity regulator behind the expansion operators, there exits at least one regularization scheme in which $T_c$ and $T_\cbar$ are not commutative, e,g., $\eta$-regulator. % In this instance, I still can rewrite eq.~\eqref{eq:def:expbreg:rel:c:s:cbar} via eq.~5.14 of~\cite{Jantzen:2011nz} but I do not know how to derive eq.~\eqref{eq:reexp:sc:scbar:log} without introducing adhoc prescriptions. % As far as I understand, implementing $\eta$-regulator can be very flexible and thus ambiguous especially in regards to whether and how the subleading corrections induced by the regulator itself are retained, after all those corrections are not parts of physical integrands %%%%%%%% %%%%%%%% %%%%%%%% %%%%%%%% %%%%%%%% %%%%%%%% \begin{equation}\label{eq:def:asyexp:jantzen} \begin{split} \widetilde{\mathcal{I}}^{\rho,\sigma }_{[\kappa],\{\alpha,\beta\} } =&\; \lim_{\tau\to0} \bigg[ \sum_{\omega_c} \int^{\tilde{k}^{\mathrm{max}}_+}_{0} \mathcal{R}\, \widehat{\mathbf{T}}_{c}^{(\omega_c)}\, + \sum_{\omega_s} \int^{\infty}_{0} \mathcal{R}\, \widehat{\mathbf{T}}_{s}^{(\omega_s)} + \sum_{\omega_{\bar{c}}} \int^{\infty}_{\tilde{k}^{\mathrm{min}}_+} \mathcal{R}\, \widehat{\mathbf{T}}_{\bar{c}}^{(\omega_{\bar{c}})} \\ &\hspace*{10mm}{} - \sum_{\omega_c,\omega_s} \int^{\infty}_{0} \mathcal{R}\, \widehat{\mathbf{T}}_{c}^{(\omega_c)}\, \widehat{\mathbf{T}}_{s}^{(\omega_s)} - \sum_{\omega_c,\omega_{\bar{c}}} \int^{\infty}_{0} \mathcal{R}\, \widehat{\mathbf{T}}_{c}^{(\omega_c)}\, \widehat{\mathbf{T}}_{\bar{c}}^{(\omega_{\bar{c}})} - \sum_{\omega_s,\omega_{\bar{c}}} \int^{\infty}_{0} \mathcal{R}\, \widehat{\mathbf{T}}_{s}^{(\omega_s)}\, \widehat{\mathbf{T}}_{\bar{c}}^{(\omega_{\bar{c}})} \\ &\hspace*{10mm}{} + \sum_{\omega_c,\omega_s,\omega_{\bar{c}}} \int^{\infty}_{0} \mathcal{R}\, \widehat{\mathbf{T}}_{c}^{(\omega_c)}\, \widehat{\mathbf{T}}_{s}^{(\omega_s)}\, \widehat{\mathbf{T}}_{\bar{c}}^{(\omega_{\bar{c}})}\, \bigg]\, \frac{\done k_+}{k_+}\, I^{\rho,\sigma }_{[\kappa],\{\alpha,\beta\} }\,. \end{split} \end{equation} Taking into account the facts that expanding in the collinear scalings following the soft power-projection operator $\widehat{\mathbf{T}}_{s} $ can only result in delta functions as well as that two consecutive expansions in the collinear scalings are equivalent to one single expansion in the soft scaling upon having summed all power contributions, we see that the doubly and triply expanded terms in Eq.~\eqref{eq:def:asyexp:jantzen} are equal to an expansion in the soft scaling. To this end, we obtain, \begin{align}\label{eq:def:asyexp:jantzen:red} \widetilde{\mathcal{I}}^{\rho,\sigma }_{[\kappa],\{\alpha,\beta\}} =&\; \sum_{\omega}\, \lim_{\tau\to0}\, \bigg[ \int^{\tilde{k}^{\mathrm{max}}_+}_{0} \mathcal{R}\, \widehat{\mathbf{T}}_{c}^{(\omega)}\, + \int^{\infty}_{\tilde{k}^{\mathrm{min}}_+} \mathcal{R}\, \widehat{\mathbf{T}}_{\bar{c}}^{(\omega)} - \int^{\infty}_{0} \mathcal{R}\, \widehat{\mathbf{T}}_{s}^{(\omega)} \bigg]\, \frac{\done k_+}{k_+}\, I^{\rho,\sigma }_{[\kappa],\{\alpha,\beta\} }\,. \end{align} Comparing with Eqs.~\eqref{eq:def:asyexp:c:at:omega:nured:Texp} and \eqref{eq:def:c0:ns:Texp}, we observe that the first two terms in Eq.~\eqref{eq:def:asyexp:jantzen:red} and the collinear functions in Eq.~\eqref{eq:def:asyexp:c:at:omega:nured:Texp} are equivalent. To explore the relationship of the third term in Eq.~\eqref{eq:def:asyexp:jantzen:red} and the sum of Eq.~\eqref{eq:def:c0:ns:Texp}, we note that after bringing in the expression in Eq.~\eqref{eq:def:subjt} the soft sector in Eq.~\eqref{eq:def:asyexp:jantzen:red} evaluates to an infinite sum of the unbounded integrals, i.e., \begin{equation} \begin{split} \sum_{\eta,\lambda=0}^{\infty}\, \lim_{\tau\to0}\, \int_0^{\infty}\, \frac{\done k_+}{k_+}\, \mathcal{R}\left(k_-,k_+,\tau\right)\, \frac{k_+^{\sigma+\eta}\, k_-^{\rho+\lambda}}{\eta!\,\lambda!}\, {F}^{(\alpha_n+\eta)}_{i/n,\beta_n}\left(m_H e^{-Y_H}\right)\, {F}^{(\alpha_\nbar+\lambda)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)\,, \end{split} \end{equation} which is exactly equal to the result from Eq.~\eqref{eq:def:c0:ns:Texp} upon summing up all power contributions. Therefore, we can conclude at least the correspondence of Eq.~\eqref{eq:def:asyexp:jantzen:red} and Eqs.~\eqref{eq:def:asyexp:c:at:omega:nured:Texp} and \eqref{eq:def:c0:ns:Texp} on the cumulative level. Notwithstanding, once a power-by-power comparison is being considered between both results, the analysis becomes more subtle. In~\cite{Jantzen:2011nz}, the analytic regulator is applied throughout the calculation of the Sudakov form factors. Implementing this scheme into Eq.~\eqref{eq:def:asyexp:jantzen} (or Eq.~\eqref{eq:def:asyexp:jantzen:red}), the integrals that are expanded in the soft scaling or comprise double or triple expansions all vanish. Then, Eq.~\eqref{eq:def:asyexp:jantzen} and Eq.~\eqref{eq:def:asyexp:jantzen:red} both reduce into the same decomposition we found in Eq.~\eqref{eq:def:asyexp:central:power:omega:rap:hom} induced by the homogeneous regulators. However, if the inhomogeneous regularisation scheme is of one's particular interest, the soft function and the doubly and triply expanded constituents of Eq.~\eqref{eq:def:asyexp:jantzen} can make non-trivial contributions at a given power accuracy, for which an unambiguous counting rule is required in order to produce the correct power coefficient $\widetilde{\mathcal{I}}^{\rho,\sigma,(\omega) }_{[\kappa],\{\alpha,\beta\}}$. % Nevertheless, the discussion in this regard is absent in~\cite{Jantzen:2011nz}. To this end, we have to halt the further comparison here. \subsection{Discussion and extrapolation} \label{sec:asyexp:recap} In the previous subsections, we have carried out the power expansion of the double-differential observable ${\done \sigma_H}/{\done Y_H \done \qT^2}$ in the low \qT~domain. The result reads, \begin{align}\label{eq:asyexp:tot} &\frac{\done \sigma_H}{\done Y_H \done \qT^2} \,=\, \lambda_t^2\, \sum_{\omega,\overline{\omega}}\, \left( {\qT^2} \right)^{\omega+\overline{\omega}}\, \sum_{[\kappa]}\, \sum_{ \{\alpha,\beta\},\rho,\sigma}\, \widetilde{\mathcal{H}}^{ (\omega),\rho,\sigma }_{[\kappa], \{\alpha,\beta\} }\left(m_H,Y_H,s\right) \, \bigg\{ \widetilde{\mathcal{I}}^{ \rho,\sigma,(\overline{\omega}) }_{[\kappa], \{\alpha,\beta\} } \,+\, \Delta\widetilde{\mathcal{I}}^{ \rho,\sigma,(\overline{\omega}) }_{[\kappa], \{\alpha,\beta\} } \bigg\}\,. \end{align} Therein, $\widetilde{\mathcal{H}}^{(\omega),\rho,\sigma }_{[\kappa],\{\alpha,\beta\}}$ is a function of the hard scales $m_H$ and $s$. Its expression has been presented in Eq.~\eqref{eq:asy:mom:c} on a power-by-power basis. $\Delta\widetilde{\mathcal{I}}^{\rho,\sigma,(\overline{\omega}) }_{[\kappa],\{\alpha,\beta\}}$ accounts for the power corrections induced by the boundary conditions of the phase space integral. The results in the $n$-ultra-collinear limit can be extracted from Eqs.~\eqref{eq:asyexp:deltaI:uc}-\eqref{eq:asyexp:deltaI:ec:int}, while those in the $\nbar$-direction can be derived by exchanging the light-cone coordinates in Eqs.~\eqref{eq:def:Gp}-\eqref{eq:asyexp:deltaI:ec:int}, as appropriate. Finally, Eq.~\eqref{eq:asyexp:tot} contains $\widetilde{\mathcal{I}}^{\rho,\sigma,(\overline{\omega})}_{[\kappa],\{\alpha,\beta\}}$ which comprises the contribution from the bulk of the phase space. In Sec.~\ref{sec:asyexp:qT:mom} and Sec.~\ref{sec:asyexp:qT:extrapl}, we made use of two strategies to evaluate the expansion coefficients $\widetilde{\mathcal{I}}^{\rho,\sigma,(\overline{\omega})}_{[\kappa],\{\alpha,\beta\}}$. In Sec.~\ref{sec:asyexp:qT:mom}, owing to the fact that our integration region comprises multiple scales, we re-categorised the integration path via a two of auxiliary cutoff scales, $\nu_n$ and $\nu_\nbar$. A dedicated method is applied for each subregion to perform the expansion within the low \qT~domain. The quoted power series following this approach is illustrated in Eq.~\eqref{eq:def:asyexp:central:power:omega}. Then, in order to pave the way for future investigations of the power expansion at \NNLO and beyond, we recombined the individual terms of Eq.~\eqref{eq:def:asyexp:central:power:omega}, eliminating any dependence on the auxiliary scales. The rearranged expansion coefficients are given in Eq.~\eqref{eq:def:asyexp:central:power:omega:rap}. Equipped therewith, we are able to calculate the power series of ${\done \sigma_H}/{\done Y_H\, \done \qT^2}$ at an arbitrary power accuracy. During our analysis, in order to facilitate the establishment of the relevant scaling relations, we concentrated on the central rapidity region where $e^{\pm Y_H}\sim\mathcal{O}(1)$. As it turns out, the expression in Eq.~\eqref{eq:asyexp:tot} can also be extrapolated to the domain \begin{align}\label{eq:def:YH:etp} \mathrm{min}\{\sqrt{s}-m_He^{Y_H},\sqrt{s}-m_He^{-Y_H}\}>\mathrm{max}\{m_H e^{ Y_H},m_H e^{- Y_H}\}\,. \end{align} This extrapolation is straightforward to achieve in the kinematical reduction in Sec.~\ref{sec:setups}, since the expansion parameter therein is $(\qT^2/m_H^2)$. Regarding $\Delta\widetilde{\mathcal{I}}^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\}}$, it is worth reminding the reader that the power expansion in Sec.~\ref{sec:red:qT:boundary} primarily builds on the hierarchies, \begin{align}\label{eq:def:b.c.:YH:etp} \sqrt{s}-m_He^{\pm Y_H}\gg \left| m_H-\mT\right|e^{\pm Y_H}\,,\quad m_He^{\pm Y_H}\gg \frac{\qT^2}{\sqrt{s}-m_He^{\mp Y_H}}\,. \end{align} Both relations are maintained by Eq.~\eqref{eq:def:YH:etp} in the low \qT~domain, and therefore the power expansion of $\Delta\widetilde{\mathcal{I}}^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\}}$ proceeds as before. A similar situation can be found in the interior contribution $\widetilde{\mathcal{I}}^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\}}$, in which the categorisation and the subsequent expansion base on the following relationship, \begin{align}\label{eq:def:soft:YH:etp} \sqrt{s}-m_He^{- Y_H}> m_H e^{- Y_H} \gtrsim \nu_{n} \gg \frac{\qT^2}{\nu_\nbar} \gtrsim \frac{\qT^2}{m_He^{Y_H}}>\frac{\qT^2}{\sqrt{s}-m_He^{Y_H}} \,. \end{align} These inequalities ensure the integration variable $k_{\pm}$ is always comparable to $m_H e^{\mp Y_H}$ in magnitude in the collinear sector, while that in the transitional domain is small enough to perform the power expansion. Eq.~\eqref{eq:def:soft:YH:etp} is manifestly satisfied by the domain of Eq.~\eqref{eq:def:YH:etp} for the small~\qT~regime, from which there exists a sufficiently wide window to introduce the auxiliary cutoff scales $\nu_n$ and $\nu_\nbar$. Hence, the subsequent power series of $\widetilde{\mathcal{I}}^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\}}$ can be derived as in Sec.~\ref{sec:red:qT:central}. Following the above consideration, we can implement the expansion of Eq.~\eqref{eq:asyexp:tot} within the full range of Eq.~\eqref{eq:def:YH:etp}. At the LHC with a colliding energy $\sqrt{s}=13\,\text{TeV}$, this interval corresponds to the rapidity region $|Y_H|\lesssim4$ and, thus, enables a reliable power expansion in the bulk of the accessible phase space. Moving from $|Y_H|\approx0$ to $|Y_H|\lesssim4$, it is possible that novel hierarchies emerge from $\widetilde{\mathcal{H}}^{(\omega),\rho,\sigma }_{[\kappa],\{\alpha,\beta\}}$ or any of the contributions in $\widetilde{\mathcal{I}}^{ \rho,\sigma}_{[\kappa],\{\alpha,\beta\}}$. For instance, $m_H e^{Y_H}\gg \qT\gg m_H e^{-Y_H}$ at $Y_H=3.5$ and $\qT=30\,\text{GeV}$, which may alter the relative size of the coefficients at each power. It will not, however, impact the convergence of the~power~series of Eq.~\eqref{eq:asyexp:tot} as a whole. Eventually, it should be emphasised that our derivation of the power series expansion of the process $pp\to H+X$ primarily replies on the factorisation of the light-cone momenta in Eq.~\eqref{eq:qcd:def:H}. An analogous situation can also be found in the NLO squared amplitudes for the Drell-Yan process viewed in terms of the decomposed scalar products in Eq.~\eqref{eq:def:sji}. Therefore, our results for $\widetilde{\mathcal{I}}^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\}}$ and $\Delta\widetilde{\mathcal{I}}^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\}}$ obtained in this section are straightforwardly applicable onto the Drell-Yan process. After combining with its respective hard sector $\widetilde{\mathcal{H}}$, it will in turn generate a power series via Eq.~\eqref{eq:asyexp:tot} in the low \qT\ domain. Beside those two process classes, producing a single colour singlet boson, after appropriate generalisation of the kinematics, Eq.~\eqref{eq:asyexp:tot} can in part also be used to describe the hadroproduction of the multiple colourless bosons, $pp\to B_1+B_2\dots B_n+X(n\ge2)$, as well. We will elaborate on this procedure in App.~\ref{sec:asyexp:Bs}. \section{Implementation up to \texorpdfstring{\NNLP}{NNLP}} \label{sec:asyexp:outputs} In this section, we will analyse the asymptotic behaviour of the \qT~spectrum on the process $pp\to H+X$, and present the analytic expressions for the power corrections up to \NNLP. As illustrated in Eq.~\eqref{eq:asyexp:tot}, the power expansion within the small \qT~domain comprises two sectors, the interior contribution $\widetilde{\mathcal{I}}^{ \rho,\sigma }_{[\kappa], \{\alpha,\beta\}}$ and the boundary corrections $\Delta\widetilde{\mathcal{I}}^{ \rho,\sigma }_{[\kappa],\{\alpha,\beta\}}$. In the following, we will make use of three different methods to evaluate the interior sector. In Sec.~\ref{sec:app:cfs}, the expressions in Eqs.~\eqref{eq:def:asyexp:c:mom}-\eqref{eq:def:asyexp:cbar:mom:at:omega} and \eqref{eq:def:asyexp:cs:mom:int}-\eqref{eq:def:asyexp:cbars:mom:int} that are derived via the momentum cutoffs scales $\nu_{n(\nbar)}$ in Eq.~\eqref{eq:def:col-n:soft:col-nbar:cutoff} will be implemented. The results of Eq.~\eqref{eq:def:asyexp:c:at:omega:nured} and Eq.~\eqref{eq:def:c0:ns} using a homogeneous regulator will be detailed in Sec.~\ref{sec:app:prap} while an inhomogeneous prescription is used Sec.~\ref{sec:app:exp}. It will be demonstrated that all three methods result in identical expressions for the interior contribution after combining all relevant terms. We expect the comparative study here can help the interpretation of the rapidity-divergence regularisation and present a viable prescription in the resummation beyond the leading power in the future. \subsection{Power expansion with momentum cutoffs} \label{sec:app:cfs} In line with the categorisation of phase space in Eq.~\eqref{eq:def:col-n:soft:col-nbar:cutoff}, the interior contributions are decomposed in terms of the collinear and transitional sectors, from which we can re-write Eq.~\eqref{eq:asyexp:tot} here, \begin{align}\label{eq:def:asyexp:mcfs} \frac{\done \sigma_H}{\done Y_H \done \qT^2}\, =\, \frac{\done \sigma^{\langle \mathrm{m.c.}\rangle}_H} {\done Y_H \done \qT^2} \Bigg|_{c}\, +\, \frac{\done \sigma^{\langle \mathrm{m.c.}\rangle}_H} {\done Y_H \done \qT^2} \Bigg|_{cs}\, +\, \frac{\done \sigma^{\langle \mathrm{m.c.}\rangle}_H} {\done Y_H \done \qT^2} \Bigg|_{\bar{c}s}\, +\, \frac{\done \sigma^{\langle \mathrm{m.c.}\rangle}_H} {\done Y_H \done \qT^2} \Bigg|_{\bar{c}}\, +\, \frac{\done \sigma_H}{\done Y_H \done \qT^2} \Bigg|_{b.c.}\,. \end{align} Therein, the ingredients with the subscripts $``c"$ and $``\bar{c}"$ account for the collinear pieces defined in Eqs.~\eqref{eq:def:asyexp:c:mom:at:omega} and \eqref{eq:def:asyexp:cbar:mom:at:omega}, respectively, while those indicated by $``cs"$ and $``\bar{c}s"$ encode the transitional elements from Eqs.~\eqref{eq:def:asyexp:cs:mom:int}-\eqref{eq:def:asyexp:cbars:mom:int}. In all these four terms, the superscript $``\mathrm{m.c.}"$ is introduced to manifest the fact that the momentum cutoffs $\nu_n$ and $\nu_\nbar$ are utilised during the power expansion. At last, we take account of the boundary corrections derived in Sec.~\ref{sec:red:qT:boundary}, termed $``b.c."$. In the last section, the power expansions on those sectors are performed directly in the momentum space. To render their expressions more compact, we here recast them in terms of dimensionless parameters, \begin{align}\label{eq:def:kin:xn:xnbar} x_n\, \equiv\, \frac{m_H\,e^{-Y_H}}{\sqrt{s}}\,\equiv 1-\bar{x}_n\,, \qquad\quad x_{\nbar}\, \equiv\, \frac{m_H\,e^{+Y_H}}{\sqrt{s}}\,\equiv 1-\bar{x}_{\nbar}\,, \end{align} and those related to the integration variables, \begin{align}\label{eq:def:kin:zn:znbar} k_+\, &\equiv\, m_H\,e^{-Y_H}\,\left(\frac{1-z_n}{z_n} \right)\,, \qquad\quad k_-\, \equiv\, m_H\,e^{+Y_H}\,\left(\frac{1-z_{\nbar}}{z_{\nbar}} \right)\,, \\ \label{eq:def:kin:znt:znbart} \nu_n\, &\equiv\, m_H\,e^{-Y_H}\,\left(\frac{1-\tilde{z}_n}{\tilde{z}_n} \right)\,, \qquad\quad \nu_{\nbar}\, \equiv\, m_H\,e^{+Y_H}\,\left(\frac{1-\tilde{z}_{\nbar}}{\tilde{z}_{\nbar}} \right) \,. \end{align} Implementing this parameterisation is straightforward in the boundary corrections of Eq.~\eqref{eq:asyexp:deltaI:uc}, the collinear sectors of Eqs.~\eqref{eq:def:asyexp:c:mom:at:omega} and \eqref{eq:def:asyexp:cbar:mom:at:omega}, and the regular terms in the transitional contributions of Eqs.~\eqref{eq:def:asyexp:cs:mom:int}-\eqref{eq:def:asyexp:cbars:mom:int}. For contributions involving the star-distribution, e.g.\ Eq.~\eqref{eq:def:sDist}, we first make use of the method of integration by parts to reduce the higher ranked contributions to lower ones, and then introduce the dimensionless kinematic variables defined above to convert the star-distribution to the customary plus-distribution. Up to \NNLP, the identities relevant to the reduction of the star-distributions read, \begin{equation}\label{eq:plus2:convertor} \begin{split} \int_0^{\Lambda}\,\done x\,\left[\frac{1}{x^2}\right]^{\nu}_{*}\,f(x)\, =\,& \int_0^{\Lambda}\,\done x\,\left[\frac{1}{x}\right]^{\nu}_{*}\,f'(x) \,-\, \frac{f(\Lambda)}{\Lambda} \,+\, f'(0) \,+\, \frac{f(0)}{\nu} \,,\\ \int_0^{\Lambda}\,\done x\,\left[\frac{1}{x^3}\right]^{\nu}_{*}\,f(x)\, =\,& \frac{1}{2}\, \int_0^{\Lambda}\,\done x\,\left[\frac{1}{x}\right]^{\nu}_{*}\,f''(x) \,-\, \frac{f(\Lambda)}{2\,\Lambda^2}-\,\frac{f'(\Lambda)}{2\,\Lambda} \,+\, \frac{3}{4}\,f''(0) \,+\, \frac{f'(0)}{\nu} \,+\, \frac{f(0)}{2\nu^2}\,, \end{split} \end{equation} where $f(x)$ stands for a generic function sufficiently differentiable at $x=0$. Regarding the transformation of the star-distributions to the plus distribution, the following relationships are used during our calculation, \begin{equation}\label{eq:trans:plusD:starD:n} \begin{split} \int^{\sqrt{s}\bar{x}_{n}}_0\done k_+\, \left[\frac{1}{k_+}\right]^{\nu_n}_{*}\,f(k_+) &\,=\, \int^1_{x_n}\done z_n\,\left[\frac{1}{1-z_n}\right]_+ \,f(z_n) \,+\, \int^1_{x_n} \frac{\done z_n}{z_n}\,f(z_n) \,+\, \ln\left[\frac{\sqrt{s}\,x_n}{\nu_n}\right]\,f(0) \,,\\ \int^{\sqrt{s}\bar{x}_{\nbar}}_0\done k_-\, \left[\frac{1}{k_-}\right]^{\nu_{\nbar}}_{*}\,f(k_-) &\,=\, \int^1_{x_{\nbar}}\done z_{\nbar}\, \left[\frac{1}{1-z_{\nbar}}\right]_+ \,f(z_{\nbar}) \,+\, \int^1_{x_{\nbar}} \frac{\done z_{\nbar}}{z_{\nbar}}\,f(z_{\nbar}) \,+\, \ln\left[\frac{\sqrt{s}\,x_{\nbar}}{\nu_{\nbar}}\right]\,f(0)\,, \end{split} \end{equation} where the plus-distribution is defined as, \begin{align}\label{eq:deef:plusD} \int^1_x\done z \,\left[\frac{1}{1-z}\right]_+\,f(z) \,=\, \int^1_x\done z \, \frac{f(z)-f(1)}{1-z} \,-\int^x_0 \done z\,\frac{f(1)}{1-z} \,. \end{align} \subsection*{Transitional domain} We have now all tools in place to present the respective expressions for each term on the r.h.s.\ of Eq.~\eqref{eq:def:asyexp:mcfs}. We begin with the transitional contributions that are associated with $n$-collinear and soft scalings, \begin{equation}\label{eq:def:asyexp:mcfs:cs} \begin{split} \frac{\done \sigma^{\langle \mathrm{m.c.}\rangle}_H} {\done Y_H \done \qT^2}\Bigg|_{cs} \,\equiv\,& \frac{\alpha_s^3C_t^2}{192\pi^2s v^2}\, \sum_{i,j=\{g,q,\bar{q}\}}\, \sum_{\omega=-1}^{\infty}\, \left(\frac{\qT^2}{m_H^2}\right)^{\omega}\, \int^{1}_{\tilde{z}_n}\,\done z_n\, \left[\mathbf{F}_{i/n}\left(\frac{x_n}{z_n}\right)\right]^{\mathbf{T}} \\ & \,\times\, \left\{ \mathbf{R}_{cs}^{(\omega),ij}(z_n) \,+\, \mathbf{P}_{cs}^{(\omega),ij}\, \left[\frac{1}{1-z_n}\right]_+\!\! \,+\, \mathbf{D}_{cs}^{(\omega),ij}\, \delta\left(1-z_n\right) \,+\, \mathbf{B}_{cs}^{(\omega),ij}(\tilde{z}_n)\, \delta\left(\tilde{z}_n-z_n\right) \right\} \\ & \,\times\, \mathbf{F}_{j/\nbar}(x_{\nbar})\,. \end{split} \end{equation} Therein, the \qT~spectrum is expanded in the small parameter $(\qT^2/m^2_H)$ on the r.h.s., and at each power of the resulting series, the coefficient comprises the convolution of the PDFs and the reduced squared amplitudes over the domain $z_n\in[\tilde{z}_n,1]$. To facilitate the discussion, we here express the power series for each PDF in array form, more explicitly, \begin{equation}\label{eq:PDF:N:ary} \begin{split} \left[ \mathbf{F}_{i/n} (\xi_n)\right]^{\mathbf{T}} \,\equiv\, \Big[ f_{i/n}(\xi_n)\,, \xi_n\,f'_{i/n}(\xi_n)\,, \frac{(\xi_n)^2}{2!}\,f''_{i/n}(\xi_n)\,, \ldots\,, \frac{(\xi_n)^k}{k!}\,f^{(k)}_{i/n}(\xi_n)\,, \ldots \Big]\,, \\ \mathbf{F}_{j/\nbar} (\xi_{\nbar}) \,\equiv\, \Big[ f_{j/\nbar}(\xi_\nbar)\,, \xi_\nbar\,f'_{j/\nbar}(\xi_\nbar)\,, \frac{(\xi_\nbar)^2}{2!}\,f''_{j/\nbar}(\xi_\nbar)\,, \ldots \frac{(\xi_\nbar)^k}{k!}\,f^{(k)}_{j/\nbar}(\xi_\nbar)\,, \ldots \Big]^{\mathbf{T}}\,, \end{split} \end{equation} where the superscript ${\mathbf{T}}$ denotes the transposition operation. The shorthands $f^{(k)}_{i/n}$ and $f^{(k)}_{j/\nbar}$ are employed to represent the $k$-th derivative of the PDFs, \begin{align} f^{(k)}_{i/n}(\tilde{\xi}_n)\, \equiv\, \frac{\partial^k}{\partial \xi_n^k}\, f_{i/n }(\xi_n)\bigg|_{\xi_n=\tilde{\xi}_n}\,,\qquad f^{(k)}_{j/\nbar}(\tilde{\xi}_{\nbar})\, \equiv\, \frac{\partial^k}{\partial \xi_{\nbar}^k}\, f_{j/\nbar }(\xi_{\nbar})\bigg|_{\xi_{\nbar}=\tilde{\xi}_{\nbar}}\,. \end{align} Further, the reduced squared amplitudes $\mathbf{R}_{cs}^{(\omega),ij}$ are matrices in the rank of the PDF derivative encoded in $ \mathbf{F}_{i/n}$. % they are sandwiched in between. They characterise the $\omega$th-power regular contributions from the transitional domain initiated by the partons $i$ and $j$. For the partonic channel $gg\to Hg$, the results up to N$^2$LP read, \begin{equation}\label{eq:Rcs:lp_nlp_nnlp:gg} \begin{split} &\mathbf{R}_{cs}^{(-1),gg} = %%%%%%%%%%%%%% % 1st row -z_n+1-\frac{1}{z_n}+\frac{1}{z_n^2}\,, % End %%%%%%%%%%%%%% \\ & \mathbf{R}_{cs}^{(0),gg} = \left[ \begin{array}{ccc} %%%%%%%%%%%%%% % 1st row -\frac{3 z_n^2}{2}-4 z_n-\frac{1}{2}+\frac{1}{2 z_n^2} & \begin{smallmatrix} 3 z_n^2\\ +\frac{5 z_n}{2}+\frac{3}{2}+\frac{1}{2 z_n}+\frac{1}{2 z_n^2} \end{smallmatrix} \\[2.5ex] %%%%%%%%%%%%%% %. 2nd row \frac{z_n^2}{2}+\frac{3 z_n}{2}+\frac{1}{2 z_n} & -z_n^2-z_n-1 % End %%%%%%%%%%%%%% \end{array} \right]\,, \\ &\mathbf{R}_{cs}^{(1),gg}= \left[ \begin{array}{ccc} %%%%%%%%%%%%%% % 1st row \begin{smallmatrix} -\frac{27 z_n^3}{2}+\frac{3 z_n^2}{8}-\frac{15 z_n}{4}-\frac{19}{8}\\-\frac{1}{8 z_n^2} \end{smallmatrix} & \begin{smallmatrix} \frac{27 z_n^2}{4}+\frac{45z_n}{8}+\frac{29}{8}+\frac{5}{8 z_n}\\ +\frac{1}{8 z_n^2} \end{smallmatrix} & \begin{smallmatrix} \frac{3 z_n}{4}-\frac{3}{4}+\frac{3}{4 z_n}+\frac{1}{4 z_n^2} \\ -6 z_n^3+3 z_n^2 \end{smallmatrix} \\[4.ex] %%%%%%%%%%%%%% %. 2nd row \begin{smallmatrix} \frac{27 z_n^3}{4}+\frac{13 z_n^2}{8}+\frac{25 z_n}{8}+\frac{7}{4}\\ +\frac{1}{8 z_n} \end{smallmatrix} & -\frac{9 z_n^2}{4}-\frac{11 z_n}{4}-3+\frac{1}{4z_n} & 3 z_n^3 \\[4.ex] %%%%%%%%%%%%%% % 3rd row -\frac{9 z_n^3}{4}-\frac{7 z_n^2}{4}-\frac{5 z_n}{2}-2 & 0 & -z_n^3-z_n^2-z_n-1 % End %%%%%%%%%%%%%% \\ \end{array} \right]\,. \end{split} \end{equation} Here, all the entries that will vanish in the following are omitted for brevity. In the case of $i=q(\bar{q})$ and $j=g$, we have, \begin{equation}\label{eq:Rcs:lp_nlp_nnlp:qg} \begin{split} &\mathbf{R}_{cs}^{(-1),q(\bar{q})g} = %%%%%%%%%%%%%% % 1st row \frac{2}{9}-\frac{4}{9 z_n}+\frac{4}{9 z_n^2} \,, % End %%%%%%%%%%%%%% \\ &\mathbf{R}_{cs}^{( 0),q(\bar{q})g} = \left[ \begin{array}{ccc} %%%%%%%%%%%%%% % 1st row -\frac{2 z_n}{9}+\frac{1}{3}+\frac{2}{9 z_n^2} & -\frac{1}{9}+\frac{2}{9 z_n}+\frac{2}{9 z_n^2} \\[2.ex] %%%%%%%%%%%%%% % 2nd row \frac{z_n}{9}-\frac{2}{9}+\frac{2}{9 z_n} & 0 \\ % End %%%%%%%%%%%%%% \end{array} \right] \,,\\ &\mathbf{R}_{cs}^{( 1),q(\bar{q})g} = \left[ \begin{array}{ccc} %%%%%%%%%%%%%% % 1st row \frac{z_n^2}{6}-\frac{z_n}{6}+\frac{1}{36}-\frac{1}{18 z_n^2} & \frac{5 z_n}{9}+\frac{1}{4}+\frac{5}{18 z_n}+\frac{1}{18 z_n^2} & \frac{4 z_n}{9}+\frac{5}{18}+\frac{1}{3 z_n}+\frac{1}{9 z_n^2} \\[2.ex] %%%%%%%%%%%%%% % 2nd row -\frac{z_n^2}{9}+\frac{5 z_n}{36}-\frac{1}{18}+\frac{1}{18 z_n} & -\frac{5 z_n}{18}-\frac{2}{9}+\frac{1}{9 z_n} & -\frac{2 z_n}{9}-\frac{2}{9} \\[2.ex] %%%%%%%%%%%%%% % 3rd row \frac{z_n^2}{18}-\frac{z_n}{9}+\frac{1}{9} & 0 & 0 \\ % End %%%%%%%%%%%%%% \end{array} \right] \,. \end{split} \end{equation} Finally, those for the $q\bar{q}$ initial state read as follows, \begin{equation}\label{eq:Rcs:qq} \begin{split} &\mathbf{R}_{cs}^{(-1),q \bar{q} } =0\,, \;\;\;\quad\quad\quad \mathbf{R}_{cs}^{(0),q \bar{q} } = \frac{16}{27 z_n}-\frac{16}{27}\,, \;\;\;\quad\quad\quad \mathbf{R}_{cs}^{(1),q \bar{q} }= \left[ \begin{array}{ccc} \frac{16 z_n}{27}-\frac{16}{27} & \frac{8}{27}+\frac{8}{27 z_n} \\[2.ex] %%%%%%%%%%%%%%%%% \frac{8}{27}-\frac{8 z_n}{27} & 0 \end{array} \right] \,. \end{split} \end{equation} We next advance to the singular terms on the r.h.s.\ of Eq.~\eqref{eq:def:asyexp:mcfs}. $\mathbf{P}^{(\omega)}_{cs}$, consisting of only the constant coefficients, captures the contribution associated with the plus-distribution in Eq.~\eqref{eq:deef:plusD}. Up to \NNLP, they evaluate to, \begin{equation} \begin{split} \label{eq:Pcs:gg_gq_qq} \mathbf{P}_{cs}^{(-1),gg}&=1\,,\quad\quad\quad\quad\quad %======================================== \mathbf{P}_{cs}^{(0),gg} = \left[ \begin{matrix} 4 & -\frac{1}{2}\\[2.ex] -\frac{1}{2} & 1\\ \end{matrix} \right] \,,\quad\quad\quad\quad\quad %======================================== \mathbf{P}_{cs}^{(1),gg} = \left[ \begin{array}{ccc} 3 & -\frac{13}{8} & \frac{9}{4} \\[2.ex] -\frac{13}{8} & \frac{13}{4} & 0 \\[2.ex] \frac{9}{4} & 0 & 1 \end{array} \right]\,, %======================================== \\ \mathbf{P}_{cs}^{(-1),q(\bar{q})g}&=0\,,\quad\quad\quad\quad\quad %======================================== \mathbf{P}_{cs}^{(0),q(\bar{q})g} = \left[ \begin{matrix} \frac{2}{9} & \frac{2}{9} \end{matrix} \right] \,,\quad\quad\quad\quad\quad\quad \mathbf{P}_{cs}^{(1),q(\bar{q})g} = \left[ \begin{array}{ccc} 0 & \frac{2}{9} & \frac{2}{9}\\[2.ex] \frac{1}{9} & \frac{1}{3} & \frac{2}{9} \end{array} \right]\,, \\ %======================================== \mathbf{P}_{cs}^{(-1),q \bar{q} } &=0\,,\quad\quad\quad\quad\quad \mathbf{P}_{cs}^{(0),q \bar{q} } =0\,,\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad \mathbf{P}_{cs}^{(1),q \bar{q} } =0\,. \end{split} \end{equation} Herein, due to the finiteness of the squared amplitude of Eq.~\eqref{eq:msq} in the limit $k_{\pm}\to0$, the $\mathbf{P}_{cs}^{(\omega),q\bar{q}}$ all vanish in the first few power corrections. The remaining singular terms of Eq.~\eqref{eq:msq} are governed by the delta function and the coefficients $\mathbf{D}_{cs}^{(\omega)}$. Their expressions for \LP, \NLP, and \NNLP are, \begin{equation}\label{eq:Dcs:lp_nlp_nnlp} \begin{split} %======================================== \mathbf{D}_{cs}^{(-1),gg}&=\,L_{\mathrm{cs}}\,\mathbf{P}_{cs}^{(-1),gg}\,,\quad \qquad \qquad \qquad \qquad \quad \; %======================================== \mathbf{D}_{cs}^{(-1),q(\bar{q})g}\,=\,\mathbf{D}_{cs}^{(-1),q \bar{q} }\,=\,\mathbf{D}_{cs}^{(0),q \bar{q} } \,=\,\mathbf{D}_{cs}^{(1),q \bar{q} } \,=\,0\,,\\ %======================================== \mathbf{D}_{cs}^{(0),gg} &=\, L_{\mathrm{cs}}\, \mathbf{P}_{cs}^{(0),gg}\, +\, \left[ \begin{array}{ccc} 3 & -3 \\ -1 & +1 \end{array} \right]\,,\qquad\qquad\,\, %======================================== \mathbf{D}_{cs}^{(0),q(\bar{q})g} =\,L_{\mathrm{cs}}\,\mathbf{P}_{cs}^{(0),q(\bar{q})g}\,,\\ %======================================== \mathbf{D}_{cs}^{(1),gg} &=\, L_{\mathrm{cs}}\,\mathbf{P}_{cs}^{(1),gg}\, +\, \left[ \begin{array}{ccc} 9 & -9 & 0 \\[2.ex] -\frac{13}{2} & +\frac{7}{2} & -\frac{3}{2} \\[2.ex] \frac{7}{2} & -\frac{1}{2} & \frac{3}{2} \end{array} \right]\,,\quad %======================================== \mathbf{D}_{cs}^{(1),q(\bar{q})g}=\,L_{\mathrm{cs}}\,\mathbf{P}_{cs}^{(1),q(\bar{q})g}\,+\, \left[ \begin{array}{ccc} 0 & -\frac{4}{9} & -\frac{4}{9} \\[2.ex] 0 & \frac{2}{9} & \frac{2}{9} \end{array} \right]\,,\hspace*{-20mm} \end{split} \end{equation} where the logarithm $L_{\mathrm{cs}}\equiv\ln[\sqrt{s}x_n/\qT]$ results from the logarithmic contributions in the transitional sectors of Eqs.~\eqref{eq:def:asyexp:cs:mom:int} and \eqref{eq:trans:plusD:starD:n}. We note that all $L_{\mathrm{cs}}$ dependences in $\mathbf{D}_{cs}^{(\omega)}$ are correlated to the coefficients $\mathbf{P}_{cs}^{(\omega)}$ at each power. To interpret this phenomenon, it merits recalling that in Eq.~\eqref{eq:def:asyexp:cs:mom:int}, the coefficient function that is convoluted in the star-distribution reads ${F}^{(\alpha_n)}_{i/n,\beta_n} {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}$, which, after reducing the rank with the help of Eq.~\eqref{eq:plus2:convertor}, is recast into ${F}^{(\alpha_n+\omega-\sigma)}_{i/n,\beta_n} {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}$, corresponding to the coefficient of the logarithmic term. During the subsequent transformation in Eq.~\eqref{eq:trans:plusD:starD:n}, this correspondence is inherited by the coefficient associated with the plus distribution, which, within the parametrisation of Eq.~\eqref{eq:def:asyexp:mcfs:cs}, correlates $\mathbf{P}_{cs}^{(\omega)}$ to the logarithmic terms in $\mathbf{D}_{cs}^{(\omega)}$. The last constituent in Eq.~\eqref{eq:def:asyexp:mcfs:cs} is $\mathbf{B}_{cs}^{(\omega)}$. It accommodates the boundary terms on the r.h.s.\ of Eq.~\eqref{eq:plus2:convertor}, as a result of using an integration by parts in its derivation. The outputs for the first three orders read, \begin{equation}\label{eq:Bcs:lp_nlp_nnlp} \begin{split} &\mathbf{B}_{cs}^{(-1),gg} =\mathbf{B}_{cs}^{(-1),q(\bar{q})g} =\mathbf{B}_{cs}^{(-1),q \bar{q}} =\mathbf{B}_{cs}^{(0),q(\bar{q})g} =\mathbf{B}_{cs}^{(0),q \bar{q}} =\mathbf{B}_{cs}^{(1),q \bar{q}} =0\,,\\ & \mathbf{B}_{cs}^{(0),gg} =\left[ \begin{array}{ccc} -\frac{\tilde{z}_n^4}{\tilde{z}_n-1} & \frac{\tilde{z}_n^4}{\tilde{z}_n-1} \\ \end{array} \right]\,,\\ &\mathbf{B}_{cs}^{(1),gg}= \left[ \begin{array}{ccc} \frac{\tilde{z}_n^4 [(11-6 \tilde{z}_n) \tilde{z}_n-8]}{2 (\tilde{z}_n-1)^2} & \frac{\tilde{z}_n^4 (5 \tilde{z}_n-4)}{2 (\tilde{z}_n-1)^2} & \frac{\tilde{z}_n^4 [(8-3 \tilde{z}_n) \tilde{z}_n-6]}{2 (\tilde{z}_n-1)^2} \\[2.ex] \frac{\tilde{z}_n^5}{\tilde{z}_n-1} & 0 & \frac{\tilde{z}_n^5}{2 (\tilde{z}_n-1)} \\ \end{array} \right]\,, \quad \mathbf{B}_{cs}^{(1),q(\bar{q})g} = \left[ \begin{array}{ccc} 0 & \frac{2 \tilde{z}_n^3}{9 (\tilde{z}_n-1)} & \frac{2 \tilde{z}_n^3}{9 (\tilde{z}_n-1)} \\ \end{array} \right]\,.\hspace*{-20mm} \end{split} \end{equation} Since this contribution primarily arises from the reduction of the higher ranked star-distributions, $\mathbf{B}_{cs}^{(\omega),q\bar{q}}$ vanishes for $\omega\in[-1,0,1]$, similarly to the $\mathbf{P}_{cs}^{(\omega),q \bar{q}}$ earlier. The other part of the transitional region is subject to the $\nbar$-collinear and soft scalings, which can be organised in an analogous manner to Eq.~\eqref{eq:def:asyexp:mcfs:cs}, more specifically, \begin{equation}\label{eq:def:asyexp:mcfs:cbars} \begin{split} \frac{\done \sigma^{\langle \mathrm{m.c.}\rangle}_H}{\done Y_H \done \qT^2} \Bigg|_{\bar{c}s} \,\equiv\,& \frac{\alpha_s^3C_t^2}{192\pi^2s v^2}\, \sum_{i,j=\{g,q,\bar{q}\}}\, \sum_{\omega=-1}^{\infty}\, \left(\frac{\qT^2}{m_H^2}\right)^{\omega}\, \int^{1}_{\tilde{z}_\nbar}\,\done z_\nbar\, \left[\mathbf{F}_{i/n}\left( {x_n} \right)\right]^{\mathbf{T}} \\ &\,\times\, \left\{ \mathbf{R}_{\bar{c}s}^{(\omega),ij}(z_\nbar) \,+\, \mathbf{P}_{\bar{c}s}^{(\omega),ij}\, \left[\frac{1}{1-z_\nbar}\right]_+\!\! \,+\, \mathbf{D}_{\bar{c}s}^{(\omega),ij}\, \delta\left(1-z_\nbar\right) \,+\, \mathbf{B}_{\bar{c}s}^{(\omega),ij}(\tilde{z}_\nbar)\,\delta\left(\tilde{z}_\nbar-z_\nbar\right) \right\}\hspace*{-5mm} \\ &\,\times\, \mathbf{F}_{j/\nbar}\left(\frac{x_{\nbar}}{z_\nbar}\right)\,. \end{split} \end{equation} Herein, Eq.~\eqref{eq:def:asyexp:mcfs:cbars} comprises the matrices $\mathbf{R}_{\bar{c}s}$, $\mathbf{P}_{\bar{c}s}$, $\mathbf{D}_{\bar{c}s}$, and $\mathbf{B}_{\bar{c}s}$ to likewise encapsulate the different facets of partonic contributions, akin to those in Eq.~\eqref{eq:def:asyexp:mcfs:cs}. Of them, the matrices for the partonic processes $gg\to Hg$ and $q\bar{q}\to Hg$ can be immediately derived from those appearing in Eq.~\eqref{eq:def:asyexp:mcfs:cs}, as the squared amplitudes for these channels in Eq.~\eqref{eq:msq} (gg and qq) symmetric under the exchange of their initial states, more explicitly, \begin{align} \label{eq:Xcbars:nnlp} \mathbf{X}_{\bar{c}s}^{(\omega),ij}=\left[\mathbf{X}_{cs}^{(\omega),ij}\right]^{\mathbf{T}}\Bigg|_{\substack {z_n\to z_\nbar\,,\; \tilde{z}_n\to \tilde{z}_\nbar\\[0.6ex] L_{\mathrm{cs}}\to L_{\mathrm{\bar{c}s}}}}\,, \quad \mathrm{where} ~\mathbf{X}\in\{\mathbf{R}, \mathbf{P},\mathbf{D},\mathbf{B}\}\; \mathrm{and}\; \{ij\}\in\{gg,q\bar{q}\}\,. \end{align} An analogous strategy can also be applied to evaluate the matrices $\mathbf{P}_{\bar{c}s}^{(\omega),q(\bar{q})g}$ that are induced by the initial state $q(\bar{q})g$. As discussed before, $\mathbf{P}_{\bar{c}s}^{(\omega),q(\bar{q})g}$ is associated with the coefficient of the logarithmic term of $\widetilde{\mathcal{I}}^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\}}|_{\bar{c}s}$ in Eq.~\eqref{eq:def:asyexp:cbars:mom:int}, which, by comparison, is same as that from $\widetilde{\mathcal{I}}^{\rho,\sigma}_{[\kappa],\{\alpha,\beta\} }|_{cs}$ in Eq.~\eqref{eq:def:asyexp:cs:mom:int}. To this end, we have, \begin{align} \label{eq:Pcbars:qg:nnlp} \mathbf{P}_{\bar{c}s }^{(\omega),q(\bar{q})g}=\mathbf{P}_{cs }^{(\omega),q(\bar{q})g}\,. \end{align} This correspondence also holds for the logarithmic contributions in $\mathbf{D}_{\bar{c}s }^{(\omega),q(\bar{q})g}$, \begin{equation}\label{eq:Dcbars:lp_nlp_nnlp} \begin{split} \mathbf{D}_{\bar{c}s }^{(-1),q(\bar{q})g}&=\,0\,,\\ \mathbf{D}_{\bar{c}s }^{(0),q(\bar{q})g} &=\, L_{\mathrm{\bar{c}s}}\, \mathbf{P}_{cs }^{(0),q(\bar{q})g} \, + \left[ \begin{array}{ccc} -\frac{2}{9} &+\frac{2}{9} \\ \end{array} \right]\,, \\ \mathbf{D}_{\bar{c}s }^{(1),q(\bar{q})g}&=\, L_{\mathrm{\bar{c}s}}\, \mathbf{P}_{cs }^{(1),q(\bar{q})g}\, +\, \left[ \begin{array}{ccc} 0 &0 & \frac{2}{9} \\[2ex] -\frac{2}{9} &\frac{2}{9} &\frac{1}{3} \end{array} \right]\,, \end{split} \end{equation} where $L_{\mathrm{\bar{c}s}}\equiv\ln[\sqrt{s}x_\nbar/\qT ]$. Comparing with Eq.~\eqref{eq:Dcs:lp_nlp_nnlp}, the constant terms in Eq.~\eqref{eq:Dcbars:lp_nlp_nnlp} are very different, mirroring the asymmetry of the matrix element of $q(\bar{q})+g\to H+q(\bar{q})$ in Eq.~\eqref{eq:msq} (gq) under the $n$-collinear and $\nbar$ collinear scalings. Unsurprisingly, this asymmetric behaviour also emerges from the regular coefficients, \begin{equation}\label{eq:Rcbars:lp_nlp_nnlp} \begin{split} &\mathbf{R}_{\bar{c}s }^{(-1),q(\bar{q})g} =0 \,,\\ &\mathbf{R}_{\bar{c}s}^{( 0),q(\bar{q})g} = \left[ \begin{array}{ccc} \frac{2}{9}+\frac{2}{9 {z}_\nbar} & -\frac{2}{9} \\ \end{array} \right] \,,\\ &\mathbf{R}_{\bar{c}s}^{( 1),q(\bar{q})g} = \left[ \begin{array}{ccc} \frac{1}{9}-\frac{2 {z}_\nbar}{9} & \frac{2 {z}_\nbar}{9}-\frac{1}{9} & -\frac{2 {z}_\nbar}{9}-\frac{2}{9} \\[2ex] -\frac{2 {z}_\nbar}{9}+\frac{1}{3}+\frac{1}{9 {z}_\nbar} & \frac{2 {z}_\nbar}{9}-\frac{1}{3} & -\frac{2 {z}_\nbar}{9}-\frac{2}{9} \end{array} \right]\,, \end{split} \end{equation} and the boundary corrections, \begin{equation}\label{eq:Bcbars:lp_nlp_nnlp} \begin{split} &\mathbf{B}_{\bar{c}s}^{(-1),q(\bar{q})g} =0\,,\quad \mathbf{B}_{\bar{c}s}^{(0),q(\bar{q})g}=\frac{2 \tilde{z}_\nbar^2}{9 (\tilde{z}_\nbar-1)}\,, \quad \mathbf{B}_{\bar{c}s}^{(1),q(\bar{q})g}= \left[ \begin{array}{ccc} -\frac{(\tilde{z}_\nbar-2) \tilde{z}_\nbar^2}{9 (\tilde{z}_\nbar-1)} & \frac{\tilde{z}_\nbar^3}{9 (\tilde{z}_\nbar-1)} \\[2ex] -\frac{\tilde{z}_\nbar^2 [(\tilde{z}_\nbar-5) \tilde{z}_\nbar+5]}{9 (\tilde{z}_\nbar-1)^2} & \frac{\tilde{z}_\nbar^3}{9 (\tilde{z}_\nbar-1)} \end{array} \right]\,. \end{split} \end{equation} \subsection*{Collinear and ultra-collinear regimes} The collinear contributions governed by Eq.~\eqref{eq:def:asyexp:c:mom:at:omega} and Eq.~\eqref{eq:def:asyexp:cbar:mom:at:omega} are formally aligned with the integrals from the transitional sectors as exhibited in Eqs.~\eqref{eq:def:asyexp:cs:mom:int}-\eqref{eq:def:asyexp:cbars:mom:int}. This correspondence even holds after reducing their rank using Eq.~\eqref{eq:plus2:convertor} and transforming them with the help of Eq.~\eqref{eq:trans:plusD:starD:n} if the plus distribution terms are treated to be regular functions and the boundary terms emerging from the integration by parts are all adapted to the collinear regimes as appropriate. The results then read, \begin{equation}\label{eq:def:asyexp:mcfs:c} \begin{split} \frac{\done \sigma^{\langle \mathrm{m.c.}\rangle}_H}{\done Y_H \done \qT^2} \Bigg|_c \,\equiv\,& \frac{\alpha_s^3C_t^2}{192\pi^2s v^2}\, \sum_{i,j=\{g,q,\bar{q}\}}\, \sum_{\omega=-1}^{\infty}\, \left(\frac{\qT^2}{m_H^2}\right)^{\omega}\, \int^{\tilde{z}_n}_{x_n}\,\done z_n\, \left[ \mathbf{F}_{i/n}\left( \frac{x_n}{z_n} \right)\right]^{\mathbf{T}} \\ &\,\times\, \left\{ \mathbf{R}_{cs}^{(\omega),ij}(z_n) \,+\, \frac{\mathbf{P}_{cs}^{(\omega),ij}}{1-z_n} \,+\, \mathbf{B}_{cs}^{(\omega),ij}(z_n)\, \Big[ \delta\left(x_n-z_n\right) - \delta\left(\tilde{z}_n-z_n\right) \Big] \right\} \\ &\,\times\, \mathbf{F}_{j/\nbar}\left( x_\nbar \right)\,, \\ \frac{\done \sigma^{\langle \mathrm{m.c.}\rangle}_H}{\done Y_H \done \qT^2} \Bigg|_{\bar{c}} \,\equiv\,& \frac{\alpha_s^3C_t^2}{192\pi^2s v^2}\, \sum_{i,j=\{g,q,\bar{q}\}}\, \sum_{\omega=-1}^{\infty}\, \left(\frac{\qT^2}{m_H^2}\right)^{\omega}\, \int^{\tilde{z}_\nbar}_{x_\nbar}\,\done z_\nbar\, \left[\mathbf{F}_{i/n}\left( {x_n} \right)\right]^{\mathbf{T}} \\ &\,\times\, \left\{ \mathbf{R}_{\bar{c}s}^{(\omega),ij}(z_\nbar) \,+\, \frac{\mathbf{P}_{\bar{c}s}^{(\omega),ij}}{1-z_\nbar} \,+\, \mathbf{B}_{\bar{c}s}^{(\omega),ij}(z_\nbar)\, \Big[ \delta\left(x_\nbar-z_\nbar\right) - \delta\left(\tilde{z}_\nbar-z_\nbar\right) \Big] \right\} \\ &\,\times\, \mathbf{F}_{j/\nbar}\left(\frac{x_{\nbar}}{z_\nbar}\right)\,. \end{split} \end{equation} Combining this result with the results from the moderate domain in Eqs.~\eqref{eq:def:asyexp:mcfs:cs} and \eqref{eq:def:asyexp:mcfs:cbars}, we observe that all the dependences on the parameters $\tilde{z}_{n}$ and $\tilde{z}_{\nbar}$, which are associated with auxiliary cutoff scales $\nu_n$ and $\nu_{\nbar}$, drop out. This cancellation is in agreement with the vanishing derivatives in Eq.~\eqref{eq:def:asyexp:central:power:omega:nundiff} and \eqref{eq:def:asyexp:central:power:omega:nunbardiff} as well as the expectation from a direct power expansion on the analytic expressions of the \qT~spectrum (if they are known). Finally, we move to the ultra-collinear contributions, which contains the maximal longitudinal momentum of an emitted parton allowed by the colliding energy. As discussed in Sec.~\ref{sec:red:qT:boundary}, this sector stems from the power expansion on the boundary conditions in Eq.~\eqref{eq:def:b.c.}. Therefore, the resulting expression will be proportional to the derivatives of the respective PDFs at the end point. Moreover, since, as defined in Eqs.~\eqref{eq:def:kc:boundary} and \eqref{eq:def:kcbar:boundary}, the phase space integrals of this region are all restricted in the boundary strips of power-suppressed sizes, the ultra-collinear contribution will not invoke any singular behaviour in the low~\qT~region but can be relevant starting from \NLP as a non-logarithmic power correction. The expression up to \NNLP can be organised as, \begin{equation} \label{eq:def:asyexp:mcfs:uc:ucbar} \begin{split} \frac{\done \sigma_H}{\done Y_H \done \qT^2}\Bigg|_{b.c.} \,\equiv\,& \frac{\alpha_s^3C_t^2}{192\pi^2s v^2}\, \sum_{i,j=\{g,q,\bar{q}\}}\, \sum_{\omega=-1}^{\infty}\, \left(\frac{\qT^2}{m_H^2}\right)^{\omega}\, \Bigg\{\, \left[ \mathbf{F}_{i/n}\left(1\right)\right]^{\mathbf{T}} \,\cdot\, \mathbf{B}^{(\omega),ij}_{u {c}}(x_n) \,\cdot\, \mathbf{F}_{j/\nbar}\left(x_\nbar\right) \\ &\hspace*{58mm} \,+\, \left[ \mathbf{F}_{i/n}\left(x_n\right)\right]^{\mathbf{T}} \,\cdot\, \mathbf{B}^{(\omega),ij}_{u\bar{c}}(x_\nbar) \,\cdot\, \mathbf{F}_{j/\nbar}\left(1\right)\, \Bigg\}\,. \end{split} \end{equation} Therein, the leading power coefficients all vanish, \begin{align} \mathbf{B}^{(-1),ij}_{uc}=\mathbf{B}^{(-1),ij}_{u\bar{c}}=0\,. \end{align} The partonic matrices at the (sub-)subleading power induced by the $\nbar$-collinear mode evaluate to, \begin{equation}\label{eq:Bucbar:nlp_nnlp} \begin{split} %%%%%%%%%%%%% &\mathbf{B}^{(0),gg}_{u\bar{c}}(x_\nbar)= \frac{[({x}_\nbar-1) {x}_\nbar+1]^2}{2 ({x}_\nbar-1)}\,,\\ %%%%%%%%%%%%% &\mathbf{B}^{(1),gg}_{u\bar{c}}(x_\nbar)= \left[ \begin{array}{ccc} \frac{-3 {x}_\nbar^6+11 {x}_\nbar^5-12 {x}_\nbar^4+17 {x}_\nbar^3-10 {x}_\nbar^2+{x}_\nbar-1}{8 ({x}_\nbar-1)^2} & \frac{{x}_\nbar [({x}_\nbar-1) {x}_\nbar+1]^2}{8 ({x}_\nbar-1)} \\[2.0ex] -\frac{({x}_\nbar+1) [({x}_\nbar-1) {x}_\nbar+1]^2}{4 ({x}_\nbar-1)^2} & 0 \\ \end{array} \right]\,,\\ %%%%%%%%%%%%% &\mathbf{B}^{(0),q(\bar{q})g}_{u\bar{c}}(x_\nbar)=\mathbf{B}^{(0),q\bar{q}}_{u\bar{c}}(x_\nbar)=0\,,\\ %%%%%%%%%%%%% &\mathbf{B}^{(1),q(\bar{q})g}_{u\bar{c}}(x_\nbar)= -\frac{{x}_\nbar}{9 ({x}_\nbar-1)^2}\,,\\ %%%%%%%%%%%%% &\mathbf{B}^{(1),q \bar{q} }_{u\bar{c}}(x_\nbar)= \frac{8}{27} ({x}_\nbar-1) {x}_\nbar \,. \end{split} \end{equation} Those from the $n$-collinear mode can be derived from the relation below, \begin{align} \mathbf{B}^{(\omega),ij}_{uc}(x_n) = \left[\mathbf{B}^{(\omega),ij}_{u\bar{c}}(x_\nbar)\right]^{\mathbf{T}} \Bigg|_{x_\nbar\to x_n}\,, \quad \text{where} ~ \omega\in\{-1,0,+1\}\; \text{and}\; \{ij\}\in\{gg,q\bar{q}\}\,, \end{align} together with, \begin{equation} \begin{split} &\mathbf{B}^{(0) q(\bar{q})g}_{uc} =\frac{1}{9} [-({x}_n-2) {x}_n-2]\,,\\ &\mathbf{B}^{(1) q(\bar{q})g}_{uc} = \left[ \begin{array}{ccc} \frac{[{x}_n (2 {x}_n-5)+5] {x}_n^2+2}{36 ({x}_n-1)} & \frac{1}{18} \left({x}_n^2+\frac{2}{{x}_n-1}\right) \\[2.ex] -\frac{1}{36} {x}_n [({x}_n-2) {x}_n+2] & 0 \\ \end{array} \right]\,. \end{split} \end{equation} We have presented here the analytic expressions of the first three terms in the power series of ${\done \sigma_H}/({\done Y_H \done \qT^2})$ in the vicinity of $\qT=0$, using $p+p \to H+X$ with the partonic channels $gg\to Hg$, $q(\bar{q})g\to Hq(\bar{q})$, and $q\bar{q}\to Hg$ as an example. In addition, the \qT~distribution also comprises the channels $gq(\bar{q})\to H q(\bar{q})$ and $\bar{q}q\to H g$, for which the partonic matrices from the corresponding sectors can be derived from those in the $q(\bar{q})g\to Hq(\bar{q})$ and $q\bar{q}\to Hg$ processes by exchanging the labels $n\leftrightarrow \nbar$ as appropriate. In the previous investigations on the process $pp\to H+X$, the ingredients contributing to the leading singular behaviour of the \qT~distributions are known up to \NNNLO~\cite{Catani:2007vq, Catani:2012qa,Catani:2022sgr,Catani:2011kr,Luo:2020epw,Luo:2019szz, Ebert:2020yqt,Gehrmann:2012ze,Gehrmann:2014yya,Echevarria:2016scs, Luo:2019hmp,Luo:2019bmw,Gutierrez-Reyes:2019rug,Chetyrkin:1997iv, Chetyrkin:1997un,Gehrmann:2014vha,Gehrmann:2010ue,Baikov:2009bg, Gehrmann:2005pd,Harlander:2000mg}. Comparing the \NLO expressions in \cite{Li:2016ctv,Luo:2019bmw} derived with the exponential rapidity regulator with the leading terms of the sum of Eq.~\eqref{eq:def:asyexp:mcfs:cs}, \eqref{eq:def:asyexp:mcfs:cbars}, and \eqref{eq:def:asyexp:mcfs:c}, we find perfect agreement between the two upon performing an inverse Fourier transformation. In addition, the \NLP power corrections have also been evaluated in \cite{Ebert:2018gsn} via the $\eta$- and pure rapidity regularisation schemes. Here as well, we have verified that the sum of Eq.~\eqref{eq:def:asyexp:mcfs:cs}, \eqref{eq:def:asyexp:mcfs:cbars}, and \eqref{eq:def:asyexp:mcfs:c} can exactly reproduce the expressions in \cite{Ebert:2018gsn}, \changed{ except for the boundary terms encoded in the $\mathbf{B}_{cs}$ matrix in Eq.~\eqref{eq:def:asyexp:mcfs:cs}, $\mathbf{B}_{\bar{c}s}$ in Eq.~\eqref{eq:def:asyexp:mcfs:cbars}, and $\mathbf{B}_{uc,u\bar{c}}$ in Eq.~\eqref{eq:def:asyexp:mcfs:uc:ucbar}. The reason for the difference in the boundary terms is that all PDFs in \cite{Ebert:2018gsn} are assumed to vanish at the far end, i.e., $ \mathbf{F}_{i/n}(1)= \mathbf{F}_{j/\nbar}(1)=0$, thereby diminishing all boundary corrections therein.} However, in this paper, all contributions from the boundary regions are retained for completeness and generality, and we find non-vanishing boundary terms at least in the PDF set \texttt{MSHT20nlo\_as118}, which is used in Sec.\ \ref{sec:asyexp:numeric}. Further details of this comparison can be found in App.~\ref{sec:comp:nlp}. \subsection{Power expansion with the pure rapidity regulator}\label{sec:app:prap} In this part, we re-derive the power series of ${\done \sigma_H}/({\done Y_H \done \qT^2})$ up to \NNLP with the interior contribution evaluated from the rearranged ingredients, as illustrated in Sec.~\ref{sec:asyexp:qT:extrapl}. An appropriate regularisation scheme is required to be put in place to tame the rapidity divergences emerging from the domains $k_{\pm}\to0$. In the following, the pure rapidity regularisation prescription proposed in \cite{Ebert:2018gsn,Moult:2019vou} will be employed to facilitate our calculation. In this regard, the regulator $\mathcal{R}$ takes the form \begin{align}\label{eq:def:p:rap} \mathcal{R} =\left|\frac{\tilde{\nu}_n}{k_+}\,\frac{k_-}{\tilde{\nu}_\nbar}\right|^{\tau} \,. \end{align} Here $\tilde{\nu}_n$ and $\tilde{\nu}_\nbar$ represent two auxiliary scales, from which an effective cutoff can be imposed upon the rapidity of the emitted partons~\cite{Ebert:2018gsn}, akin to dimensional regularisation. In this paper, for simplicity, we take $\tilde{\nu}_n=\tilde{\nu}_\nbar=m_H$ throughout the calculation. Applying Eq.~\eqref{eq:def:p:rap} onto the $n$-collinear function defined in Eq.~\eqref{eq:def:asyexp:c:at:omega:nured} concerns only the integrand with $\sigma\le\omega$ in the limit $\tau\to0$, more explicitly, \begin{equation}\label{eq:def:asyexp:c:at:omega:nured:prap} \begin{split} \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|^{\langle \mathrm{p.ra.}\rangle}_{c}\!\!\!\! =\;& \frac{\bar{\theta}\left(\omega-\sigma\right)}{(\omega-\rho)!} \int^{\tilde{k}^{\mathrm{max}}_+}_{0}\! \frac{\done k_+}{k_+}\,(k_+)^{\sigma-\omega} {F}^{(\alpha_n)}_{i/n,\beta_n}\!\!\left(k_++m_H e^{-Y_H}\right) {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\!\!\left(m_H e^{+Y_H}\right) \\ & + \frac{\theta\left(\omega-\sigma\right)}{(\omega-\rho)!} \lim_{\tau\to0} \int^{\tilde{k}^{\mathrm{max}}_+}_{0}\! \frac{\done k_+}{k_+}\,(k_+)^{\sigma-\omega} \left|\frac{\qT^2}{k_+^2}\right|^{\tau} {F}^{(\alpha_n)}_{i/n,\beta_n}\!\!\left(k_++m_H e^{-Y_H}\right) {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\!\!\left(m_H e^{+Y_H}\right) .\hspace*{-20mm} \end{split} \end{equation} To compute the second term on the r.h.s., we make use of the generalised star-distribution of Eq.~\eqref{eq:def:sDist} to regularise all singular contributions, and then, within the pure rapidity regularisation scheme, we complete the phase space integrals over those singular terms. The result reads, \begin{equation}\label{eq:def:asyexp:c:at:omega:nured:prap:2nd} \begin{split} \lefteqn{ \theta\left(\omega-\sigma\right) \lim_{\tau\to0} \int^{\tilde{k}^{\mathrm{max}}_+}_{0} \frac{\done k_+}{k_+}\,(k_+)^{\sigma-\omega} \left|\frac{\qT^2}{k_+^2}\right|^{\tau} {F}^{(\alpha_n)}_{i/n,\beta_n}\left(k_++m_H e^{-Y_H}\right) {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right) }\\ &=\, \theta\left(\omega-\sigma\right)\int^{\tilde{k}^{\mathrm{max}}_+}_{0} {\done k_+} \left[\frac{1}{k_+^{\omega-\sigma+1}}\right]_*^{\nu_n} {F}^{(\alpha_n)}_{i/n,\beta_n}\left(k_++m_H e^{-Y_H}\right) {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)\\ &\phantom{=}{}+\theta\left(\omega-\sigma-1\right) \sum_{\eta=0}^{\omega-\sigma-1} \frac{ {F}^{(\alpha_n+\eta)}_{i/n,\beta_n}\left( m_H e^{-Y_H}\right) {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)}{\eta!} \frac{\nu_n^{\sigma+\eta-\omega}}{\sigma+\eta-\omega}\\ &\phantom{=}{}+\theta( \omega-\sigma)\left\{ \ln\left[\frac{\nu_n}{\qT}\right]-\frac{1}{2\tau}\right\}\, \frac{ {F}^ {(\alpha_n+\omega-\sigma)}_{i/n,\beta_n}\left( m_H e^{-Y_H}\right)\, {F}^{ (\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)\,}{ (\omega-\sigma)!}\,, \end{split} \end{equation} where we have expanded in the small parameter $\tau$ and kept only contributions up to $\mathcal{O}(\tau^0)$. From Eqs.~\eqref{eq:def:asyexp:c:at:omega:nured:prap} and \eqref{eq:def:asyexp:c:at:omega:nured:prap:2nd}, we note that except for the pole term, the recombined collinear sector here exactly reproduces the sum of Eq.~\eqref{eq:def:asyexp:c:mom:at:omega} and \eqref{eq:def:asyexp:cs:mom:int} constructed via the explicit cutoffs. Likewise, the first term of Eq.~\eqref{eq:def:asyexp:c:at:omega:nured:prap}, proportional to $\bar{\theta}\left(\omega-\sigma\right)$, and the term containing the star-distribution in Eq.~\eqref{eq:def:asyexp:c:at:omega:nured:prap:2nd} are equivalent to the sum of Eq.~\eqref{eq:def:asyexp:c:mom:at:omega} and the first two lines of Eq.~\eqref{eq:def:asyexp:cs:mom:int}, as can be seen with the help of Eq.~\eqref{eq:def:asyexp:c:at:omega:nured} and the fact that the integrands in those sectors are all regular in the limit $k_+\to0$. In order to interpret the correspondence between the last two lines of Eq.~\eqref{eq:def:asyexp:cs:mom:int} and Eq.~\eqref{eq:def:asyexp:c:at:omega:nured:prap:2nd}, it is beneficial to recall that the $\nu_n$-dependent terms in Eq.~\eqref{eq:def:asyexp:cs:mom:int} in fact stem from the boundary condition in the phase space integral of Eq.~\eqref{eq:def:asyexp:s:mom1}, which, through applying the star distribution in Eq.~\eqref{eq:def:sDist}, is entirely inherited by the singular terms in Eq.~\eqref{eq:def:asyexp:c:at:omega:nured:prap:2nd} and then mostly preserved in evaluating the $k_+$ integral within the pure rapidity regularisation scheme. Therefore, an analogous pattern is presented by the expressions in Eqs.~\eqref{eq:def:asyexp:c:at:omega:nured:prap} and \eqref{eq:def:asyexp:c:at:omega:nured:prap:2nd} and those in Eq.~\eqref{eq:def:asyexp:c:mom:at:omega} and Eq.~\eqref{eq:def:asyexp:cs:mom:int}. A similar strategy can also be used to calculate the $\nbar$-collinear term in Eq.~\eqref{eq:def:asyexp:c:at:omega:nured}, which evaluates to, \begin{equation}\label{eq:def:asyexp:cbar:at:omega:nured:prap} \begin{split} \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}} \Bigg|^{\langle \mathrm{p.ra.}\rangle}_{\bar{c}} =&\; \frac{\bar{\theta}( \omega-\rho)}{(\omega-\sigma)!}\, \int^{{\frac{\qT^2}{\tilde{k}^{\mathrm{min}}_+}} }_0\, \frac{\done k_-}{k_-}\,k_-^{\rho-\omega}\, {F}^{(\alpha_n+\omega-\sigma)}_{i/n,\beta_n}\left(m_H e^{-Y_H}\right)\, {F}^{(\alpha_\nbar)}_{j/\nbar,\beta_\nbar}\left(k_-+m_H e^{+Y_H}\right) \\ &+ \frac{{\theta}( \omega-\rho)}{(\omega-\sigma)!}\, \int^{{\frac{\qT^2}{\tilde{k}^{\mathrm{min}}_+}}}_0\, \done k_-\, \left[\frac{1}{k_-^{\omega-\rho+1}}\right]^{\nu_{\nbar}}_{*}\, {F}^{(\alpha_n+\omega-\sigma)}_{i/n,\beta_n}\left(m_H e^{-Y_H}\right)\, {F}^{(\alpha_\nbar)}_{j/\nbar,\beta_\nbar}\left(k_-+m_H e^{+Y_H}\right) \hspace*{-20mm} \\ &+ \frac{{\theta}(\omega-\rho-1)}{(\omega-\sigma)!}\,\sum_{\lambda=0}^{\omega-\rho-1}\, \frac{ {F}^{(\alpha_n+\omega-\sigma)}_{i/n,\beta_n}\left(m_H e^{-Y_H}\right)\, {F}^{(\alpha_\nbar+\lambda)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)\, }{\lambda!} \, \frac{ \nu_{\nbar}^{\rho+\lambda-\omega}}{\rho+\lambda-\omega} \\ &+ \frac{ {\theta}( \omega-\rho)}{(\omega-\sigma)!}\, \left\{\ln\left[\frac{\nu_{\nbar}}{\qT}\right]+\frac{1}{2\tau}\right\}\, \frac{ {F}^{(\alpha_n+\omega-\sigma)}_{i/n,\beta_n}\left(m_H e^{-Y_H}\right)\, {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)\, }{(\omega-\rho)!} \,. \end{split} \end{equation} In comparison with Eq.~\eqref{eq:def:asyexp:c:at:omega:nured:prap:2nd}, we note that the sign in front of the pole term is reversed. % compared to Eq.~\eqref{eq:def:asyexp:c:at:omega:nured:prap}. This indicates that the rapidity regulator in appraising the $\nbar$-collinear sector is in practice activated in a distinct extremal region than in the $n$-collinear case. Combining the $n$-collinear function in Eq.~\eqref{eq:def:asyexp:c:at:omega:nured:prap:2nd} with the $\nbar$-collinear piece of Eq.~\eqref{eq:def:asyexp:c:at:omega:nured:prap}, it is immediate to find that all poles cancel, fully reproducing our previous results summing Eqs.~\eqref{eq:def:asyexp:c:mom:at:omega} and \eqref{eq:def:asyexp:cbar:mom:at:omega} as well as Eqs.~\eqref{eq:def:asyexp:cs:mom:int} and \eqref{eq:def:asyexp:cbars:mom:int} derived using the momentum cutoffs. In fact, this agreement suggests that within the pure-rapidity regularisation scheme, the soft contribution of Eq.~\eqref{eq:def:s:fs:rap} and zero-bin subtrahends of Eq.~\eqref{eq:def:c0:ns} could be redundant. To confirm this, it is worth noting that the phase space integrals in these two functions are all unbounded by definition, such that applying the pure rapidity regulator here only results in vanishing quantities in the limit $\tau\to0$. It thus leads to, \begin{align}\label{eq:def:asyexp:s:c0:cbar0:prap} \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|^{\FSmeth,\langle\mathrm{p.ra.} \rangle}_{s}= \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|^{\langle \mathrm{NS}\rangle,\langle\mathrm{p.ra.}\rangle}_{c0} =\widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|^{\langle \mathrm{NS}\rangle,\langle\mathrm{p.ra.} \rangle}_{\bar{c}0}=0\,. \end{align} In absence of the soft function and the zero-bin subtraction within the pure-rapidity regularisation scheme, we can then skip indulging in the inhomogeneous behaviour induced by the doubly and triply projected integrands of Eq.~\eqref{eq:def:asyexp:jantzen}. Similarly, we can also freely switch from Jantzen's formalism~\cite{Jantzen:2011nz} in Eq.~\eqref{eq:def:asyexp:jantzen:red} to our proposal in Eq.~\eqref{eq:def:asyexp:central:power:omega:rap:hom} to perform the power expansion. This forms in part the reason why $\mathcal{R}$ in Eq.~\eqref{eq:def:p:rap} is categorised to be one of the homogeneous regulators here. Applying the expressions of Eqs.~\eqref{eq:def:asyexp:c:at:omega:nured:prap}-% \eqref{eq:def:asyexp:s:c0:cbar0:prap} to Eq.~\eqref{eq:def:asyexp:central:power:omega:rap} or Eq.~\eqref{eq:def:asyexp:central:power:omega:rap:hom}, we arrive at the expression of the interior contribution and, in turn, the power expansion of ${\done \sigma_H}/(\done Y_H \done \qT^2)$. To make their expressions more compact, we recast them once again in terms of the dimensionless parameters defined in Eqs.~\eqref{eq:def:kin:xn:xnbar} by means of the identities in Eqs.~\eqref{eq:plus2:convertor}. Up to \NNLP, the results can be organised below, \begin{equation}\label{eq:def:asyexp:prap} \begin{split} \frac{\done \sigma_H}{\done Y_H \done \qT^2} \,=&\, \frac{\done \sigma_H}{\done Y_H \done \qT^2}\Bigg|_{b.c.} \,+\, \frac{\done \sigma^{\langle \mathrm{p.ra.}\rangle}_H}{\done Y_H \done \qT^2} \Bigg|_{c} \,+\, \frac{\done \sigma^{\langle \mathrm{p.ra.}\rangle}_H}{\done Y_H \done \qT^2} \Bigg|_{\bar{c}} \,, \end{split} \end{equation} where the first term on the r.h.s accounts for the boundary correction as illustrated in eq.~\eqref{eq:def:asyexp:mcfs:uc:ucbar}. The second and third terms govern the $n$-collinear contributions in eqs.~(\ref{eq:def:asyexp:c:at:omega:nured:prap}-\ref{eq:def:asyexp:c:at:omega:nured:prap:2nd}) and the $\nbar$-collinear case in eq.~\eqref{eq:def:asyexp:cbar:at:omega:nured:prap}, respectively. Their expressions read, \begin{equation} \begin{split} \frac{\done \sigma^{\langle \mathrm{p.ra.}\rangle}_H}{\done Y_H \done \qT^2}\Bigg|_c \,\equiv\,& \frac{\alpha_s^3C_t^2}{192\pi^2s v^2}\, \sum_{i,j=\{g,q,\bar{q}\}}\, \sum_{\omega=-1}^{\infty}\, \left(\frac{\qT^2}{m_H^2}\right)^{\omega}\, \int^{1}_{x_n}\,\done z_n\, \left[\mathbf{F}_{i/n}\left(\frac{x_n}{z_n}\right)\right]^{\mathbf{T}} \\ &\,\times\, \Bigg\{ \mathbf{R}_{cs}^{(\omega),ij}(z_n) \,+\, \mathbf{P}_{cs}^{(\omega),ij}\,\left[\frac{1}{1-z_n}\right]_+ +\, \left(\mathbf{S}^{(\omega),ij}_c+\mathbf{D}_{cs}^{(\omega),ij}\right)\,\delta\left(1-z_n\right) \\ &\hspace*{8mm} \,+\, \mathbf{B}_{cs}^{(\omega),ij}(z_n)\, \delta\left(x_n-z_n\right) \Bigg\}\; \mathbf{F}_{j/\nbar}(x_{\nbar})\,, \end{split} \end{equation} and \begin{equation} \begin{split} \frac{\done \sigma^{\langle \mathrm{p.ra.}\rangle}_H}{\done Y_H \done \qT^2} \Bigg|_{\bar{c}} \,\equiv\,& \frac{\alpha_s^3C_t^2}{192\pi^2s v^2}\, \sum_{i,j=\{g,q,\bar{q}\}}\, \sum_{\omega=-1}^{\infty}\, \left(\frac{\qT^2}{m_H^2}\right)^{\omega}\, \int^{1}_{x_\nbar}\,\done z_\nbar\, \left[\mathbf{F}_{i/n}\left(x_n\right)\right]^{\mathbf{T}} \\ &\,\times\, \Bigg\{ \mathbf{R}_{ \bar{c}s}^{(\omega),ij}(z_\nbar) \,+\, \mathbf{P}_{\bar{c}s}^{(\omega),ij}\,\left[\frac{1}{1-z_\nbar}\right]_+ +\, \left(\mathbf{S}^{(\omega),ij}_{\bar{c}} \,+\, \mathbf{D}_{\bar{c}s}^{(\omega),ij}\right)\, \delta\left(1-z_\nbar\right) \\ &\hspace*{8mm} \,+\, \mathbf{B}_{\bar{c}s}^{(\omega),ij}(z_\nbar)\, \delta\left(x_\nbar-z_\nbar\right) \Bigg\}\; \mathbf{F}_{j/\nbar}\left(\frac{x_{\nbar}}{z_\nbar}\right)\,, \end{split} \end{equation} where the matrices $\mathbf{R}$, $\mathbf{P}$, $\mathbf{D}$, and $\mathbf{B}$ have been previously displayed in Sec.~\ref{sec:app:cfs}. The novel ingredients here are $\mathbf{S}_c$ and $\mathbf{S}_{\bar{c}}$, characterising the pole terms in Eqs.~\eqref{eq:def:asyexp:c:at:omega:nured:prap:2nd} and \eqref{eq:def:asyexp:cbar:at:omega:nured:prap}. The coefficients of these singularities in the $n$-($\nbar$-)collinear sector are of opposite (same) sign, but otherwise identical, to those associated with the logarithmic contributions. \changed{The} latter are, as discussed in Sec.~\ref{sec:app:cfs}, associated with the partonic matrices in front of the plus distributions. Hence, we can now express $\mathbf{S}_{c}$ and $\mathbf{S}_{\bar{c}}$ in terms of $\mathbf{P}_{cs}$ in Eqs.~\eqref{eq:Pcs:gg_gq_qq}, more specifically, \begin{align} \label{eq:Sc:nnll} \mathbf{S}^{(\omega),ij}_{c}\, =\, -\,\mathbf{S}^{(\omega),ij}_{\bar{c}}\, =\, -\,\frac{1}{2\tau}\, \mathbf{P}^{(\omega),ij}_{cs}\,, \quad \mathrm{where}~ \omega\in\{-1,0,1\}~ \mathrm{and}~ \{ij\}=\{gg,q(\bar{q})g,q \bar{q}\}\,. \end{align} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% % pole expressions %\begin{align} %\mathbf{S}^{(-1),gg}_c= -\frac{1}{2 \eta } %\,,\quad\quad %\mathbf{S}^{(0),gg}_c= %\left[ %\begin{array}{ccc} % -\frac{2}{\eta } & \frac{1}{4 \eta } \\[2.ex] % \frac{1}{4 \eta } & -\frac{1}{2 \eta } \\ %\end{array} %\right] %\,,\quad\quad %\mathbf{S}^{(1),gg}_c= %\left[ %\begin{array}{ccc} % -\frac{3}{2 \eta } & \frac{13}{16 \eta } & -\frac{9}{8 \eta } \\[2.ex] % \frac{13}{16 \eta } & -\frac{13}{8 \eta } & 0 \\[2.ex] % -\frac{9}{8 \eta } & 0 & -\frac{1}{2 \eta } \\ %\end{array} %\right]\,, %\end{align} % %\begin{align} %\mathbf{S}^{(-1),q(\bar{q})g}_c= 0 %\,,\quad\quad %\mathbf{S}^{(0),q(\bar{q})g}_c= %\left[ %\begin{array}{ccc} % -\frac{1}{9 \eta } & -\frac{1}{9 \eta } \\ %\end{array} %\right] %\,,\quad\quad %\mathbf{S}^{(1),q(\bar{q})g}_c= %\left[ %\begin{array}{ccc} % 0 & -\frac{1}{9 \eta } & -\frac{1}{9 \eta } \\[2.ex] % -\frac{1}{18 \eta } & -\frac{1}{6 \eta } & -\frac{1}{9 \eta } \\ %\end{array} %\right]\,, %\end{align} % %\begin{align} %\mathbf{S}^{(-1),q \bar{q} }_c=\mathbf{S}^{(0),q \bar{q} }_c= \mathbf{S}^{(1),q \bar{q} }_c=0\,, %\end{align} %.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%. %. nbar collinear case % \begin{align} %\mathbf{S}^{(\omega),ij}_{\bar{c}}=-\mathbf{S}^{(\omega),ij}_{c} %\end{align} %.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%.%. \subsection{Power expansion with the exponential rapidity regulator} \label{sec:app:exp} In order to explore the pattern of the power expansion of ${\done \sigma_H}/({\done Y_H \done \qT^2})$ in a more generic way, in the following we re-appraise the interior region with the aid of the exponential regulator~\cite{Li:2016axz,Li:2016ctv}. As will be illustrated below, the zero-bin subtrahends at this moment are non-trivial and play an important role in the cancellation of the pole terms, at variance to those derived in Sec.~\ref{sec:app:prap}. We will use the \NSmeth prescription here and make use of Eq.~\eqref{eq:def:c0:ns} to establish them. The exponential regulator takes the form, \begin{align}\label{eq:def:exp} \mathcal{R}=\exp\left(-\tau\,b_0\,k_0\right)\,, \end{align} where $b_0=2e^{-\gamma_{\mathrm{E}}}$. At \LP, where non-Abelian exponentiation \cite{Li:2016ctv,Luo:2019hmp} holds, this type of regularisation scheme has been extensively utilised to calculate the fixed-order ingredients related to \qT~resummation. For instance, the leading power beam and soft functions are now available up to \NNNLO~\cite{Li:2016ctv,Li:2016axz,Luo:2019hmp, Luo:2019bmw,Luo:2020epw,Luo:2019szz}, while the anomalous dimensions are available at \NNNNLO accuracy~\cite{Duhr:2022yyp,Moult:2022xzt}. In the following, we will implement this method to the \NLO~\qT~spectrum up to \NNLP, for the first time. Our deliberations may also be useful for future analyses of power suppressed contribution at \NNLO and beyond, within an inhomogeneous regularisation scheme. We start our discussion by considering the collinear sectors of Eq.~\eqref{eq:def:asyexp:c:at:omega:nured}. Applying the exponential regularisation method here follows an analogous pattern to our steps leading up to Eqs.~\eqref{eq:def:asyexp:c:at:omega:nured:prap} and \eqref{eq:def:asyexp:c:at:omega:nured:prap:2nd}. First, we use the star-distribution of Eq.~\eqref{eq:def:sDist} to separate the regular and singular terms in the limit $k_{\pm}\to0$. The regular terms maximally preserve the form of Eq.~\eqref{eq:def:asyexp:c:at:omega:nured}, while the singular ones contain rapidity divergences under the phase space integral necessitating the exponential regulator. Here we use the functions $\Upsilon_{n}^{(h)}$ and $\Upsilon_{\nbar}^{(h)}$ to collect those singular contributions in the $n$- and $\nbar$-collinear sectors, respectively. Within the exponential regularisation scheme, their expressions read, \begin{align}\label{eq:def:ups:exp} \Upsilon_{n}^{(h)}\, \equiv\, \lim_{\tau\to0}\,\int_0^{\nu_n} \done k_+\,\frac{e^{-\tau b_0k_0}}{k_+^{h+1}}\,, \qquad\qquad\qquad \Upsilon_{\nbar}^{(h)}\, \equiv\, \lim_{\tau\to0}\,\int_0^{\nu_\nbar} \done k_-\,\frac{e^{-\tau b_0k_0}}{k_-^{h+1}}\, =\,\Upsilon_{n}^{(h)}\Bigg|_{\nu_n\to\nu_\nbar}\,. \end{align} As for the first few ranks, $\Upsilon_{n}^{(h)}$ evaluates to, \begin{equation}\label{eq:def:ups:exp:1} \begin{split} \Upsilon_{n}^{(0)}\,&=\,\ln\left[\frac{\nu_n}{\qT}\right]\,-\,L_{\tau}\,,\quad\quad \Upsilon_{n}^{(1)}\,=\,\frac{1}{\qT^2\,\tilde{\tau}}\,-\,\frac{1}{\nu_n}\,,\quad\quad \Upsilon_{n}^{(2)}\,=\,\frac{1}{\qT^4\,\tilde{\tau}^2}\,-\,\frac{1}{2\,\nu^2_n}\,-\,\frac{1}{\qT^2}\,,\\ \Upsilon_{n}^{(3)}\,&=\,\frac{2}{\qT^6\,\tilde{\tau}^3}\,-\,\frac{1}{3\,\nu^3_n}\,-\,\frac{1}{\qT^4\,\tilde{\tau}}\,,\quad\quad\dots\dots\,, \end{split} \end{equation} where $L_{\tau}=\ln(\qT\tau)$ and $\tilde{\tau}=\tau e^{-\gamma_{\mathrm{E}}}$. The expression of $\Upsilon_{\nbar}^{(h)}$ can be derived from $\Upsilon_{n}^{(h)}$ by the replacement $n\leftrightarrow \nbar$. Thus equipped, we are now poised to establish the collinear contribution of Eq.~\eqref{eq:def:asyexp:c:at:omega:nured} within the exponential regularisation scheme, more explicitly \begin{align}\label{eq:def:asyexp:c:at:omega:nured:exp} \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} } \Bigg|^{\langle \mathrm{exp}\rangle}_{c} =\,& \frac{\bar{\theta}\left(\omega-\sigma\right)}{(\omega-\rho)!} \int^{\tilde{k}^{\mathrm{max}}_+}_{0} \frac{\done k_+}{k_+}\,(k_+)^{\sigma-\omega} {F}^{(\alpha_n)}_{i/n,\beta_n}\left(k_++m_H e^{-Y_H}\right) {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)\nnb\\ & + \frac{\theta\left(\omega-\sigma\right)}{(\omega-\rho)!} \int^{\tilde{k}^{\mathrm{max}}_+}_{0}{\done k_+} \left[\frac{1}{k_+^{\omega-\sigma+1}}\right]_*^{\nu_n} {F}^{(\alpha_n)}_{i/n,\beta_n}\left(k_++m_H e^{-Y_H}\right) {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right)\nnb\\ & + \frac{\theta\left(\omega-\sigma-1\right)}{(\omega-\rho)!} \sum_{\eta=0}^{\omega-\sigma-1} \frac{ {F}^{(\alpha_n+\eta)}_{i/n,\beta_n}\left( m_H e^{-Y_H}\right) {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right) }{\eta!}\, \Upsilon_{n}^{(\omega-\sigma-\eta)} % \frac{\nu_n^{\sigma+\eta-\omega}}{\sigma+\eta-\omega} \nnb\\ & + \frac{\theta( \omega-\sigma)}{(\omega-\rho)!} \, \frac{ {F}^{(\alpha_n+\omega-\sigma)}_{i/n,\beta_n}\left( m_H e^{-Y_H}\right)\, {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right) }{(\omega-\sigma)!}\, %\left\{ \ln\left[\frac{\nu_n}{\qT}\right]-\frac{1}{2\tau}\right\} \Upsilon_{n}^{(0)}\,,\\ \label{eq:def:asyexp:cbar:at:omega:nured:exp} \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} } \Bigg|^{\langle \mathrm{exp}\rangle}_{\bar{c}} =&\, \frac{\bar{\theta}( \omega-\rho)}{(\omega-\sigma)!}\, \int^{{\frac{\qT^2}{\tilde{k}^{\mathrm{min}}_+}} }_0\, \frac{\done k_-}{k_-}\,k_-^{\rho-\omega}\, {F}^{(\alpha_n+\omega-\sigma)}_{i/n,\beta_n}\left( m_H e^{-Y_H}\right)\, {F}^{(\alpha_\nbar)}_{j/\nbar,\beta_\nbar}\left(k_-+m_H e^{+Y_H}\right) \,\nnb\\ & + \frac{{\theta}( \omega-\rho)}{(\omega-\sigma)!}\, \int^{{\frac{\qT^2}{\tilde{k}^{\mathrm{min}}_+}}}_{0}{\done k_-} \left[\frac{1}{k_-^{\omega-\rho+1}}\right]^{\nu_{\nbar}}_{*}\, {F}^{(\alpha_n+\omega-\sigma)}_{i/n,\beta_n}\left(m_H e^{-Y_H}\right)\, {F}^{(\alpha_\nbar)}_{j/\nbar,\beta_\nbar}\left(k_-+m_H e^{+Y_H}\right)\,\nnb\\ & + \frac{{\theta}(\omega-\rho-1)}{(\omega-\sigma)!}\, \sum_{\lambda=0}^{\omega-\rho-1}\, \frac{ {F}^{(\alpha_n+\omega-\sigma)}_{i/n,\beta_n}\left( m_H e^{-Y_H}\right)\, {F}^{(\alpha_\nbar+\lambda)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right) }{\lambda!} \, \Upsilon_{\nbar}^{(\omega-\rho-\lambda)}\nonumber\\ % \frac{ \nu_{\nbar}^{\rho+\lambda-\omega}}{\rho+\lambda-\omega}\, & + \frac{{\theta}(\omega-\rho)}{(\omega-\sigma)!}\, %\left\{\ln\left[\frac{\nu_{\nbar}}{\qT}\right]+\frac{1}{2\tau}\right\}\, \frac{ {F}^{(\alpha_n+\omega-\sigma)}_{i/n,\beta_n}\left( m_H e^{-Y_H}\right)\, {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right) }{(\omega-\rho)!} \, \Upsilon_{\nbar}^{(0)}\,. \end{align} By comparison with the expressions in Eqs.~\eqref{eq:def:asyexp:c:at:omega:nured:prap}-% \eqref{eq:def:asyexp:cbar:at:omega:nured:prap} evaluated in the pure-rapidity regularisation scheme, the above expressions possess the same regular contributions in the first two lines, as the regulator has no relevance in the absence of rapidity divergences. In their third lines, aside from identical $\nu_n$ and $\nu_\nbar$ dependences residing in $\Upsilon_{n(\nbar)}$ compared to those in Eqs.~\eqref{eq:def:asyexp:c:at:omega:nured:prap:2nd}-% \eqref{eq:def:asyexp:cbar:at:omega:nured:prap}, the power series in terms of $\qT$ and $\tilde{\tau}$ is appearing. This behaviour stems from the definition of the exponential regulator in Eq.~\eqref{eq:def:exp}, comprising the temporal component $k^0= k_++(\qT^2/k_+)$ as a whole. In deriving the $n$-collinear function, for instance, its second part $(\qT^2/k_+)$ suppresses the rapidity divergences, thereby yielding the leading singularity in the limit $\tilde{\tau}\to0$, whilst the first part $k_+$ gives rise to corrections of $\mathcal{O}(\tilde{\tau})$ and in turn generates subleading singular terms and the constant contributions, as exhibited in Eqs.~\eqref{eq:def:ups:exp:1}. Ultimately, confronting the fourth line of Eqs.~\eqref{eq:def:asyexp:c:at:omega:nured:prap:2nd}-% \eqref{eq:def:asyexp:cbar:at:omega:nured:prap} to the results in Eqs.~\eqref{eq:def:asyexp:c:at:omega:nured:exp}-% \eqref{eq:def:asyexp:cbar:at:omega:nured:exp}, we observe that addition logarithms $L_{\tau}=\ln(\qT\tau)$ emerge in the exponential regularisation scheme. In the limit $\tau\to0$, those logarithms in practice play an equivalent role to the pole term in Eqs.~\eqref{eq:def:asyexp:c:at:omega:nured:prap:2nd}-% \eqref{eq:def:asyexp:cbar:at:omega:nured:prap}. Combining the collinear functions we have derived using the exponential regulator above, a cancellation of all pole terms is not found, at variance with our earlier findings for Eqs.~\eqref{eq:def:asyexp:c:at:omega:nured:prap}-% \eqref{eq:def:asyexp:cbar:at:omega:nured:prap}. %%%%%%%%%%%%%% % memo: the vanishing soft && 0-bin also hold for higher order of $\mathcal{O}(\tau)$ for the pure rap.ra. %%%%%%%%%%%%%% This therefore calls for the zero-bin subtraction procedure derived in Eq.~\eqref{eq:def:c0:ns} to remove all overlapping contributions. Implementing the exponential regulator in Eq.~\eqref{eq:def:c0:ns} prompts the $k_{\pm}$-integrals over the interval $k_{\pm}\in[0,\infty]$, which are encoded by the function $\Upsilon_{zb}^{(h)}$ in this paper, more specifically, \begin{align} \label{eq:def:ups:exp:zb} \Upsilon_{zb}^{(h)}\, \equiv\, \lim_{\tau\to0}\, \int^{\infty}_{0}\, \done k_{\pm} \, \frac{e^{-\tau b_0k_0}}{(k_{\pm})^{h+1}}\,. \end{align} The results for the first few ranks read, \begin{align} \label{eq:def:ups:exp:zb:n2lp} \Upsilon_{zb}^{(0)}\,=\,-\,2\,L_{\tau}\,,\quad\; \Upsilon_{zb}^{(1)}\,=\,\frac{1}{\qT^2\,\tilde{\tau}}\,,\quad\; \Upsilon_{zb}^{(2)}\,=\,\frac{1}{\qT^4\,\tilde{\tau}^2} \,-\,\frac{1}{\qT^2}\,, \quad\; \Upsilon_{zb}^{(3)}\,&=\,\frac{2}{\qT^6\,\tilde{\tau}^3} \,-\, \frac{1}{\qT^4\,\tilde{\tau}}\,, \quad\;\dots\dots \,. \end{align} With the help of Eq.~\eqref{eq:def:ups:exp:zb}, the zero-bin subtrahends in the exponential regularisation can be written as, \begin{equation}\label{eq:def:c0:ns:exp} \begin{split} \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\}} \Bigg|^{\NSmeth, \langle \mathrm{exp} \rangle}_{c0}\, \!\!\!=\,& \theta\left(\omega-\sigma\right) \sum_{\eta=0}^{\omega-\sigma } %\sum_{\lambda=0}^{\omega-\rho}\, \frac{ {F}^{(\alpha_n+\eta)}_{i/n,\beta_n}\left(m_H e^{-Y_H}\right)\, {F}^{(\alpha_\nbar+\omega-\rho)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right) }{\eta!\, (\omega-\rho)!} %\lim_{\tau\to0} % \int^{\infty}_{0} % \frac{\done k_+}{k_+} \left(1-\frac{\delta_{\omega}^{\sigma+\eta}}{2}\right) \Upsilon_{zb}^{(\omega-\sigma-\eta)},\hspace*{-20mm} %\mathcal{R}(k_-,k_+,\tau)\, %(k_+)^{\sigma-\omega+\eta} \, %\delta^{\omega}_{\lambda+\rho}\, \\ \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} } \Bigg|^{\NSmeth, \langle \mathrm{exp} \rangle}_{\bar{c}0}\, \!\!\!=\,& \theta\left(\omega-\rho\right) %\sum_{\eta=0}^{\omega-\sigma }\, \sum_{\lambda=0}^{\omega-\rho} \frac{ {F}^{(\alpha_n+\omega-\sigma)}_{i/n,\beta_n}\left( m_H e^{-Y_H}\right) {F}^{(\alpha_\nbar+\lambda)}_{j/\nbar,\beta_\nbar}\left(m_H e^{+Y_H}\right) }{\lambda!\,(\omega-\sigma)!} %\lim_{\tau\to0}\, % \int^{\infty}_{0}\, % \frac{\done k_-}{k_-}\, \left(1-\frac{\delta_{\omega}^{\rho+\lambda}}{2}\right) \Upsilon_{zb}^{(\omega-\rho-\lambda)}.\hspace*{-20mm} %\mathcal{R}(k_-,k_+,\tau)\, % (k_-)^{\rho-\omega+\lambda}\, % \delta^{\omega}_{\eta+\sigma}\,. \end{split} \end{equation} At leading power $\omega=-1$, where the integrand of Eq.~\eqref{eq:def:subjt} with $\rho=\sigma=-1$ is the relevant contributor, the sum of the contribution above amounts to the leading soft function in Eq.~\eqref{eq:def:s:fs:rap}, agreeing with the assertion made in \cite{Li:2016axz}. Nevertheless, it is worth emphasising that this coincidence will not hold in general. At \NLP, for instance, the zero-bin subtrahends here comprise the terms \begin{equation}\label{eq:sub:nlp:eg} \begin{split} \widetilde{\mathcal{G}}^{-1,-1,(0)}_{[\kappa],\{\alpha,\beta\} } \Bigg|^{\NSmeth, \langle \mathrm{exp} \rangle}_{c0}\, +\, \widetilde{\mathcal{G}}^{-1,-1,(0)}_{[\kappa],\{\alpha,\beta\} } \Bigg|^{\NSmeth, \langle \mathrm{exp} \rangle}_{\bar{c}0}\, =\,& {F}^{(\alpha_n+1)}_{i/n } {F}^{(\alpha_\nbar+1)}_{j/\nbar } \Upsilon_{zb}^{(0)}\,\\ & +\, {F}^{(\alpha_n )}_{i/n } {F}^{(\alpha_\nbar+1)}_{j/\nbar } \Upsilon_{zb}^{(1)}\, +\, {F}^{(\alpha_n+1)}_{i/n } {F}^{(\alpha_\nbar )}_{j/\nbar } \Upsilon_{zb}^{(1)}\,. \end{split} \end{equation} Recalling to the definition in Eq.~\eqref{eq:def:s:fs:rap}, the soft sector at the same power accuracy reads, \begin{equation}\label{eq:s:nlp:eg} \begin{split} \widetilde{\mathcal{G}}^{-1,-1,(0)}_{[\kappa],\{\alpha,\beta\} }\Bigg|^{\FSmeth}_{s}\, =\, {F}^{(\alpha_n+1)}_{i/n } {F}^{(\alpha_\nbar+1)}_{j/\nbar } \Upsilon_{zb}^{(0)}\, +\, \frac{{F}^{(\alpha_n )}_{i/n } {F}^{(\alpha_\nbar+2)}_{j/\nbar }}{2} \Upsilon_{zb}^{(2)}\, +\, \frac{{F}^{(\alpha_n+2)}_{i/n } {F}^{(\alpha_\nbar )}_{j/\nbar } }{2}\Upsilon_{zb}^{(2)}\,. \end{split} \end{equation} Comparing those two expressions, with the exception of the first term on the r.h.s.\ of Eq.~\eqref{eq:s:nlp:eg}, the other constituents in Eq.~\eqref{eq:s:nlp:eg} both differ from those in Eq.~\eqref{eq:sub:nlp:eg}. This discrepancy highlights the structural differences between the soft function and zero-bin subtrahends beyond leading power. Indeed, both of them contain unbounded integrals over integrands expanded in line with soft scaling. However, the soft function consists of all ingredients at a given power, whereas the zero-bin subtrahends concern only those associated with the collinear functions from the lowest power accuracy up to the current power under consideration. Combining the results in Eq.~\eqref{eq:def:c0:ns:exp} with their corresponding collinear ingredients in Eqs.~\eqref{eq:def:asyexp:c:at:omega:nured:exp} and \eqref{eq:def:asyexp:cbar:at:omega:nured:exp}, we observe that all the $\tau$-dependences will drop out as they should, from which we can separately reproduce the $n$- and $\nbar$-collinear contributions in Eqs.~\eqref{eq:def:asyexp:c:mom:at:omega}-% \eqref{eq:def:asyexp:cbar:mom:at:omega} and Eqs.~\eqref{eq:def:asyexp:cs:mom:int}-% \eqref{eq:def:asyexp:cbars:mom:int} derived via the momentum cutoffs, more explicitly, \begin{equation} \begin{split} \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} } \Bigg|^{\langle \mathrm{exp}\rangle}_{c} \, -\, \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} } \Bigg|^{\NSmeth, \langle \mathrm{exp} \rangle}_{c0}\, =\, \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} } \Bigg|_{c} \, +\, \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} } \Bigg|_{cs} \,, \\ \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} } \Bigg|^{\langle \mathrm{exp}\rangle}_{\bar{c}} \, -\, \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} } \Bigg|^{\NSmeth, \langle \mathrm{exp} \rangle}_{\bar{c}0}\, =\, \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} } \Bigg|_{\bar{c}} \, +\, \widetilde{\mathcal{I}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} } \Bigg|_{\bar{c}s} \,. \end{split} \end{equation} Now we are ready to use the zero-bin subtracted collinear contributions to evaluate the internal region in Eq.~\eqref{eq:def:asyexp:central:power:omega:rap} and in turn the \qT~spectrum. Akin to the previous subsections, to make our results more compact, we rewrite the momentum space expressions in Eqs.~\eqref{eq:def:asyexp:c:at:omega:nured:exp}-% \eqref{eq:def:asyexp:cbar:at:omega:nured:exp} and Eq.~\eqref{eq:def:c0:ns:exp} in terms of the dimensionless parameters defined in Eq.~\eqref{eq:def:kin:xn:xnbar}. Up to \NNLP, this kind of transformation can be always achieved through Eqs.~\eqref{eq:plus2:convertor} and \eqref{eq:trans:plusD:starD:n}. Collectively, we express the result below, \begin{equation}\label{eq:asyexp:exp:sum} \begin{split} \frac{\done \sigma_H}{\done Y_H \done \qT^2} \,=&\, \frac{\done \sigma_H}{\done Y_H \done \qT^2}\Bigg|_{b.c.} \,+\, \frac{\done \sigma^{\langle \mathrm{exp}\rangle}_H}{\done Y_H \done \qT^2}\Bigg|_{c} \,-\, \frac{\done \sigma^{\langle \mathrm{exp}\rangle}_H}{\done Y_H \done \qT^2}\Bigg|_{c0} \,+\, \frac{\done \sigma^{\langle \mathrm{exp}\rangle}_H}{\done Y_H \done \qT^2}\Bigg|_{\bar{c}} \,-\, \frac{\done \sigma^{\langle \mathrm{exp}\rangle}_H}{\done Y_H \done \qT^2}\Bigg|_{\bar{c}0} \,, \end{split} \end{equation} where the term with the subscript $``b.c."$ indicates the ultra-collinear contributions as presented in Eq.~\eqref{eq:def:asyexp:mcfs:uc:ucbar}. The following four terms in Eq.~\eqref{eq:asyexp:exp:sum}, marked by the superscripts $``\langle \mathrm{exp}\rangle"$, stand for the collinear sectors and their corresponding zero-bin subtrahends evaluated within the exponential regularisation scheme. Of them, the constituents dressed with the subscripts $``c"$ and $``\bar{c}"$ are induced by Eq.~\eqref{eq:def:asyexp:c:at:omega:nured:exp} and Eq.~\eqref{eq:def:asyexp:cbar:at:omega:nured:exp}, respectively. Their expressions read, \begin{align} \label{eq:asyexp:exp:sum:c} \frac{\done \sigma^{\langle \mathrm{exp}\rangle}_H}{\done Y_H \done \qT^2}\Bigg|_{c} \,\equiv\,& \frac{\alpha_s^3C_t^2}{192\pi^2s v^2} \, \sum_{i,j=\{g,q,\bar{q}\}} \, \sum_{\omega=-1}^{\infty} \, \left(\frac{\qT^2}{m_H^2}\right)^{\omega} \, \int^{1}_{x_n}\,\done z_n \, \left[ \mathbf{F}_{i/n}\left(\frac{x_n}{z_n}\right)\right]^{\mathbf{T}} \nonumber \\ &\,\cdot\, \left\{ \mathbf{R}_{ cs}^{(\omega),ij}(z_n)\,+\, \mathbf{P}_{ cs }^{(\omega),ij} \,\left[\frac{1}{1-z_n}\right]_++\,\left(\mathbf{T}^{(\omega),ij}_c+ \mathbf{D}_{ cs }^{(\omega),ij}\right)\,\delta\left(1-z_n\right) +\, \mathbf{B}_{ c }^{(\omega),ij}(z_n)\,\delta\left(x_n-z_n\right) \right\} \nonumber\\ &\,\cdot\, \mathbf{F}_{j/\nbar}(x_{\nbar})\,,\\ \label{eq:asyexp:exp:sum:cbar} \frac{\done \sigma^{\langle \mathrm{exp}\rangle}_H}{\done Y_H \done \qT^2}\Bigg|_{\bar{c}} \,\equiv\,& \frac{\alpha_s^3C_t^2}{192\pi^2s v^2} \, \sum_{i,j=\{g,q,\bar{q}\}} \, \sum_{\omega=-1}^{\infty} \, \left(\frac{\qT^2}{m_H^2}\right)^{\omega} \, \int^{1}_{x_\nbar}\,\done z_\nbar \, \left[ \mathbf{F}_{i/n}\left( x_n \right)\right]^{\mathbf{T}} \nonumber \\ &\,\cdot\, \left\{ \mathbf{R}_{ \bar{c}s}^{(\omega),ij}(z_\nbar)\,+\, \mathbf{P}_{ \bar{c}s }^{(\omega),ij} \,\left[\frac{1}{1-z_\nbar}\right]_++\,\left(\mathbf{T}^{(\omega),ij}_{\bar{c}}+ \mathbf{D}_{ \bar{c}s }^{(\omega),ij}\right)\,\delta\left(1-z_\nbar\right) +\, \mathbf{B}_{ \bar{c}s}^{(\omega),ij}(z_\nbar)\,\delta\left(x_\nbar-z_\nbar\right) \right\} \nonumber\\ &\,\cdot\, \mathbf{F}_{j/\nbar}\left(\frac{x_{\nbar}}{z_\nbar}\right)\,. \end{align} Here the partonic matrices $\mathbf{R}$, $\mathbf{P}$, $\mathbf{D}$, and $\mathbf{B}$ are same as those in Eq.~\eqref{eq:def:asyexp:mcfs:cs} and Eq.~\eqref{eq:def:asyexp:mcfs:cbars}. The new ingredients are $\mathbf{T}_{c}$ and $\mathbf{T}_{\bar{c}}$, accommodating all the $\tau$-dependences from $\Upsilon_n$ and $\Upsilon_\nbar$ in Eq.~\eqref{eq:def:ups:exp} and \eqref{eq:def:ups:exp:1}. Up to \NNLP, the results for $\mathbf{T}_{c}$ read, \begin{equation} \begin{split} &\mathbf{T}^{(-1),q(\bar{q})g}_{c}\,=\,\mathbf{T}^{(-1),q \bar{q} }_{c}\,=\,\mathbf{T}^{(0),q \bar{q} }_{c}\,=\,\mathbf{T}^{(1),q \bar{q} }_{c}\,=\,0\,,\\ &\mathbf{T}^{(-1),gg}_{c}\,=\,-\,L_{\tau}\,\mathbf{P}^{(-1),gg}_{c}\,,\qquad\qquad \mathbf{T}^{(0),q(\bar{q})g}_{c}\,=\,-\,L_{\tau}\,\mathbf{P}^{(0),q(\bar{q})g}_{c}\,,\\ & \mathbf{T}^{(0),gg}_{c}\,=\,-\,L_{\tau}\,\mathbf{P}^{(0),gg}_{c}\,+\, \left[ \begin{array}{cc} -\frac{r_n}{\qT \tilde{\tau}} & \frac{r_n}{\qT \tilde{\tau}} \end{array} \right]\,,\\ &\mathbf{T}^{(1),gg}_{c} \,=\,-\,L_{\tau}\,\mathbf{P}^{(1),gg}_{c}\,+\, \left[ \begin{array}{ccc} \frac{3 r_n^2}{\qT^2 \tilde{\tau}^2}-3 r_n^2-\frac{7 r_n}{2 \qT \tilde{\tau}} & -\frac{r_n^2}{\qT^2 \tilde{\tau}^2}+r_n^2+\frac{7 r_n}{2 \qT \tilde{\tau}} & \frac{r_n^2}{\qT^2 \tilde{\tau}^2 }-r_n^2 \\[2ex] +\frac{5 r_n}{2 \qT \tilde{\tau}} & -\frac{r_n}{2 \qT \tilde{\tau}} & \frac{r_n}{\qT \tilde{\tau}} \end{array} \right]\,,\\ & \mathbf{T}^{(1),q(\bar{q})g}_{c}\,=\,-\,L_{\tau}\,\mathbf{P}^{(1),q(\bar{q})g}_{c}\,+\, \left[ \begin{array}{ccc} 0 & \frac{2 r_n}{9 \qT \tilde{\tau}} & \frac{2 r_n}{9 \qT \tilde{\tau}} \\ \end{array} \right]\,, \end{split} \end{equation} where $r_n=x_n\,\sqrt{s}/\qT$ and ${r_\nbar}= x_\nbar\,\sqrt{s}/\qT$. As for the partonic processes $gg\to Hg$ and $q\bar{q}\to Hg$, the expressions for $\mathbf{T}_{\bar{c}}$ can be derived by $\mathbf{T}_{c}$ via the following relationship, \begin{align} \mathbf{T}^{(\omega),gg}_{\bar{c}}=\left[\mathbf{T}^{(\omega),gg}_{c}\right]^{\mathbf{T}}\Bigg|_{r_n\to r_\nbar}\,,\quad\quad \mathbf{T}^{(\omega),q\bar{q} }_{\bar{c}}=\left[\mathbf{T}^{(\omega),q\bar{q} }_{c}\right]^{\mathbf{T}}\Bigg|_{r_n\to r_\nbar}\,. \end{align} For those induced by the channel $q(\bar{q})g\to Hq(\bar{q})$, they evaluate to \begin{equation} \begin{split} & \mathbf{T}^{(-1),q(\bar{q})g}_{\bar{c}}\,=\,0\,,\qquad\qquad \mathbf{T}^{(0),q(\bar{q})g}_{\bar{c}}\,=\,-\,L_{\tau}\,\mathbf{P}^{(0),q(\bar{q})g}_{\bar{c}}\,+\,\frac{2 r_\nbar}{9 \qT \tilde{\tau}}\,, \\ & \mathbf{T}^{(1),q(\bar{q})g}_{\bar{c}}\,=\,-\,L_{\tau}\,\mathbf{P}^{(1),q(\bar{q})g}_{\bar{c}}\,+\, \left[ \begin{array}{ccc} \frac{r_\nbar}{9 \qT \tilde{\tau}} & \frac{r_\nbar}{9 \qT \tilde{\tau}} \\[2.ex] \frac{2 r_\nbar^2}{9 \qT^2 \tilde{\tau}^2}-\frac{2 r_\nbar^2}{9}+\frac{r_\nbar}{3 \qT \tilde{\tau}} & \frac{2 r_\nbar}{9 \qT \tilde{\tau}} \\ \end{array} \right]\,. \end{split} \end{equation} On the other hand, Eq.~\eqref{eq:asyexp:exp:sum} also includes the components $``c0"$ and $``\bar{c}0"$, accounting for the zero-bin subtraction terms in Eq.~\eqref{eq:def:c0:ns:exp}. Their results are, \begin{equation}\label{eq:asyexp:exp:sum:c0} \begin{split} \frac{\done \sigma^{\langle \mathrm{exp}\rangle}_H}{\done Y_H \done \qT^2}\Bigg|_{c0} \,\equiv\,& \frac{\alpha_s^3C_t^2}{192\pi^2s v^2} \, \sum_{i,j=\{g,q,\bar{q}\}} \, \sum_{\omega=-1}^{\infty} \, \left(\frac{\qT^2}{m_H^2}\right)^{\omega} \, \left[ \mathbf{F}_{i/n}\left( {x_n} \right)\right]^{\mathbf{T}} \,\cdot\, \mathbf{T}^{(\omega),ij}_c \,\cdot\, \mathbf{F}_{j/\nbar}(x_{\nbar})\,,\\ \frac{\done \sigma^{\langle \mathrm{exp}\rangle}_H}{\done Y_H \done \qT^2}\Bigg|_{\bar{c}0} \,\equiv\,& \frac{\alpha_s^3C_t^2}{192\pi^2s v^2} \, \sum_{i,j=\{g,q,\bar{q}\}} \, \sum_{\omega=-1}^{\infty} \, \left(\frac{\qT^2}{m_H^2}\right)^{\omega} \, \left[ \mathbf{F}_{i/n}\left( {x_n} \right)\right]^{\mathbf{T}} \,\cdot\, \mathbf{T}^{(\omega),ij}_{\bar{c}} \,\cdot\, \mathbf{F}_{j/\nbar}(x_{\nbar})\,. \end{split} \end{equation} Since $\Upsilon_{zb}$ in Eqs.~\eqref{eq:def:ups:exp:zb} and \eqref{eq:def:ups:exp:zb:n2lp} exactly reproduces all the $\tau$-dependent contributions from $\Upsilon_n$ and $\Upsilon_\nbar$ in Eq.~\eqref{eq:def:ups:exp} and \eqref{eq:def:ups:exp:1}, respectively, the partonic matrices $\mathbf{T}_{c}$ and $\mathbf{T}_{\bar{c}}$ governing the zero-bin subtrahends here are identical to those in the collinear sectors in Eqs.~\eqref{eq:asyexp:exp:sum:c} and \eqref{eq:asyexp:exp:sum:cbar}. \section{Numerical results} \label{sec:asyexp:numeric} Having introduced all building blocks in the previous sections, we will now present numerical results for the \qT~spectrum for the process $pp\to H+X$ at LHC by the means of the power expansion derived in Sec.~\ref{sec:asyexp:outputs}. Since we have shown that this power series is equivalent whether it is computed using momentum cutoffs to regulate rapidity divergences, as in Eq.~\eqref{eq:def:asyexp:mcfs}, the pure-rapidity regulator in Eq.~\eqref{eq:def:asyexp:prap}, or the exponential rapidity regulator in Eq.~\eqref{eq:asyexp:exp:sum}, any one can be employed. We would like to stress again, though, that although individual constituents are dependent on the rapidity regularisation scheme, the sum of all sectors is identical in all three choices with no scheme-dependent power-suppressed terms remaining. Hence, it is scheme-independent sum of sectors that we implement. During our calculation, we take the mass $m_H$ of the Higgs boson and the vacuum expectation value $v$ from PDG \cite{ParticleDataGroup:2022pth}. The Wilson coefficient $C_t$, although it is known up to four-loop order \cite{Inami:1982xt,Djouadi:1991tk,Chetyrkin:1997iv, Chetyrkin:1997un,Chetyrkin:2005ia,Schroder:2005hy,Baikov:2016tgj}, we only consider at LO contribution here in accordance with the perturbative accuracy of the amplitudes presented in Eqs.~\eqref{eq:msq}. In this paper, we use the \texttt{MSHT20nlo\_as118} \cite{Bailey:2020ooq} PDF set, with the associated value and evolution of $\alpha_s$, interfaced through \LHAPDF \cite{Buckley:2014ana,Bothmann:2022thx}. We set the renormalisation scale to $\mu_R=m_H$, entering our calculation only as the scale we evaluate the strong coupling at. In implementing \texttt{MSHT20nlo\_as118} for Eq.~\eqref{eq:def:asyexp:mcfs} particular attention should be paid to the fact that the PDFs and their higher order derivatives are both involved in the power correction expansion, as illustrated in Eq.~\eqref{eq:PDF:N:ary}. \changed{ Since, to our best knowledge, there is no public built-in portal in \LHAPDF\ to straightforwardly access the grids for the PDFs' derivatives, in this work, we make use of the method~\cite{Bonvini:2014joa,Diehl:2021gvs} to fit \texttt{MSHT20nlo\_as118} in terms of Chebyshev polynomials at the factorisation scale $\mu_F=m_H$ in the first place, from which the derivatives of the PDFs can be evaluated analytically. The virtue of this strategy is that the robustness of the PDFs' derivatives is maintained in regards to the fitted PDFs throughout our numerical calculation, which, as a matter of fact, is one of prerequisites for delivering the validation procedure. To examine our fitted PDFs, we compare the $q_{\mathrm{T}}$ distributions appraised by \Sherpa~\cite{Gleisberg:2003xi, Gleisberg:2008ta,Sherpa:2019gpd} and \Rivet~\cite{Buckley:2010ar,Bierlich:2019rhm} with \LHAPDF against those from the fitted ones, finding only per-mill level discrepancies in between. } Equipped with those inputs, we are capable of calculating the power series of the \qT~distribution via Eq.~\eqref{eq:def:asyexp:mcfs}. In the following, we will emphasis three types of results, i.e., \begin{equation}\label{eq:def:acc:lp_nlp_nnlp} \begin{split} \frac{\done \sigma^{\langle \mathrm{asy }\rangle}_H}{\done Y_H\, \done \qT^2}\Bigg|_{\text{\LP}}\,=& \, \sum_m\, \frac{\Delta_{\text{\LP}}^{(m)}}{\qT^2}\, (L_H)^m\,,\\ \frac{\done \sigma^{\langle \mathrm{asy }\rangle}_H}{\done Y_H\, \done \qT^2}\Bigg|_{\text{\NLP}}\,=& \, \sum_m\, \frac{\Delta_{\text{\LP}}^{(m)}}{\qT^2}\, (L_H)^m \, +\, \sum_m\, \Delta_{\text{\NLP}}^{(m)}\, (L_H)^m \,,\\ \frac{\done \sigma^{\langle \mathrm{asy }\rangle}_H}{\done Y_H\, \done \qT^2}\Bigg|_{\text{\NNLP}}\,=& \, \sum_m\, \frac{\Delta_{\text{\LP}}^{(m)}}{\qT^2}\, (L_H)^m \, +\, \sum_m\, \Delta_{\text{\NLP}}^{(m)}\, (L_H)^m \, + \, \sum_m\, \qT^2\,\Delta_{\text{\NNLP} }^{(m)}\, (L_H)^m \,, \end{split} \end{equation} where the superscript $``\mathrm{asy}"$ signifies the truncated asymptotic series in the low~\qT~domain. $\Delta_{\mathrm{N}^k\text{\LP}} $ stands for the partonic contribution at the $k$-th power convoluted with PDFs and their derivatives, which can be extracted from the power coefficients in Eq.~\eqref{eq:def:asyexp:mcfs}, Eq.~\eqref{eq:def:asyexp:prap}, or Eq.~\eqref{eq:asyexp:exp:sum}. In Eq.~\eqref{eq:def:acc:lp_nlp_nnlp}, the \qT~spectrum at \LP encodes the most singular behavior in the low \qT~domain, consisting of the first term of the power series in Eq.~\eqref{eq:def:acc}. The \NLP result in Eq.~\eqref{eq:def:acc:lp_nlp_nnlp} includes also the first power correction term, comprising the first two constituents of Eq.~\eqref{eq:def:acc} in total. Our most precise result is calculated at N$^2$LP, given in the last line of Eq.~\eqref{eq:def:acc:lp_nlp_nnlp}. It includes the contributions from $\Delta_{\text{\LP}}$ up to $\Delta_{\text{\NNLP}}$ in eq.~\eqref{eq:def:acc}. Moreover, in order to deliver a quantitative assessment of the quality of these approximate results, we also showcase the exact fixed-order \qT~distribution below as a benchmark. It is derived based on eq.~\eqref{eq:qcd:qT} and dubbed ``F.O." hereafter. \begin{figure}[h!] \centering \begin{subfigure}{0.32\textwidth} \centering \includegraphics[height=.8\linewidth]{Plots_Ratios/qTDist_Lin_AsyExp_ggHg_YHabs_0.pdf} \caption{ } \label{fig:results:val:qTratios:asyexp:ggHg:YH0} \end{subfigure} \begin{subfigure}{0.32\textwidth} \centering \includegraphics[height=.8\linewidth]{Plots_Ratios/qTDist_Lin_AsyExp_qgHq_YHabs_0.pdf} \caption{ } \label{fig:results:val:qTratios:asyexp:qgHq:YH0} \end{subfigure} \begin{subfigure}{0.32\textwidth} \centering \includegraphics[height=.8\linewidth]{Plots_Ratios/qTDist_Lin_AsyExp_qqHg_YHabs_0.pdf} \caption{ } \label{fig:results:val:qTratios:asyexp:qqHg:YH0} \end{subfigure} \caption{ Comparisons of the \qT\ spectra between the exact fixed-order calculation (black) and approximations constructed using the power expansion up to \LP (blue), \NLP (red), and \NNLP (green) for different partonic processes at $|Y_H|=0$. While the upper plot contains the absolute differential cross sections, the lower plot contains the ratios of the approximations w.r.t.\ the exact fixed-order result. Throughout we include the boundary corrections $\mathbf{B}_{cs}$, $\mathbf{B}_{\bar{c}s}$, and $\mathbf{B}_{uc(\bar{c})}$. } \label{fig:results:val:qTratios:asyexp:YH0} \end{figure} We start the discussion of our results by considering the \qT\ spectrum at central rapidities, setting $Y_H=0$ for definitiveness. Fig.~\ref{fig:results:val:qTratios:asyexp:YH0} therefore details a comparison of our power-expanded approximate result of Secs.\ \ref{sec:asyexp:mom} and \ref{sec:asyexp:outputs} including terms up to \LP (blue), \NLP (red), and \NNLP (green) to its exact fixed-order counter-part (black) for all three partonic channels, $gg\to Hg$ (left), $q(\bar{q})g\to Hq(\bar{q})$ (center), and $q\bar{q}\to Hg$ (right). Generally, the main plot focusses on the absolute values of the \qT\ distribution, while the ratio plot shows the the ratio of each of the approximate results to the exact one, allowing to judge the quality of the individual approximation. We will retain this pattern of visualisation throughout this section. Examining at our results in more detail, we begin by discussing the $gg\to Hg$ subprocess, shown in Fig.~\ref{fig:results:val:qTratios:asyexp:ggHg:YH0}. This process dominates the inclusive cross section and any improvements in the quality of the power-expanded approximation will be exceedingly beneficial to the description of the inclusive \qT\ spectrum. Due to the presence of singular terms, see Eq.~\eqref{eq:def:acc}, the \qT\ spectrum is divergent as $\qT\to 0$, hence we limit our deliberations to $\qT>1\,\text{GeV}$. In this limit, the \LP contribution is, of course, dominant and the approximated calculations, independent of the number of higher-power terms included, reproduce the exact result. Nevertheless, departing from the low~\qT~domain towards higher values of our observable, the power corrections manifest themselves progressively. More specifically, the \LP-only result deteriorates in quality the quickest, failing to describe the exact spectrum by about $4\%$ at $\qT=10\,\text{GeV}$ and increasing to about $30\%$ near $\qT=30\,\text{GeV}$. Including the \NLP terms alleviates this deviation somewhat, decreasing it to about $1\%$ at $\qT=10\,\text{GeV}$ and about $10\%$ at $\qT=30\,\text{GeV}$. The best approximation provided in this work, including terms up to \NNLP, reproduces the \qT\ spectrum on level of 1\% up to values in excess of 30\,GeV, leaving higher-power corrections to contribute more than percent level only for $\qT\gtrsim40\,\text{GeV}$. Fig.~\ref{fig:results:val:qTratios:asyexp:qgHq:YH0} now shows the contributions from the partonic channel characterised by $q(\bar{q})g$ initial states. This channel contributes on the 10\% level to the inclusive spectrum. Our results here in general demonstrate an analogous behaviour to those of $gg\to Hg$ in the vicinity of $\qT=0$~GeV, including the presence of a divergence for $\qT\to 0$ as well as the mutual agreement between the fixed-order and approximate curves in that limit. However, advancing to the intermediate \qT~range, distinct features are found between the two in regard to the relative magnitudes of subleading and sub-subleading power corrections. While in Fig.~\ref{fig:results:val:qTratios:asyexp:ggHg:YH0}, these two terms observe convergent but still comparable magnitudes, respectively accounting for$~20\%$ and$~10\%$ contributions of the full theory in the vicinity of $\qT=30$~GeV, the \NLP terms in Fig.~\ref{fig:results:val:qTratios:asyexp:qgHq:YH0} play a dominant role and relegate the terms at \NNLP and beyond to an almost insignificant role. Moving onto the last partonic process contributing at our accuracy, $q\bar{q}\to Hg$, depicted in Fig.~\ref{fig:results:val:qTratios:asyexp:qqHg:YH0}, a very different scenario presents itself. For lack of the LP contributions and the associated singularity at $\qT\to 0$, the fixed-order and approximate results here both approach constants in the low~\qT~region. In particular, the \NLP spectrum here takes the leading role and remains constant throughout the \qT~interval of our interest. The \NNLP corrections, meanwhile, exhibit the linear dependences on the variable \qT\ as the logarithmic contributions in Eqs.~\eqref{eq:Pcs:gg_gq_qq} and \eqref{eq:Dcs:lp_nlp_nnlp} vanish. Comparing with the fixed-order spectrum, the \NLP and \NNLP results both yield the correct regular behaviour in the small \qT~range but give oscillatorily converging power corrections for moderate \qT. For instance, the \NLP approximation overshoots the full theory by about $20\%$ near $\qT=30\,\text{GeV}$, whilst incorporating \NNLP corrections underestimates the exact one by a few percent here. \begin{figure}[h!] \centering \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth]{Plots_Diffs/qTDist_Log_AsyExp_ggHg_YHabs_0.pdf} \caption{ } \label{fig:results:val:qTdist:asyexp:ggHg:YH0} \end{subfigure} \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth]{Plots_Diffs/qTDist_Log_AsyExp_qgHq_YHabs_0.pdf} \caption{ } \label{fig:results:val:qTdist:asyexp:qgHq:YH0} \end{subfigure} \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth]{Plots_Diffs/qTDist_Log_AsyExp_qqHg_YHabs_0.pdf} \caption{ } \label{fig:results:val:qTdist:asyexp:qqHg:YH0} \end{subfigure} \caption{ Difference of the exact spectra and the approximations for the three different partonic processes at $|Y_H|=0$. The solid (dashed) lines present the results including (excluding) the boundary corrections $\mathbf{B}_{cs}$ in Eq.~\eqref{eq:def:asyexp:mcfs:cs}, $\mathbf{B}_{\bar{c}s}$ in Eq.~\eqref{eq:def:asyexp:mcfs:cbars}, and $\mathbf{B}_{uc(\bar{c})}$ in Eq.~\eqref{eq:def:asyexp:mcfs:uc:ucbar}. The blue, red, and green lines detail the \LP, \NLP, and \NNLP approximations, respectively. } \label{fig:results:val:qTdist:asyexp:YH0} \end{figure} In pursuit of further examining the higher-power correction terms derived in Sec.~\ref{sec:asyexp:outputs}, we look into the differences between the fixed order results and the approximate ones. We note at this point that although we have already seen that their respective ratios approach unity in the limit $\qT\to 0$, finite differences in this limit play an important role when the approximants are used to subtract or replace the exact spectrum in higher-order calculations where the divergences cancel against the virtual corrections in the $\qT=0$ bin. Similarly, while the ratio tests above emphasise the relative sizes between the full theory and the sum of all corrections to each power considered, their differences allow to examine the individual term of the power series. To this end, according to the power series in Eq.~\eqref{eq:def:acc} as well as the definitions in Eq.~\eqref{eq:def:acc}, the differences between the two are expected to take the following asymptotic behaviour, \begin{equation}\label{eq:def:acc:diff} \begin{split} \frac{\done \sigma^{\langle \mathrm{F.O. }\rangle}_H}{\done Y_H \done \qT^2}\,-\, \frac{\done \sigma^{\langle \mathrm{asy }\rangle}_H}{\done Y_H \done \qT^2}\Bigg|_{\text{\LP}}\,=& \, \sum_m\, \Delta_{\text{\NLP}}^{(m)}\, (L_H)^m \,+\dots\,,\\ \frac{\done \sigma^{\langle \mathrm{F.O. }\rangle}_H}{\done Y_H \done \qT^2}\,-\, \frac{\done \sigma^{\langle \mathrm{asy }\rangle}_H}{\done Y_H \done \qT^2}\Bigg|_{\text{\NLP}}\,=& \, \sum_m\, \qT^2\,\Delta_{\text{\NNLP} }^{(m)}\, (L_H)^m \, +\,\dots \,,\\ \frac{\done \sigma^{\langle \mathrm{F.O. }\rangle}_H}{\done Y_H \done \qT^2}\,-\, \frac{\done \sigma^{\langle \mathrm{asy }\rangle}_H}{\done Y_H \done \qT^2}\Bigg|_{\text{\NNLP}}\,=& \, \sum_m\, \qT^4\,\Delta_{\mathrm{N}^3\text{\LP} }^{(m)}\, (L_H)^m \, +\,\dots \,. \end{split} \end{equation} The numerical results for the magnitudes of these missing, or yet uncalculated, higher-power corrections are presented in Fig.~\ref{fig:results:val:qTdist:asyexp:YH0} for all three partonic processes at $Y_H=0$. Therein, the solid lines denote our results including both the interior contribution from Sec.~\ref{sec:red:qT:central} and the boundary correction discussed in Sec.~\ref{sec:red:qT:boundary}. Due to the presence of the logarithmic contributions in Eqs.~\eqref{eq:Dcs:lp_nlp_nnlp} and \eqref{eq:Dcbars:lp_nlp_nnlp}, the differences between the exact \qT~spectra and its \LP approximations (blue solid line) experience mild enhancements in magnitude in the low~\qT~regime, agreeing with the expectation in Eq.~\eqref{eq:def:acc:diff}.\footnote{% In fact, the difference between the \LP expression and the exact result forms an integrable divergence as $\qT\to 0$. This integrable divergence is removed once \NLP corrections are introduced. } After incorporating the \NLP corrections, as exhibited in the red solid line, the difference between the full theory and our \NLP-correct approximation starts to decrease as $\qT\to 0$ for all three partonic channels. This echoes again, our \NLP expectation of Eq.~\eqref{eq:def:acc:diff} that, starting at this order, the difference vanishes in this limit. This also demonstrates that at least up to \NLP, the power coefficients of the~\qT~distribution can be reproduced as appropriate by the expressions in Sec.~\ref{sec:asyexp:outputs}. Similarly, including the power corrections up to \NNLP results, detailed by the green line, results in the difference vanishing twice as fast. On the other hand, Fig.~\ref{fig:results:val:qTdist:asyexp:YH0} also depicts our results for which we have removed the boundary contributions of Eq.~\eqref{eq:def:asyexp:mcfs:uc:ucbar}, induced by expanding the integral boundaries of Eq.~\eqref{eq:def:b.c.} as well as those in Eq.~\eqref{eq:def:asyexp:mcfs:cs} and Eq.~\eqref{eq:def:asyexp:mcfs:cbars} which arise from integrating the preceding expressions by parts, in dashed lines. Since those boundary corrections will start at \NLP accuracy, our \LP result (blue) remains unchanged. At \NLP, these boundary impacts play only a small role in both the $gg$ and $q\bar{q}$ channels, but manifest themselves in the $q(\bar{q})g$-initiated process for $\qT\lesssim\mathcal{O}(10^{-2})$. The resulting expression then ceases to reproduce the entire \NLP coefficient of Eq.~\eqref{eq:def:acc}, halting the $\propto\qT^2$ behaviour we would expect the difference with the exact result to exhibit. At \NNLP, the sensitivity of the result to the presence of these boundary contributions is even larger, being noticeable already for \qT\ of $\mathcal{O}(10^{-1})$ in the $gg$-initiated and $\mathcal{O}(1)$ for the $q(\bar{q})g$-initiated partonic channels. In both cases, the respective power accuracy is lost in that domain, and only \LP accuracy is maintained, exemplifying the necessity of the boundary corrections. It is worth noting that despite their indispensable effects in reproducing the power coefficients at a given power, at least up to \NNLP, those boundary terms can only generate constant corrections of comparably small magnitude. They may therefore not play a role of phenomenological interest when the larger \qT\ region, where power corrections are larger by construction, is being investigated, and our results may form the basis of a subleading power resummation. However, it should be stressed that, from a theoretical point of view, the emergence of the boundary corrections highlights one of the main differences between the asymptotic expansion of loop integrals and phase space integrals in the small \qT~regime. While the loop integrals generally involve unbounded integrals and, thus, only incur relevant power expansions of the integrand within a variety of scalings, the expansion of phase space integrals in the small, but finite, \qT\ regime additionally induces phase space boundaries through Eq.~\eqref{eq:def:b.c.}, from which the appearance of hierarchies $\qT\ll m_H$ (and the application of the integration by parts identities) will introduce a novel type of power corrections associated with the PDFs at the end point, as shown in Eq.~\eqref{eq:asyexp:deltaI:uc} and \eqref{eq:trans:plusD:starD:n}. \begin{figure}[t!] \centering \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth]{Plots_Diffs/qTDist_wt_Log_AsyExp_ggHg_YHabs_0.pdf} \caption{ } \label{fig:results:val:qTwt:asyexp:ggHg:YH0} \end{subfigure} \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth]{Plots_Diffs/qTDist_wt_Log_AsyExp_qgHq_YHabs_0.pdf} \caption{ } \label{fig:results:val:qTwt:asyexp:qgHq:YH0} \end{subfigure} \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth]{Plots_Diffs/qTDist_wt_Log_AsyExp_qqHg_YHabs_0.pdf} \caption{ } \label{fig:results:val:qTwt:asyexp:qqHg:YH0} \end{subfigure} \caption{ Difference of the weighted exact spectra and the approximations for the three different partonic processes at $|Y_H|=0$. The solid (dashed) lines present the results including (excluding) the boundary corrections $\mathbf{B}_{cs}$ in Eq.~\eqref{eq:def:asyexp:mcfs:cs}, $\mathbf{B}_{\bar{c}s}$ in Eq.~\eqref{eq:def:asyexp:mcfs:cbars}, and $\mathbf{B}_{uc(\bar{c})}$ in Eq.~\eqref{eq:def:asyexp:mcfs:uc:ucbar}. The blue, green, and red lines detail the \LP, \NLP, \NNLP approximations, respectively. } \label{fig:results:val:qTwt:asyexp:YH0} \end{figure} To scrutinise the power correction at \NNLP, we investigate the differences between the weighted \qT~distribution in the full theory and the power-expanded approximations below. From Eqs.~\eqref{eq:def:acc} as well as \eqref{eq:def:acc:lp_nlp_nnlp}, we expect these differences to exhibit the following asymptotic properties, \begin{equation}\label{eq:def:acc:lp_nlp_nnlp:diff:wt} \begin{split} \frac{1}{\qT^2}\,\frac{\done \sigma^{\langle \mathrm{F.O. }\rangle}_H}{\done Y_H \done \qT^2}\,-\, \frac{1}{\qT^2}\,\frac{\done \sigma^{\langle \mathrm{asy }\rangle}_H}{\done Y_H \done \qT^2}\Bigg|_{\text{\LP}}\,=& \, \sum_m\, \frac{1}{\qT^2}\,\Delta_{\text{\NLP}}^{(m)}\, (L_H)^m \,+\dots\,,\\ \frac{1}{\qT^2}\,\frac{\done \sigma^{\langle \mathrm{F.O. }\rangle}_H}{\done Y_H \done \qT^2}\,-\, \frac{1}{\qT^2}\, \frac{\done \sigma^{\langle \mathrm{asy }\rangle}_H}{\done Y_H \done \qT^2}\Bigg|_{\text{\NLP}}\,=& \, \sum_m\,\Delta_{\text{\NNLP} }^{(m)}\, (L_H)^m \, +\,\dots \,,\\ \frac{1}{\qT^2}\, \frac{\done \sigma^{\langle \mathrm{F.O. }\rangle}_H}{\done Y_H \done \qT^2}\,-\, \frac{1}{\qT^2}\, \frac{\done \sigma^{\langle \mathrm{asy }\rangle}_H}{\done Y_H \done \qT^2}\Bigg|_{\text{\NNLP}}\,=& \, \sum_m\, \qT^2\,\Delta_{\mathrm{N}^3\text{\LP} }^{(m)}\, (L_H)^m \, +\,\dots \,. \end{split} \end{equation} Comparing with Eqs.~\eqref{eq:def:acc:diff}, the remainders on the r.h.s.\ of Eq.~\eqref{eq:def:acc:lp_nlp_nnlp:diff:wt} are generally one power lower. Their numeric results are displayed in Fig.~\ref{fig:results:val:qTwt:asyexp:YH0}. Our attention is immediately drawn to the observation that the difference between the exact and approximate weighted spectrum divergences at \LP as $\qT\to 0$ whereas it approaches a constant at \NLP. Only once the \NNLP corrections are taken into account, including the boundary terms, does the difference of the weighted spectra vanish in the $\qT\to 0$ limit, in line with the \NNLP expectation of Eq.~\eqref{eq:def:acc:lp_nlp_nnlp:diff:wt} justifying (at least the first three terms of) our power series derived in Sec.~\ref{sec:asyexp:outputs}. \begin{figure}[h!] \centering \begin{subfigure}{0.32\textwidth} \centering \includegraphics[height=.8\linewidth]{Plots_Ratios/qTDist_Lin_AsyExp_ggHg_YHabs_1.pdf} \caption{ } \label{fig:results:val:qTratios:asyexp:ggHg:YH1} \end{subfigure} \begin{subfigure}{0.32\textwidth} \centering \includegraphics[height=.8\linewidth]{Plots_Ratios/qTDist_Lin_AsyExp_qgHq_YHabs_1.pdf} \caption{ } \label{fig:results:val:qTratios:asyexp:qgHq:YH1} \end{subfigure} \begin{subfigure}{0.32\textwidth} \centering \includegraphics[height=.8\linewidth]{Plots_Ratios/qTDist_Lin_AsyExp_qqHg_YHabs_1.pdf} \caption{ } \label{fig:results:val:qTratios:asyexp:qqHg:YH1} \end{subfigure}\\[2mm] \centering \begin{subfigure}{0.32\textwidth} \centering \includegraphics[height=.8\linewidth]{Plots_Ratios/qTDist_Lin_AsyExp_ggHg_YHabs_3.pdf} \caption{ } \label{fig:results:val:qTratios:asyexp:ggHg:YH3} \end{subfigure} \begin{subfigure}{0.32\textwidth} \centering \includegraphics[height=.8\linewidth]{Plots_Ratios/qTDist_Lin_AsyExp_qgHq_YHabs_3.pdf} \caption{ } \label{fig:results:val:qTratios:asyexp:qgHq:YH3} \end{subfigure} \begin{subfigure}{0.32\textwidth} \centering \includegraphics[height=.8\linewidth]{Plots_Ratios/qTDist_Lin_AsyExp_qqHg_YHabs_3.pdf} \caption{ } \label{fig:results:val:qTratios:asyexp:qqHg:YH3} \end{subfigure} \caption{ Comparisons of the \qT\ spectra between the exact fixed-order calculation (black) and approximations constructed using the power expansion up to \LP (blue), \NLP (red), and \NNLP (green) for different partonic processes at $|Y_H|=1$ (top) and $|Y_H|=3$ (bottom). Throughout we include the boundary corrections $\mathbf{B}_{cs}$, $\mathbf{B}_{\bar{c}s}$, and $\mathbf{B}_{uc(\bar{c})}$. } \label{fig:results:val:qTratios:asyexp:YH3} \end{figure} In the previous figures we have focussed on the \qT~spectra at central rapidities, $|Y_H|=0$, where $e^{\pm Y_H}\sim\order(1)$. We now increase the rapidity of the Higgs boson to affect the scaling of the relevant light cone momenta $k_\pm$, associated momentum fractions of Eq.\ \eqref{eq:def:kin:xn:xnbar}, and phase space boundaries of Eq.\ \eqref{eq:def:b.c.}. To this end, Fig.~\ref{fig:results:val:qTratios:asyexp:YH3} displays the \qT\ spectra at $|Y_H|=1$ and $|Y_H|=3$. We observe that the \qT~distributions at $|Y_H|=1$ generally observe similar patterns to those at $|Y_H|=0$ from Fig.~\ref{fig:results:val:qTratios:asyexp:YH0} for all three partonic channels, as $e^{\pm Y_H}$ is still more or less of $\order(1)$. At $|Y_H|=3$, where $e^{|Y_H|}$ is now of $\order(10)$, even though ability of the \LP approximation to reproduce the exact result is further reduced in the moderate domain, the higher power corrections are still convergent as before. More specifically, nearing $\qT=30\,\text{GeV}$, the \LP contribution to the process $gg\to Hg$ accounts for less than $60\%$ of the full theory, which is raised to nearly $80\%$ after including the \NLP corrections and about $97\%$ with the \NNLP terms. A marked difference, even at \NNLP, w.r.t.\ the central rapidity region is only observed at very high \qT\ around 50\,GeV. We would like to note that the non-monotonous behaviour of the \NLP result in Fig.~\ref{fig:results:val:qTratios:asyexp:ggHg:YH3} around $\qT\sim45\,\text{GeV}$ is caused by a changing sign of the \NLP approximants. \begin{figure}[t!] \centering \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth]{Plots_Diffs/qTDist_Log_AsyExp_ggHg_YHabs_1.pdf} \caption{ } \label{fig:results:val:qTdist:asyexp:ggHg:YH1} \end{subfigure} \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth]{Plots_Diffs/qTDist_Log_AsyExp_qgHq_YHabs_1.pdf} \caption{ } \label{fig:results:val:qTdist:asyexp:qgHq:YH1} \end{subfigure} \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth]{Plots_Diffs/qTDist_Log_AsyExp_qqHg_YHabs_1.pdf} \caption{ } \label{fig:results:val:qTdist:asyexp:qqHg:YH1} \end{subfigure} \\[2mm] \centering \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth]{Plots_Diffs/qTDist_Log_AsyExp_ggHg_YHabs_3.pdf} \caption{ } \label{fig:results:val:qTdist:asyexp:ggHg:YH3} \end{subfigure} \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth]{Plots_Diffs/qTDist_Log_AsyExp_qgHq_YHabs_3.pdf} \caption{ } \label{fig:results:val:qTdist:asyexp:qgHq:YH3} \end{subfigure} \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth]{Plots_Diffs/qTDist_Log_AsyExp_qqHg_YHabs_3.pdf} \caption{ } \label{fig:results:val:qTdist:asyexp:qqHg:YH3} \end{subfigure} \\[2mm] \centering \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth]{Plots_Diffs/qTDist_wt_Log_AsyExp_ggHg_YHabs_1.pdf} \caption{ } \label{fig:results:val:qTwt:asyexp:ggHg:YH1} \end{subfigure} \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth]{Plots_Diffs/qTDist_wt_Log_AsyExp_qgHq_YHabs_1.pdf} \caption{ } \label{fig:results:val:qTwt:asyexp:qgHq:YH1} \end{subfigure} \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth]{Plots_Diffs/qTDist_wt_Log_AsyExp_qqHg_YHabs_1.pdf} \caption{ } \label{fig:results:val:qTwt:asyexp:qqHg:YH1} \end{subfigure} \\[2mm] \centering \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth]{Plots_Diffs/qTDist_wt_Log_AsyExp_ggHg_YHabs_3.pdf} \caption{ } \label{fig:results:val:qTwt:asyexp:ggHg:YH3} \end{subfigure} \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth]{Plots_Diffs/qTDist_wt_Log_AsyExp_qgHq_YHabs_3.pdf} \caption{ } \label{fig:results:val:qTwt:asyexp:qgHq:YH3} \end{subfigure} \begin{subfigure}{0.32\textwidth} \centering \includegraphics[width=.9\linewidth]{Plots_Diffs/qTDist_wt_Log_AsyExp_qqHg_YHabs_3.pdf} \caption{ } \label{fig:results:val:qTwt:asyexp:qqHg:YH3} \end{subfigure} \\ \caption{ Differences of the \qT\ ($1^\text{st}\,\&\,2^\text{nd}$ row) and weighted \qT\ ($3^\text{rd}\,\&\,4^\text{th}$ row) spectra between the exact fixed-order calculation and the approximations for the three different partonic processes at $|Y_H|=1$ ($1^\text{st}\,\&\,3^\text{rd}$ row) and $|Y_H|=3$ ($2^\text{nd}\,\&\,4^\text{th}$ row). The solid (dashed) lines present the results including (excluding) the boundary corrections $\mathbf{B}_{cs}$ in Eq.~\eqref{eq:def:asyexp:mcfs:cs}, $\mathbf{B}_{\bar{c}s}$ in Eq.~\eqref{eq:def:asyexp:mcfs:cbars}, and $\mathbf{B}_{uc(\bar{c})}$ in Eq.~\eqref{eq:def:asyexp:mcfs:uc:ucbar}. The blue, green, and red lines detail the \LP, \NLP, and \NNLP approximations, respectively. } \label{fig:results:val:qTwt:asyexp:YH1:YH3} \end{figure} Finally, to assess the coefficients at each power, we investigate the difference between the exact (weighted) \qT~spectra and their approximations on different levels of the power expansion in Fig.~\ref{fig:results:val:qTwt:asyexp:YH1:YH3}. We find that the power series appraised in Sec.~\ref{sec:asyexp:outputs} is capable of reproducing the asymptotic behaviour of the full theory for both $|Y_H|=1$ and $|Y_H|=3$. Moreover, an interesting phenomenon can be observed here: the ranges that are sensitive to the boundary corrections grow with increasing rapidity $|Y_H|$ for all three partonic processes. For instance, the \NNLP accurate computation, represented by the green curves, shows discrepancies between the solid and dashed lines, which are driven by the boundary corrections, arise below $\qT\approx 0.4\,\text{GeV}$ in the $|Y_H|=1$ case in the $gg$ channel but already below $\qT\approx 1\,\text{GeV}$ in the $|Y_H|=3$ case. To interpret this behaviour, it merits recalling that in the central rapidity regime where $e^{\pm Y_H}\sim\order(1)$, the momentum fractions $x_n$ and $x_\nbar$ in Eq.~\eqref{eq:def:kin:xn:xnbar} both approach zero. Hence, while the interior contribution experiences no suppression from the PDFs, the boundary correction in Eq.~\eqref{eq:asyexp:deltaI:uc} does, suppressing it in the majority of the phase space. However, nearing the rapidity extremes $Y_H\to\pm 4.5$, one of $x_n$ and $x_\nbar$ approaches unity. Now, the interior contribution will be suppressed by one of the PDFs, analogous to that in Eq.~\eqref{eq:asyexp:deltaI:uc}, thereby losing its predominant role, relatively enlarging the boundary terms. \clearpage \section{Conclusions} \label{sec:conclusions} % general power expansion framework In this paper, we constructed a systematic and mathematically well-defined framework to construct a small-\qT\ expansion at \NLO up to arbitrary power accuracy. This framework is applicable to all possible conservative regulators of the emerging rapidity divergences, and we have shown that the results are identical for three radically different choices. In our power expansion we have refactored all \qT~dependences from the transition amplitudes and PDFs, except for those residing in the integration path and phase space boundaries. To achieve this, we have divided the phase space into two sectors, the interior of the integration domain and the segments in the vicinity of the integration boundaries. The contributions originating from the integration boundaries, which we have evaluated in this paper for the first time, are always associated with the PDF of the beam at the opposite side and, ultimately, give rise to power suppressed constant corrections at \NLO. We have summarised their analytic expressions in Eqs.~\eqref{eq:def:Gp} and \eqref{eq:asyexp:deltaI:ec:int}. The analysis of the contributions from the interior domain, on the other hand, is more involved due to the number of scales that are enclosed in the phase space integral. To derive the asymptotic series of the interior contributions, we have introduced a set of auxiliary cutoff scales to disentangle the scale hierarchies and in turn perform the appropriate power expansion. The recombination of all artificially separated contributions at each power removes all dependence on the auxiliary scales, such that the final result is independent of them. In any case, the contributions from the interior domain are comprised of three sectors, the $n$- and $\nbar$-collinear domains, and the zero-bin subtrahends. At a given $\omega$-th power, for example, the two collinear contributions can be derived by expanding the integrands according to the respective collinear scaling of the integration variable and projecting onto the $\omega$-th power contributions. Conversely, the zero-bin subtrahends are organised by dual-scalings, in which a second expansion of the $\omega$-th power collinear functions needs to be performed according to the soft scaling, giving contributions from the lowest power precision up to the $\omega$-th power. This algorithm is presented in Eqs.~\eqref{eq:def:asyexp:c:at:omega:nured:Texp} and \eqref{eq:def:c0:ns:Texp} in terms of the expansion operators. % application to pp->H+X To demonstrate the applicability of our algorithm, two additional fundamentally different rapidity regulators, the pure-rapidity and exponential regulators, in addition to the above cutoff scale regulator, have been embedded into Eqs.~\eqref{eq:def:asyexp:c:at:omega:nured:Texp}-\eqref{eq:def:c0:ns:Texp} in order to calculate the power corrections from the interior domain up to \NNLP accuracy, which we present here for the first time. We found that even though substantial differences emerge from the individual sectors in those two regularisation schemes, after summing all contributions both results produce the same power series as we have obtained via the momentum cutoffs. Together with the correction terms induced by the kinematical variables and the integral boundaries, we have derived analytic expressions for the expanded \qT~distribution for Higgs hadroproduction up to \NNLP, following Eq.~\eqref{eq:asyexp:tot}. To validate our results, we confronted the resulting power series approximation to the full QCD calculation at the same order. We have shown that our expanded \qT~spectra can satisfactorily replicate the desired qualities of the full theory for all contributing partonic channels at three different rapidity slices, $|Y_H|=0,1,3$. In particular, when including \NNLP corrections, the approximate predictions can capture the exact ones within (sub)percent level accuracy up to $\qT=30\,\text{GeV}$. In addition, to explore the relationship between the sizes of the different ingredients at a given power, we produced results without accounting for contributions stemming from the integral boundaries, a situation that may arise if PDFs and their derivatives are considered to vanish at the opposite in these regions. We found that the boundary contributions are generally small at \qT\ larger than a few GeV, but can play a decisive role as $\qT\to 0$. Here, their omission effectively degrades the \NLP and \NNLP results to \LP accuracy. %This is particularly relevant if a higher-power expanded result is to be used in a higher-order calculation using \qT-subtraction or -slicing. To give an example, the \NNLP corrections in the partonic process $q(\bar{q})g\to H q(\bar{q})$ are driven by the boundary corrections already at $\qT\lesssim 10\,\text{GeV}$ at $Y_H=3$. % Outlook towards further applications At last, it is worth emphasising that although Higgs hadroproduction is used as an example here to illustrate the capabilities and practicability of our results in Eq.~\eqref{eq:asyexp:tot}, the algorithm developed in this paper is expected to be directly applicable to the Drell-Yan family of processes and other colour-singlet processes containing similar denominators in the transition amplitudes. Furthermore, during our investigation, except for the indispensable ansatz made on the analytic properties of the PDFs, the power expansions are all carried out following a mathematically well-defined manner. % Therefore, we expect the conclusions from this work can not only serve as a robust recipe to derive the power series of the \qT\ distribution at NLO, but also offer the theoretical baseline for exploring the asymptotic properties of contributions at higher perturbative order. % \commentWJ{Novel contributions from this paper: % \begin{itemize} % \item I think we had better highlight ``We first make use of a mathematically well-defined approach to derive an algorithm to perform the small \qT\ expansion at NLO, that is applicable on a generic choice of rapidity regulator up to an arbitrary power accuracy. " Ref.~\cite{Jantzen:2011nz} has addressed similar point but his framework is only compatible with the homogeneous regulators. Refs.~\cite{Inglis-Whalen:2022vyn,Inglis-Whalen:2021bea} propose their approach based on the observation of the pole structure at NLP, which is basically a conjecture; % \item ``We first evaluate the power corrections induced by the asymptotic expansion of the boundary corrections, and numerically investigate their impacts at the first three power accuracies onto the double-differential observable $\done\sigma_H/(\done Y_H\done\qT^2)$". I find no boundary effects from Ref.~\cite{Ebert:2018gsn}. % \item ``We first present the \NNLP approximation for the \qT\ distributions in three different rapidity slices $|Y_H|=0,1,3$." Maybe we can also stress that ``\NNLP can be more important when applying the \qT\ subtraction onto the calculation at \NNLO\ and beyond, since the logarithmic contributions on higher perturbative level are generally enhanced than the NLO results, which in turn calls for stronger damping factors to render the power corrections under control. ". % \end{itemize} % } % \commentMS{Thanks, I'll think about working them into abstract and conclusion.} \subsection*{Acknowledgements} %GF is ??? % MS is funded by the Royal Society through a University Research Fellowship (URF\textbackslash{}R1\textbackslash{}180549 and URF\textbackslash{}R\textbackslash{}231031) and a Royal Society Enhancement Award (RGF\textbackslash{}EA\textbackslash{}181033, CEC19\textbackslash{}100349, and RF\textbackslash{}ERE\textbackslash{}210397). \section{Application and adaptation of the dissipative regulators}\label{sec:dis:reg} Here we will demonstrate that, after suitable adaptation, our zero-bin subtrahends in Eqs.~\eqref{eq:def:c0:ns:Texp} can also be utilized to the power expansion governed by the dissipative regulators. In the followings, we will illustrate this by implementing the $\Delta$- and $\eta$-regulators. \subsection{The~\texorpdfstring{$\Delta$}{Delta}-regulator} The~$\Delta$-regulator was proposed in \cite{Chiu:2009yx} to harness the rapidity divergence in the massive Sudakov factor, which was afterwards generalized in \cite{Echevarria:2011epo,Echevarria:2015usa,Echevarria:2015byo,Echevarria:2016scs} for fulfilling the restrictions from the non-abelian exponentiation theorem in the higher-perturbative order calculation. The method behind this regularization scheme is to shift the mass of the mediating particles in the transition amplitudes by an infinitesimal amount, such that approaching the rapidity extremities, i.e., $y_k\to\pm\infty$, the ensuing propagators can never reach the on-shell position and thus are always insulated from the rapidity divergences. The~$\Delta$-regulator is dedicated to the rapidity divergences at LP, as extra residual momenta can be generated during the expansion on the squared amplitudes beyond LP~\cite{Inglis-Whalen:2021bea}, which are singular in the limit $y_k\to\pm\infty$ and stay unprotected by the $\Delta$-regulator. To this end, in the following discussion, we will lay stress on the LP contribution. At LP, the zero-bin subtraction for the small~\qT~expansion primarily concerns the process $gg\to Hg$ up to NLO, which, as presented in Eq.~\eqref{eq:msq}, corresponds to the integrand $ I^{ -1,-1 }_{[\kappa], \{\alpha,\beta\} }$ based on the definition on Eq.~\eqref{eq:def:subjt}. Applying the~$\Delta$-regulator onto Eq.~\eqref{eq:def:subjt} with $\rho=\sigma=-1$ amounts to re-weight the squared amplitudes by a factor of, \begin{align} \label{eq:def:delta:rap} \mathcal{R} (k_-,k_+,\tau)\,=\,\frac{\qT^2}{(k_++\tau)\,(k_-+\tau)}\,, \end{align} where $\tau$ denotes an infinitesimal positive parameter. It is seen that $\mathcal{R} $ in Eq.~\eqref{eq:def:delta:rap} indeed satisfies the criteria of Eq.~\eqref{rap:def:feat}, which keeps void for the rapidity-safe integrands but becomes activated for the singular transition amplitudes. Substituting Eq.~\eqref{eq:def:delta:rap} into Eqs.~\eqref{eq:def:asyexp:c:at:omega:nured:Texp} and \eqref{eq:def:c0:ns:Texp} and then truncate out the corrections beyond LP, it yields, \begin{align} \label{eq:def:asyexp:c:at:omega:nured:delta} \widetilde{\mathcal{G}}^{-1,-1,(-1)}_{[\kappa],\{\alpha,\beta\} }\Bigg|^{\langle \Delta\rangle}_{c} =\, & \int^{\tilde{k}^{\mathrm{max}}_+}_{0} {\done k_+} \left[\frac{1}{k_+}\right]_*^{\nu_n} {F}^{(\beta_2)}_{i/N,\beta_1}\left(k_++m_H e^{-Y_H}\right) {F}^{(\alpha_2)}_{j/\bar{N},\alpha_1}\left(m_H e^{+Y_H}\right)\nnb\\ &+ \, {F}^ {(\beta_2 )}_{i/N,\beta_1}\left( m_H e^{-Y_H}\right)\, {F}^{ (\alpha_2 )}_{j/\bar{N},\alpha_1}\left(m_H e^{+Y_H}\right)\, \ln\left[\frac{\nu_n}{\tau}\right]\,,\\ \label{eq:def:asyexp:cbar:at:omega:nured:delta} \widetilde{\mathcal{G}}^{-1,-1,(-1)}_{[\kappa],\{\alpha,\beta\} }\Bigg|^{\langle \Delta \rangle}_{\bar{c}} =\, & \int^{{\frac{\qT^2}{\tilde{k}^{\mathrm{min}}_+}}}_0\, \done k_-\,\left[\frac{1}{k_- }\right]^{\nu_{\bar{n}}}_{*} \,{F}^{ (\beta_2 )}_{i/N,\beta_1}\left( m_H e^{-Y_H}\right)\, {F}^{(\alpha_2)}_{j/\bar{N},\alpha_1}\left(k_-+m_H e^{+Y_H}\right)\,\nonumber\\ &+ {F}^{ (\beta_2 )}_{i/N,\beta_1}\left( m_H e^{-Y_H}\right)\, {F}^{ (\alpha_2 )}_{j/\bar{N},\alpha_1}\left(m_H e^{+Y_H}\right)\, \ln\left[\frac{\nu_\nbar}{\tau}\right]\,, \end{align} and \begin{align} \label{eq:def:c0:cbar0:ns:delta} \widetilde{\mathcal{G}}^{-1,-1,(-1)}_{[\kappa],\{\alpha,\beta\} }\Bigg|^{\langle \mathrm{NS} \rangle, \langle \Delta \rangle}_{c0}\, =\,& \widetilde{\mathcal{G}}^{-1,-1,(-1)}_{[\kappa],\{\alpha,\beta\} }\Bigg|^{\langle \mathrm{NS} \rangle, \langle \Delta \rangle}_{\bar{c}0}\, =\, {F}^{(\beta_2 )}_{i/N,\beta_1}\left(m_H e^{-Y_H}\right)\,{F}^{(\alpha_2 )}_{j/\bar{N},\alpha_1}\left(m_H e^{+Y_H}\right)\, \ln\left[\frac{\qT}{\tau}\right]\,. \end{align} It is immediate to find that the difference between Eqs.~\eqref{eq:def:asyexp:c:at:omega:nured:delta}-\eqref{eq:def:asyexp:cbar:at:omega:nured:delta} and Eq.~\eqref{eq:def:c0:cbar0:ns:delta} exactly replicates the leading power outputs in Eqs.~\eqref{eq:def:asyexp:c:mom:at:omega}-\eqref{eq:def:asyexp:cbar:mom:at:omega} and Eqs.~\eqref{eq:def:asyexp:cs:mom:int}-\eqref{eq:def:asyexp:cbars:mom:int} derived via momentum cutoffs, those in Eqs.~\eqref{eq:def:asyexp:cbar:at:omega:nured:prap}-\eqref{eq:def:asyexp:c:at:omega:nured:prap} by means of the pure-rapidity regulator, or those in Eqs.~\eqref{eq:def:asyexp:c:at:omega:nured:exp}-\eqref{eq:def:c0:ns:exp} from the exponential one, after setting $\omega=\rho=\sigma=-1$ therein. \subsection{The~\texorpdfstring{$\eta$}{Eta}-regulator} The $\eta$-regulator was devised by~\cite{Chiu:2011qc,Chiu:2012ir} to facilitate the establishment of the rapidity renormalisation group equations in the SCET$_{\mathrm{II}}$-based analysis of the jet broadening and \qT~distributions. Akin to the analytic regularization prescription \cite{Becher:2010tm,Becher:2011dz}, the $\eta$-regulator concerns the momenta of the emitted partons raised by the power of $\tau$ as well. However, in place of the light-cone component $k_+$ or $k_-$ entailed in \cite{Becher:2010tm,Becher:2011dz}, the $\eta$-regulator puts the magnitude of the longitudinal one into the base, namely, \begin{align} \label{eq:def:eta:rap} \mathcal{R}(k_-,k_+,\tau)\,=\,\left|k_--k_+\right| ^{-\tau}. \end{align} Implementing the $\eta$-regularization scheme is rather subtle. In its original definition~\cite{Chiu:2011qc,Chiu:2012ir} and the recent review of \cite{Ebert:2018gsn}, the calculation on the collinear sector calls for the expansions of both the rapidity regulator in Eq.~\eqref{eq:def:eta:rap} and the integrand of Eq.~\eqref{eq:def:subjt}, which, based on the notation in Eq.~\eqref{eq:def:asyexp:c:at:omega:nured:Texp}, requires that $\mathcal{R}$ always appears to the right hand side of $ \widehat{\mathbf{T}}_{c}^{(\omega)}$ and $ \widehat{\mathbf{T}}_{\bar{c}}^{(\omega)}$. In doing this, a set of evanescent power corrections can be generated from Eq.~\eqref{eq:def:eta:rap}, which are proportional to $\tau$ (or its higher powers) and will make non-trivial contributions in combination with the pole terms. Those evanescent influences have not been taken into account during the derivation of Eqs.~\eqref{eq:def:asyexp:c:at:omega:nured:Texp}-\eqref{eq:def:c0:ns:Texp}, and therefore, it is not straightforward to apply Eq.~\eqref{eq:def:eta:rap} here until appropriate adaptations are put in place. In the following, we will introduce one of strategies to adapt the $\eta$-regulator to our formalism in Eqs.~\eqref{eq:def:asyexp:c:at:omega:nured:Texp}-\eqref{eq:def:c0:ns:Texp}. Considering that the main obstacle hindering this application comes from the evanescent contributions, it could be beneficial to maintain the regulator in Eq.~\eqref{eq:def:eta:rap} always to the left of the operators $ \widehat{\mathbf{T}}_{c}^{(\omega)}$ and $ \widehat{\mathbf{T}}_{\bar{c}}^{(\omega)}$ in practical calculations. In this way, Eq.~\eqref{eq:def:eta:rap} abides by the criteria of Eq.~\eqref{rap:def:feat} and can still serve as a qualified rapidity-divergence regularization scheme at any power accuracy. Furthermore, since the $\eta$-regulator at this moment does not participate into the expansion governed by $ \widehat{\mathbf{T}}_{c}^{(\omega)}$ and $ \widehat{\mathbf{T}}_{\bar{c}}^{(\omega)}$, one can save efforts in coping with the evanescent contribution. Now applying the $\eta$-regulator onto Eqs.~\eqref{eq:def:asyexp:c:at:omega:nured:Texp}-\eqref{eq:def:c0:ns:Texp} become immediate, which evaluate to, \begin{align} \label{eq:def:asyexp:c:at:omega:nured:etarap} \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|^{\langle \eta\rangle}_{c} =\, & \frac{\bar{\theta}\left(\omega-\sigma\right)}{(\omega-\rho)!} \int^{\tilde{k}^{\mathrm{max}}_+}_{0} \frac{\done k_+}{k_+} (k_+)^{\sigma-\omega} {F}^{(\beta_2)}_{i/N,\beta_1}\left(k_++m_H e^{-Y_H}\right) {F}^{(\alpha_2+\omega-\rho)}_{j/\bar{N},\alpha_1}\left(m_H e^{+Y_H}\right)\nnb\\ &\,+ \frac{\theta\left(\omega-\sigma\right)}{(\omega-\rho)!} \int^{\tilde{k}^{\mathrm{max}}_+}_{0} {\done k_+} \left[\frac{1}{k_+^{\omega-\sigma+1}}\right]_*^{\nu_n} {F}^{(\beta_2)}_{i/N,\beta_1}\left(k_++m_H e^{-Y_H}\right) {F}^{(\alpha_2+\omega-\rho)}_{j/\bar{N},\alpha_1}\left(m_H e^{+Y_H}\right)\nnb\\ & +\frac{\theta\left(\omega-\sigma-1\right)}{(\omega-\rho)!} \sum_{\eta=0}^{\omega-\sigma-1} \frac{ {F}^{(\beta_2+\eta)}_{i/N,\beta_1}\left( m_H e^{-Y_H}\right) {F}^{(\alpha_2+\omega-\rho)}_{j/\bar{N},\alpha_1}\left(m_H e^{+Y_H}\right)}{\eta!}\, \frac{\nu_n^{\sigma+\eta-\omega}}{\sigma+\eta-\omega} % \frac{\nu_n^{\sigma+\eta-\omega}}{\sigma+\eta-\omega} \nnb\\ &+ \frac{\theta( \omega-\sigma)}{(\omega-\rho)!} \, \frac{ {F}^ {(\beta_2+\omega-\sigma)}_{i/N,\beta_1}\left( m_H e^{-Y_H}\right)\, {F}^{ (\alpha_2+\omega-\rho)}_{j/\bar{N},\alpha_1}\left(m_H e^{+Y_H}\right)\,}{ (\omega-\sigma)!}\, %\left\{ \ln\left[\frac{\nu_n}{\qT}\right]-\frac{1}{2\tau}\right\} \left\{\ln\left[\frac{\nu_{n}}{\qT^2} \right]+\frac{1}{\tau} \right\}\,,\\ \label{eq:def:asyexp:cbar:at:omega:nured:etarap} \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|^{\langle \eta\rangle}_{\bar{c}} =& \frac{\bar{\theta}( \omega-\rho)}{(\omega-\sigma)!}\, \int^{{\frac{\qT^2}{\tilde{k}^{\mathrm{min}}_+}} }_0\,\frac{\done k_-}{k_-}\, k_-^{\rho-\omega}\, {F}^{ (\beta_2+\omega-\sigma)}_{i/N,\beta_1}\left( m_H e^{-Y_H}\right)\, {F}^{(\alpha_2)}_{j/\bar{N},\alpha_1}\left(k_-+m_H e^{+Y_H}\right) \,\nonumber\\ &+ \frac{{\theta}( \omega-\rho)}{(\omega-\sigma)!}\, \int^{{\frac{\qT^2}{\tilde{k}^{\mathrm{min}}_+}}}_0\, \done k_-\,\left[\frac{1}{k_-^{\omega-\rho+1}}\right]^{\nu_{\bar{n}}}_{*}\,{F}^{ (\beta_2+\omega-\sigma)}_{i/N,\beta_1}\left( m_H e^{-Y_H}\right)\, {F}^{(\alpha_2)}_{j/\bar{N},\alpha_1}\left(k_-+m_H e^{+Y_H}\right)\,\nonumber\\ &+ \frac{{\theta}( \omega-\rho-1)}{(\omega-\sigma)!}\,\sum_{\lambda=0}^{\omega-\rho-1}\, \frac{ {F}^{ (\beta_2+\omega-\sigma)}_{i/N,\beta_1}\left( m_H e^{-Y_H}\right)\, {F}^{ (\alpha_2+\lambda)}_{j/\bar{N},\alpha_1}\left(m_H e^{+Y_H}\right)\,}{ \lambda!} \, \frac{\nu_\nbar^{\rho+\lambda-\omega}}{\rho+\lambda-\omega}\nonumber\\ % \frac{ \nu_{\bar{n}}^{\rho+\lambda-\omega}}{\rho+\lambda-\omega}\, &+ \frac{ {\theta}( \omega-\rho)}{(\omega-\sigma)!}\, %\left\{\ln\left[\frac{\nu_{\bar{n}}}{\qT}\right]+\frac{1}{2\tau}\right\}\, \frac{ {F}^{ (\beta_2+\omega-\sigma)}_{i/N,\beta_1}\left( m_H e^{-Y_H}\right)\, {F}^{ (\alpha_2+\omega-\rho)}_{j/\bar{N},\alpha_1}\left(m_H e^{+Y_H}\right)\,}{ (\omega-\rho)!} \, \left\{\ln\left[\frac{\nu_{\nbar}}{\qT^2} \right]+\frac{1}{\tau} \right\}\,, \end{align} together with the subtraction terms, \begin{align} \label{eq:def:c0:ns:etarap} \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|^{\langle \mathrm{NS} \rangle, \langle \eta \rangle}_{c0}\, =\,& \theta\left(\omega-\sigma \right) \frac{{F}^{(\beta_2+\omega-\sigma)}_{i/N,\beta_1}\left(m_H e^{-Y_H}\right)\,{F}^{(\alpha_2+\omega-\rho)}_{j/\bar{N},\alpha_1}\left(m_H e^{+Y_H}\right)}{(\omega-\sigma)!\, (\omega-\rho)!} \left\{\ln\left[\frac{1}{\qT } \right]+\frac{1}{\tau} \right\} ,\\ \label{eq:def:cbar0:ns:etarap} \widetilde{\mathcal{G}}^{\rho,\sigma,(\omega)}_{[\kappa],\{\alpha,\beta\} }\Bigg|^{\langle \mathrm{NS} \rangle, \langle \eta \rangle}_{\bar{c}0}\, =\,& \theta\left(\omega-\rho\right) \frac{{F}^{(\beta_2+\omega-\sigma)}_{i/N,\beta_1}\left(m_H e^{-Y_H}\right)\,{F}^{(\alpha_2+\omega-\rho)}_{j/\bar{N},\alpha_1}\left(m_H e^{+Y_H}\right)}{(\omega-\sigma)!\, (\omega-\rho)!} \left\{\ln\left[\frac{1}{\qT } \right]+\frac{1}{\tau} \right\}\,. \end{align} Subtracting Eqs.~\eqref{eq:def:c0:ns:etarap}-\eqref{eq:def:cbar0:ns:etarap} from Eqs.~\eqref{eq:def:asyexp:c:at:omega:nured:etarap}-\eqref{eq:def:asyexp:cbar:at:omega:nured:etarap}, it reproduces the results in Eqs.~\eqref{eq:def:asyexp:c:mom:at:omega}-\eqref{eq:def:asyexp:cbar:mom:at:omega} and Eqs.~\eqref{eq:def:asyexp:cs:mom:int}-\eqref{eq:def:asyexp:cbars:mom:int} obtained from momentum cutoffs, and also those in Sec.~\ref{sec:asyexp:outputs} by means of pure-rapidity and exponential regularization schemes. \section{Comparison of the NLP results with the previous literature}\label{sec:comp:nlp} Subleading power corrections on the process $pp\to H+X$ have been investigated in \cite{Ebert:2018gsn} as well by means of the $\eta$- and pure rapidity regulators. Here we take the partonic process $q\bar{q}\to H g$ as an illustrative example to compare the expressions in \cite{Ebert:2018gsn} and those in Eq.~\eqref{eq:def:asyexp:mcfs:cs}, \eqref{eq:def:asyexp:mcfs:cbars}, and \eqref{eq:def:asyexp:mcfs:c}. Over the course, we will particularly emphasis the interior contributions encoded by the partonic matrices $\mathbf{P}$, $\mathbf{D}$, and $\mathbf{R}$, as the boundary corrections in $\mathbf{B}$ are related to the PDFs at the opposite end, which are all assumed to be vanishing in \cite{Ebert:2018gsn}. In \cite{Ebert:2018gsn}, the analytic results for the channel $q\bar{q}\to H g$ entail the expanded amplitudes of Eq.~\eqref{eq:msq} sandwiched by the (derivatives of) PDFs. Recasting their expressions into the matrix form according to the bases in Eq.~\eqref{eq:PDF:N:ary} and also synchronizing the pre-factors in line with Eq.~\eqref{eq:def:asyexp:mcfs:cs}, we obtain \begin{align} \label{eq:sing:qq:Ebert18} \widehat{\mathbf{P}}_{cs}^{(0),q \bar{q} } =& \widehat{\mathbf{P}}_{\bar{c}s}^{(0),q \bar{q} } = \widehat{\mathbf{D}}_{cs}^{(0),q \bar{q} }= \widehat{\mathbf{D}}_{\bar{c}s}^{(0),q \bar{q} }=0\,,\\ \label{eq:Rcs:qq:Ebert18} \widehat{\mathbf{R}}_{cs}^{(0),q \bar{q} } =& \left[ \begin{array}{cc} -\frac{32}{27}+\frac{16}{27 z_n}+\frac{16}{27 z_n^2} \\[2.ex] \frac{16}{27}-\frac{32}{27 z_n}+\frac{16}{27 z_n^2} \\ \end{array} \right]\,,\\ \label{eq:Rcbars:qq:Ebert18} \widehat{\mathbf{R}}_{\bar{c}s}^{(0),q \bar{q} } = & \left[ \begin{array}{cc} -\frac{32}{27}+\frac{16}{27 z_\nbar}+\frac{16}{27 z_\nbar^2} & \frac{16}{27}-\frac{32}{27 z_\nbar}+\frac{16}{27 z_\nbar^2} \\ \end{array} \right]\,, \end{align} where the hatted bold matrices encode the outcome from \cite{Ebert:2018gsn}. It is immediate to see that the matrices in Eq.~\eqref{eq:sing:qq:Ebert18}~associated with the plus distribution and delta function are all zero, echoing the outputs from this work in Eq.~\eqref{eq:Dcs:lp_nlp_nnlp}, \eqref{eq:Pcs:gg_gq_qq}, and \eqref{eq:Xcbars:nnlp}, whereas, due the emergence of the extra off-diagonal entries in Eqs.~\eqref{eq:Rcs:qq:Ebert18}-\eqref{eq:Rcbars:qq:Ebert18}, the regular contributions from \cite{Ebert:2018gsn} appear to observe distinct patterns from ours in Eq.~\eqref{eq:Rcs:qq} and Eq.~\eqref{eq:Xcbars:nnlp}. As a matter of fact, this kind of difference can be resolved by applying the method of integration by parts as appropriate. From Eq.~\eqref{eq:PDF:N:ary}, the off-diagonal terms in Eqs.~\eqref{eq:Rcs:qq:Ebert18}-\eqref{eq:Rcbars:qq:Ebert18} always invoke the derivatives of one of the PDFs, which, via the integration by parts, can be in turn transformed into the PDFs multiplied by the derivatives of the original integrands, up to a few of boundary terms, more specifically, \begin{align} \int_{x_n}^{1}\, \done z_n\, \frac{x_n}{z_n}f'_{i/N}\left( \frac{x_n}{z_n}\right)\, f_{j/\bar{N}}\left( x_\nbar \right)\, g(z_n)\, =&\, \int_{x_n}^{1}\, \done z_n\, f_{i/N}\left( \frac{x_n}{z_n}\right)\, f_{j/\bar{N}}\left( x_\nbar \right)\, \frac{\partial\,g(z_n)}{\partial\,\ln(z_n)}\,\nonumber\\ &\,-\,f_{i/N}\left(x_n\right)\, f_{j/\bar{N}}\left( {x_\nbar}\right)\,g_n(1)\, +\,b.c.\,,\\ \int_{x_\nbar}^{1}\, \done z_\nbar\, f_{i/N}\left( x_n \right)\, \frac{x_\nbar}{z_\nbar}f'_{j/N}\left( \frac{x_\nbar}{z_\nbar}\right)\, g_n(z_\nbar)\, =&\, \int_{x_\nbar}^{1}\, \done z_\nbar\, f_{i/N}\left( x_n \right)\, f_{j/\bar{N}}\left( \frac{x_\nbar}{z_\nbar}\right)\, \frac{\partial\,g_\nbar(z_\nbar)}{\partial\,\ln(z_\nbar)}\,\nonumber\\ &\,-\,f_{i/N}\left(x_n\right)\, f_{j/\bar{N}}\left( {x_\nbar}\right)\,g_\nbar(1)\, +\,b.c.\,, \end{align} where $g_n(z_n)$ and $g_\nbar(z_\nbar)$ represent the two regular functions with finite derivatives across the domains $z_n\in[x_n,1]$ and $z_\nbar\in[x_\nbar,1]$, respectively. Applying those two relations onto Eqs.~\eqref{eq:Rcs:qq:Ebert18}-\eqref{eq:Rcbars:qq:Ebert18}, the off-diagonal entries therein are both eliminated and then, our results in Eq.~\eqref{eq:Rcs:qq} and Eq.~\eqref{eq:Xcbars:nnlp} are literally replicated. % Analogous strategy can also be utilised in comparing the outcomes of the processes $gg\to Hg$ and $q(\bar{q})g \to Hq(\bar{q})$. \section{Small \texorpdfstring{\qT}{qT} expansion for multi-boson hadroproduction}\label{sec:asyexp:Bs} Here we will demonstrate that after appropriate generalization, the method in Sec.~\ref{sec:asyexp:mom} can also be used in the power expansion on the hadroproduction of the multiple color-singlet bosons, i.e., $pp\to \{B_n\}+X$. Here a set of electroweak (or Higgs) bosons are collected within the curly brackets $\{B_n\}\equiv\{B_1,B_2,B_3,\dots B_n\}(n\ge2)$. We start with the analysis of the fixed-order results. According the QCD factorization, the differential \qT\ distributions at NLO can be expressed as, \begin{align}\label{eq:qT:Bi} \frac{\done \sigma_B}{\done\Phi_n\, \done^2\qTvec} \;= & \frac{1}{2^{4n}\,\pi^{3n-1}\, s^2}\sum_{i,j}\, \int^{k_+^{\mathrm{max}}}_{k_+^{\mathrm{min}}}\, \frac{\done k_+}{k_+} \frac{f_{i/n}(\xi_n)}{\xi_n} \frac{f _{j/\nbar}(\xi_{\nbar})}{\xi_{\nbar}}\; \overline{\sum_{\mathrm{col},\mathrm{pol}} } \big|\mathcal{M}(i+j\to \{B_n\}+k)\big|^2\,. \end{align} Now $\qT$ represents the transverse momentum of the whole colorless system $\{B_n\}$. The differential $\done\Phi_n$ collects the differentials for the rapidity $y_i$ and transverse momentum $\vec{k}^i_{\bot}$ of the $i$th boson, \begin{align}\label{eq:dPhi:Bi} % \done\Phi_n=\,\frac{1}{N_{\mathrm{id}}}\prod_{i=1}^n\,\left(\frac{1}{2}\,\frac{\done y_i}{2\pi}\,\frac{\done^2\vec{k}^i_{\bot}}{(2\pi)^2}\right)\,\delta^2\left(\qTvec-\sum_{i=1}^{n-1}\vec{k}^{i }_{\bot}\right)\,. \done\Phi_n=\left(\prod_{i=1}^n\done y_i\right)\left(\prod_{i=1}^{n-1}\done^2\vec{k}^i_{\bot}\right)\,. \end{align} Here only the transverse momenta of the first $n-1$ partons have been spelled out, as the last one is subjected to the momentum conservation condition, \begin{align} \vec{k}^n_{\bot}=\qTvec-\sum_{i=1}^{n-1}\vec{k}^i_{\bot}\,. \end{align} On the l.h.s of Eq.~\eqref{eq:qT:Bi}, the integrand concerns the momentum fractions $\xi_n$ and $\xi_\nbar$, which can be determined by the momentum conservation condition on the longitudinal direction, \begin{align}\label{eq:def:ppBn:XinXinbar} \xi_n\,=\,\frac{1}{\sqrt{s}}\,\left(k_+\,+\,\sum_{i=1}^n\mT^ie^{-y_i}\right)\,,\qquad \xi_\nbar\,=\,\frac{1}{\sqrt{s}}\,\left(k_-\,+\,\sum_{i=1}^n\mT^ie^{+y_i}\right)\,. \end{align} Here $k_{\pm}$ stands for the light-cone components of the emitted colorful particle as defined in Eq.~\eqref{eq:def:lcone}. $\mT^i$ reveals the transverse mass for the $i$th boson. According to the conditions $\xi_n\le1$ and $\xi_\nbar\le1$, we can then evaluate the boundaries for the $k_+$-integral in Eq.~\eqref{eq:qT:Bi}, \begin{align} k_+^{\mathrm{max}}\,=\,{\sqrt{s}}\,-\,\sum_{i=1}^n\mT^ie^{-y_i} \,,\qquad k_-^{\mathrm{max}}\,=\, \frac{\qT^2}{k_+^{\mathrm{min}}}\,=\, {{\sqrt{s}}\,- \,\sum_{i=1}^n\mT^ie^{+y_i} }\,. \end{align} The calculation on Eq.~\eqref{eq:qT:Bi} also entails the squared amplitudes for the ensuing partonic process $i+j\to \{B_n\}+k$. On the tree level, the Feynman diagrams presiding over this transition can be categorized into two groups: (A) the topology that the final color-singlet bosons are all directly connected to the initial partons; (B) the one that at least one of the final color-singlet bosons is emitted from the finial QCD parton. The representative circumstances on those two topologies have been illustrated in Fig.~\ref{fig:Bn:IE} and Fig.~\ref{fig:Bn:FE}. The topology (A) is expected to govern the partonic channel $q\bar{q}\to \{B_n\}+k$ with $\{B_n\}$ comprising only the electroweak vector bosons and the one $q(\bar{q})g\to \{B_n\}+q(\bar{q})$ with $\{B_n\}$ including only Higgs bosons. In the other circumstances, the contributions from topology (B) have to be addressed as appropriate. However, it merits noting that in topology (B), the emission off the QCD parton will leave all the propagators in the ensuing Feynman diagrams away from the threshold by $\mathcal{O}(m^i_{B})$, where $m^i_{B}$ indicates the mass of the $i$th final colorless boson, such that the leading singular behaviour of the process $pp\to\{B_n\}+X$ is entirely captured by the configuration (A). %, with the topology (B) only serving the power corrections at NLP and beyond. Without any loss of generality, the matrix elements induced by those two topologies can be recast in the following forms, \begin{align} \label{eq:def:ppBn:M2:TA} & \overline{\sum_{\mathrm{col},\mathrm{pol}} } \big|\mathcal{M}(i+j\to \{B_n\}+k)\big|^2\Bigg|_{\mathbf{(A)}}\, \nonumber\\ =&\, \sum_{F\in\mathbf{T}_{\mathbf{A}}}\,\lambda_{ijk}(F)\,\left[\prod_{ n=1}^{\mathbf{card}[I_{F}]} \left(p_i-\sum_{l\in I_{F}^{(n)}} k_l\right)^{-2} \right]\,\left[\prod_{m=1}^{\mathbf{card}[J_{F}]}\ \left(p_j-\sum_{l\in J_F^{(m)}}k_l\right)^{-2}\right]\, \sum_{\rho,\sigma}\,k^{\rho}_{-}\,k^{\sigma}_{+}\, \left( \widetilde{\mathcal{K}}_{\bot}{\cdot}\widetilde{\mathcal{E}}^{\rho\sigma}_{F} \right)\,, \\ \label{eq:def:ppBn:M2:TB} & \overline{\sum_{\mathrm{col},\mathrm{pol}} } \big|\mathcal{M}(i+j\to \{B_n\}+k)\big|^2\Bigg|_{\mathbf{(B)}}\, \nonumber\\ =&\, \sum_{F\in\mathbf{T}_{\mathbf{B}}}\,\lambda_{ijk}(F)\,\left[\prod_{ n=1}^{\mathbf{card}[I_{F}]} \left(p_i-\sum_{l\in I_{F}^{(n)} }k_l\right)^{-2} \right]\,\left[\prod_{m=1}^{\mathbf{card}[J_{F}]}\, \left(p_j-\sum_{l\in J_F^{(m)} }k_l\right)^{-2}\right]\,\left[\prod_{h=1}^{\mathbf{card}[K_{F}]} \left( k+\sum_{l\in K_F^{(h)} }k_l\right)^{-2} \right]\,\nonumber\\ & \times\, \sum_{\rho,\sigma}\,k^{\rho}_{-}\,k^{\sigma}_{+}\, \left( \widetilde{\mathcal{K}}_{\bot}{\cdot}\widetilde{\mathcal{E}}^{\rho\sigma}_{F} \right) \,. \end{align} Here $F$ denotes the Feynman diagrams driving the process $i+j\to \{B_n\}+k$, which, at LO, belongs to either topology $\mathbf{T}_{\mathbf{A}}$ or $\mathbf{T}_{\mathbf{B}}$. $\lambda_{ijk}(F)$ collects the coupling constants, color factors, and average factors for the initial states and the final identical particles. $I_F$ and $J_F$ encode two sets of colorless particles emitted from the initial partons $i$ and $j$, respectively. For instance, if the squared amplitudes are induced by the configuration in Fig.~\ref{fig:Bn:IE} and its complex conjugate, we have $I_F=\{I_F^{(1)}, I_F^{(2)}\}$ with $I_F^{(1,2)}=B_1$ and $J_F=\{J_F^{(1)}, J_F^{(2)}, J_F^{(3)}, J_F^{(4)},\dots \}$ with $J_F^{(1,2)}=B_n$, $J_F^{(3,4)}=\{B_{n-1},B_n\}$, etc. The number of the elements in each set is evaluated by the cardinality operator $\mathbf{card}$. With the help of $I_F$ and $J_F$, one can specify the expressions of the denominators in a given Feynman diagram as presented in the square brackets in Eqs.~(\ref{eq:def:ppBn:M2:TA}-\ref{eq:def:ppBn:M2:TB}). \begin{figure}[t!] \centering \includegraphics[width=.6\linewidth, height=0.15\linewidth]{FeynDiags_ppVVV/Initial_Emission_chopped.pdf} \caption{ Representative diagram of the topology that the final color-singlet bosons are all directly connected to the initial partons. Here the dashed lines stand for the colorful particles, while wave lines indicate the color-singlet bosons. } \label{fig:Bn:IE} \end{figure} \begin{figure}[t!] \centering \includegraphics[width=.6\linewidth, height=0.15\linewidth]{FeynDiags_ppVVV/Final_Emission_chopped.pdf} \caption{ Representative diagram of the topology that the final color-singlet bosons are in part connected to the finial QCD parton. Here the dashed lines stand for the colorful particles, while wave lines indicate the color-singlet bosons. } \label{fig:Bn:FE} \end{figure} To express the numerators of the squared amplitudes, we introduce the arrays $\widetilde{\mathcal{K}}_{\bot}$ and $\widetilde{\mathcal{E}}^{\rho\sigma}_{F}$, \begin{align} \label{eq:def:ppBn:KT} \widetilde{\mathcal{K}}_{\bot}=&\left[1,(\qTvec)_{i_1},(\qTvec)_{i_2}(\qTvec)_{j_2},(\qTvec)_{i_3}(\qTvec)_{j_3}(\qTvec)_{k_3},\dots\right]\,,\\ \label{eq:def:ppBn:ET} \left(\widetilde{\mathcal{E}}^{\rho\sigma}_{F}\right)^{\mathbf{T}}=&\left[E^{\rho\sigma,(0)}_{F},\sum_l\, (\vec{k}_{\bot}^l)_{i_1}\,E^{\rho\sigma,(1_{\rm{S}})}_{F,l}+\sum_l\,(\tilde{k}_{\bot}^l)_{i_1}\,E^{\rho\sigma,(1_{\rm{A}})}_{F,l}, \epsilon^{i_2j_2}_{\bot}E^{\rho\sigma,(2_{\rm{AA}})}_{F}+\,\sum_{l_1,l_2}\, (\vec{k}_{\bot}^{l_1})_{i_2}\,(\vec{k}_{\bot}^{l_2})_{j_2}\,E^{\rho\sigma,(2_{\rm{SS}})}_{F,l_1,l_2}\,\right. \nonumber\\ & \left. +\,\sum_{l_1,l_2}\, (\tilde{k}_{\bot}^{l_1})_{i_2}\,(\vec{k}_{\bot}^{l_2})_{j_2}\,E^{\rho\sigma,(2_{\rm{AS}})}_{F,l_1,l_2}\,+\,\sum_{l_1,l_2}\, (\vec{k}_{\bot}^{l_1})_{i_2}\,(\tilde{k}_{\bot}^{l_2})_{j_2}\,E^{\rho\sigma,(2_{\rm{SA}})}_{F,l_1,l_2}\,,\dots\right]\,. \end{align} Here $\widetilde{\mathcal{K}}_{\bot}$ consists of the tensors constructed by the momentum \qTvec\ in different ranks, while $\widetilde{\mathcal{E}}^{\rho\sigma}_{F}$ collects those formed by $k^{\mu}_{i}$ with $i\in[1,n]$. To accommodate the asymmetric behaviour induced by the Dirac traces that contain $\gamma_5$, we introduce $\epsilon^{\rho\sigma}_{\bot}=\epsilon^{\mu\nu\rho\sigma}n_{\mu}\nbar_{\nu}$ and $(\tilde{k}_{\bot})^{\rho}=\epsilon^{\rho\sigma}_{\bot}\vec{k}_{\bot,\sigma}$ in Eq.~\eqref{eq:def:ppBn:ET}, where $\epsilon^{\mu\nu\rho\sigma}$ denotes the customary anti-symmetric tensor. The coefficients $E^{\rho\sigma,(m)}_{F,\{l\}}$ in charge of tensor structures as specified in ``$(m)$" encode the hard scales $\mT^ie^{\pm y_i}$, $\left(\vec{k}^i_{\bot}{\cdot}\vec{k}^j_{\bot}\right)$, and $\left(\tilde{k}^i_{\bot}{\cdot}\vec{k}^j_{\bot}\right)$. In the following, we will show that the \qT\ spectra induced by the topology (A) can be all expanded following the method developed in Sec.~\ref{sec:asyexp:mom}. First of all, it should be noted that in Eq.~\eqref{eq:def:ppBn:M2:TA}, all the dependences on the integration variable $k_{\pm}$ have been taken out from the numerator, while the denominators, after evaluating the scaling products, present only the linear dependences on $k_{\pm}$, more explicitly, \begin{align} \label{eq:def:ppBn:sp:kp} \left(p_i-\sum_{l\in X}k_l\right)^{2}\equiv& \left(p_i-k_X\right)^{2}= -\mT^Xe^{y_X}\left(k_++\sum_{l\notin X}\mT^l e^{-y_l}+\frac{|\vec{k}^X_{\bot}|^2}{\mT^Xe^{y_X}}\right)\,,\\ \label{eq:def:ppBn:sp:km} \left(p_j-\sum_{l\in X}k_l\right)^{2}\equiv& \left(p_j-k_X\right)^{2}= -\mT^Xe^{-y_X}\left(k_-+\sum_{l\notin X}\mT^l e^{y_l}+\frac{|\vec{k}^X_{\bot}|^2}{\mT^Xe^{-y_X}}\right)\,. \end{align} Therein, $k_X$ represents the total momentum of the particles belong to the set $X$, from which we are able to calculate the transverse mass $\mT^X$ and rapidity $y_X$ for this colorless system. The factorized form in Eqs.~(\ref{eq:def:ppBn:sp:kp}-\ref{eq:def:ppBn:sp:km}) then allows us to re-categorize the dominators in Eq.~\eqref{eq:def:ppBn:M2:TA} according to their $k_{\pm}$-dependences, more explicitly, \begin{equation} \label{eq:ppBn:qcd:qT:kpm} \begin{split} \frac{\done \sigma_B}{\done\Phi_n\, \done^2\qTvec}\Bigg|_{\mathbf{(A)}} \,=&\; \sum_{F\in\mathbf{T}_{\mathbf{A}}}\, \sum_{\rho,\sigma } \, \left( \widetilde{\mathcal{K}}_{\bot}{\cdot}\widetilde{\mathcal{H}}^{\rho\sigma}_{F} \right) \, \int^{k_+^{\mathrm{max}}}_{k_+^{\mathrm{min}}} \frac{\done k_+}{k_+}\; (k_-)^{\rho} \, (k_+)^{\sigma} \, \widehat{F}^{\{0\}}_{i/n,\{\beta_n\}}\left(k_+,\{Q_n\},\{I_F\}\right)\, \\ &\times\; \widehat {F}^{\{0\}}_{j/\nbar,\{\beta_\nbar\}}\left(k_-,\{Q_\nbar\},\{J_F\}\right)\,, \end{split} \end{equation} where the novel array $\widetilde{\mathcal{H}}^{\rho\sigma}_{F}$ emerges, which is defined analogously to Eq.~\eqref{eq:def:ppBn:ET} but can absorb extra hard scales as a result of the denominator decomposition in Eqs.~(\ref{eq:def:ppBn:sp:kp}-\ref{eq:def:ppBn:sp:km}). Within the integral, all the $k_{\pm}$ reliances from the PDFs and denominators of the squared amplitudes have been collected in the generalized functions $\widehat{F}^{\{\alpha_n\}}_{i/n,\{\beta_n\}}$ and $ \widehat {F}^{\{\alpha_\nbar\}}_{j/\nbar,\{\beta_\nbar\}}$, \begin{align} \label{eq:def:ppBn:FioN} & \widehat{F}^{\{\alpha_n\}}_{i/n,\{\beta_n\}}\left(k_+,\{Q_n\},\{I_F\}\right)\nonumber\\ \equiv \,& \frac{\partial^{\alpha^{(-1)}_n}}{\partial (k_+)^{\alpha^{(-1)}_n}} \left\{ \prod_{l=0}^{\mathbf{card}[I_F]} \frac{\partial^{\alpha^{(l)}_n}}{\partial (Q^{(l)}_n)^{\alpha^{(l)}_n}}\right\} \left[ \frac{ f_{i/n}\left(\frac{k_++Q^{(0)}_n}{\sqrt{s}}\right)}{k_++Q^{(0)}_n} \right]\prod_{h=1}^{\mathbf{card}[I_F]}\left(k_++Q^{(h)}_n\right)^{-\beta^{(h)}_n}\,,\\ & \widehat {F}^{\{\alpha_\nbar\}}_{j/\nbar,\{\beta_\nbar\}}\left(k_-,\{Q_\nbar\},\{J_F\}\right)\nonumber\\ \label{eq:def:ppBn:FioNbar} \equiv \,& \frac{\partial^{\alpha^{(-1)}_\nbar}}{\partial (k_-)^{\alpha^{(-1)}_\nbar}} \left\{ \prod_{l=0}^{\mathbf{card}[J_F]} \frac{\partial^{\alpha^{(l)}_\nbar}}{\partial (Q^{(l)}_\nbar)^{\alpha^{(l)}_\nbar}}\right\} \left[ \frac{ f_{j/\nbar}\left(\frac{k_-+Q^{(0)}_\nbar}{\sqrt{s}}\right)}{k_-+Q^{(0)}_\nbar} \right]\prod_{h=1}^{\mathbf{card}[J_F]}\left(k_-+Q^{(h)}_\nbar\right)^{-\beta^{(h)}_\nbar}\,, \end{align} where $\{Q_n,Q_\nbar\}$ signify two sets of hard scales. $Q_n^{(0)}$ and $Q_\nbar^{(0)}$ can be extracted from the fractions in Eq.~\eqref{eq:def:ppBn:XinXinbar}, while $Q_n^{(l)}$ and $Q_\nbar^{(l)}$ with $l\ge1$ are derived by matching onto Eqs.~(\ref{eq:def:ppBn:sp:kp}-\ref{eq:def:ppBn:sp:km}). In comparison with the functions ${F}^{(\alpha_n)}_{i/n,\beta_n}$ and ${F}^{(\alpha_\nbar)}_{j/\nbar,\beta_\nbar}$ in Eq.~\eqref{eq:def:FioN:FjoNbar}, Eqs.~(\ref{eq:def:ppBn:FioN}-\ref{eq:def:ppBn:FioNbar}) here observe structural similarity but call for more indices to accommodate the input scales, such as $\alpha^{(h)}_{n/\nbar}$ presiding over the orders of the derivatives of the kinematics variables and $\beta^{(h)}_{n/\nbar}$ controlling the exponents of the various denominators $(k_{\pm}+Q^{(h)}_{n/\nbar})$. Equipped with those results, in Eq.~\eqref{eq:ppBn:qcd:qT:kpm}, we manage to transform the \qT\ distribution into its $k_{+}/k_-$-factorised formulation as in Eq.~\eqref{eq:qcd:qT:kpm}, for which the power expansion can be carried out by repeating the procedures in Sec.~\ref{sec:setups}, Sec.~\ref{sec:red:qT:boundary}, and Sec.~\ref{sec:red:qT:central}. However, if the contribution related to $\mathbf{T}_{\mathbf{B}}$ is of one's concern, the small \qT\ expansion becomes more involved. To see this, it is worth recalling that extra type of propagators appear from the third square bracket of Eq.~\eqref{eq:def:ppBn:M2:TB}, which prompts the quadratic dependences on $k_{\pm}$ upon evaluating the scalar products, \begin{align}\label{eq:def:ppBn:sp:kX} \left( k+\sum_{l\in X}k_l\right)^{2}\equiv& \left(k+k_X\right)^{2}\,=\,k_+\mT^Xe^{y_X}+k_-\mT^Xe^{-y_X}+m_X^2-2\qTvec\cdot\vec{k}_{\bot}^X\,. \end{align} At this moment, it is not straightforward to derive the factorized form for the squared amplitudes of Eq.~\eqref{eq:def:ppBn:M2:TB} as in Eq.~\eqref{eq:ppBn:qcd:qT:kpm}, which therefore defies an immediate implementation of the frameworks in Sec.~\ref{sec:asyexp:mom}. Promisingly, the power series of the $\mathbf{T}_{\mathbf{B}}$-induced contributions can also be derived via a set of dynamic regions from the phase space. However, more considerations and efforts should be paid to work out a group of auxiliary cutoffs that are capable of unambiguously and consistently separating all the relevant scales embedded by Eq.~\eqref{eq:def:ppBn:sp:kX}. Hence, we postpone this part of discussion to the further investigations. 
